Embodied Robot Manipulation in the Era of Foundation Models: Planning and Learning Perspectives

Recent advances in vision, language, and multimodal learning have significantly accelerated progress in robotic foundation models, with robotic manipulation remaining one of the most challenging embodied tasks. Its difficulty lies in integrating perception, semantic understanding, task reasoning, physically grounded action generation, and reliable execution. This survey examines robotic manipulation from an algorithmic perspective and organizes recent learning-based approaches through a unified abstraction of high-level planning and low-level action modeling. At the high level, we extend the classical notion of task planning to include reasoning over language, code, affordances, geometric constraints, and 3D representations. At the low level, we present a learning-paradigm-oriented taxonomy of learning-based action models, covering input modeling, latent learning, and policy learning. Within this abstraction, foundation models contribute either by generating structured planning artifacts that are instantiated as constraints or latent inputs for downstream action generation, or by directly modeling executable actions and trajectories. Finally, we summarize open challenges and future directions related to scalability, generalization, data efficiency, multimodal physical interaction, and safety. Together, this survey provides a structured view of the design space and emerging trends in foundation models for robotic manipulation.

==> figures/1_intro/summary.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{imgs/1_intro/summary.pdf}  
\caption{Overview of the survey. We provide 
% a broad introduction to benchmarks, datasets, and manipulation tasks, followed by 
an extensive introduction to embodied manipulation, including high-level planner and low-level controller. Our introduction to the low-level controller mainly focuses on the learning-based strategy.}
\label{fig: summary}
\end{figure*}

==> figures/2_background/hardware.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{imgs/2_background/hardware.pdf}  
\caption{Overview of Hardware Platforms.}
\label{fig: handware}
\end{figure*}

==> figures/3_benchmarks/benchmark.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{imgs/3_benchmarks/benchamrk.pdf}  
\caption{Overview of simulators and benchmarks.
$^1$Basic Manipulation with Single Arm, $^2$Basic Manipulation with Bimanual Arms, $^3$Deformable Object Manipulation, $^4$Mobile Manipulation, $^5$Humanoid Manipulation.
}
\label{fig: benchmark}
\end{figure*}

==> figures/4_manipulation_tasks/catergories_basic.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.80\linewidth]{imgs/4_manipulation_tasks/basic.pdf}  
\caption{Method taxonomy for basic manipulation, which provides a unified framework that can be extended to other manipulation tasks.
}
\label{fig: cat_basic}
\end{figure}

==> figures/6_low-level_control/auxiliary_tasks.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{imgs/6_low-level_controller/auxiliary_tasks.pdf}  
\caption{Overview of the taxonomy of methods for learning with auxiliary tasks, highlighting six core components: world models~\cite{mendonca2023structured, lu2024manigaussian}, image or video prediction~\cite{black2024zero, hu2025video}, contrastive learning~\cite{nair2023r3m, ma2025contrastive}, masking reconstruction~\cite{ze2023gnfactor, karamcheti2023language}, text-Grounded goal extraction~\cite{mu2023embodiedgpt, dai2025racer}, and vision-grounded goal extraction~\cite{wang2025discovering, chuang2025look, fang2025keypoint, wi2023calamari, yu2024bikc, shi2023waypoint, mehta2025l2d2, wen2024any, xu2025flow}.
}
\label{fig: learning_with_auxiliary_tasks}
\end{figure*}

==> figures/7_bottlenecks/data_collect.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{imgs/7_bottlenecks/data_collection.pdf}  
\caption{Overview of Data Collection.
DEXUMI~\cite{xu2025dexumi} employs Replica arms, and ARCAP~\cite{chen2024arcap} uses XR Interfaces to represent the data collection methods for Human Teleoperation and Demonstration. DexCap~\cite{wang2024dexcap} stands for Human-in-the-Loop Enhancement, NILS~\cite{blank2025scaling} represents Automatic Data Generation, MimicGen~\cite{mandlekar2023mimicgen} refers to Synthetic Data Generation, and RoboTur represents Crowdsourcing-based Data Collection.
}
\label{fig:data_collection}
\end{figure*}

==> figures/8_applications/case_app.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.85\linewidth]{imgs/8_applications/application.pdf}  
\caption{Overview of robotic manipulation applications across diverse domains. The figure is adapted from representative works in household assistance~\cite{zhao2025bimanual, liu2024forcemimic, sundaresan2023learning, chen2023predicting, kapelyukh2023dall, tang2025functo}, agriculture~\cite{kim2025pepper, li2025enhanced, guri2024hefty}, industry~\cite{adetunji2025vision, domel2017toward, buvs2024deepcraft}, AI4Science~\cite{maroufi2025s3d, he2025capsdt, angers2025roboculture, mishra2025enhancing}, art~\cite{wang2023style, zeulner2025learning, wang2020robocodraw}, and sports~\cite{ma2025learning, wang2025spikepingpong}.
}
\label{fig: case_app}
\end{figure*}

==> sections/1-introduction_2.tex <==
% Robot manipulation is a core problem in embodied intelligence and has been extensively studied in recent years, especially in the context of data-driven learning. It refers to a robot’s ability to perceive, plan, and control its effectors to physically interact with and modify the environment, such as grasping, moving, or using objects. Recent progress has been largely driven by deep learning approaches that leverage large-scale data and expressive function approximators to learn visuomotor policies~\cite{levine2016end, pinto2016supersizing, 10.1109/TRO.2024.3353484} and robotic foundation models~\cite{zitkovich2023rt, kim2025openvla, black2024pi_0}. These advances have been further accelerated by the widespread adoption of imitation learning (IL) and reinforcement learning (RL), which provide principled frameworks for learning manipulation behaviors from demonstrations and interaction~\cite{duan2017one, rajeswaran2018learning}. More recently, large language models and vision–language models have been integrated into IL and RL pipelines to support structured task specification and long-horizon decision making~\cite{zitkovich2023rt, kim2025openvla}. In this survey, we focus on learning-based approaches to robot manipulation and provide a structured analysis of recent methodological progress and emerging trends.

% In recent years, embodied intelligence has attracted increasing attention, driven by advances in computer vision and natural language processing, particularly the emergence of large-scale foundation models. These developments have substantially improved perceptual and semantic representations, enabling robotic systems to operate in less structured environments and to accept high-level task specifications expressed in natural language. Building on this progress, large-scale language and multimodal models~\cite{brown2020language, touvron2023llama, liu2023visual} have begun to reshape robotic manipulation by enhancing generalization, supporting compositional reasoning, and providing a unified interface for perception, decision making, and execution.

This survey aims to develop a structured understanding of robot manipulation by examining the algorithmic principles underlying modern learning-based approaches. Rather than organizing methods by task instances or specific model classes, we structure the literature along two complementary levels: high-level planning and low-level learning-based control. As detailed in Section~\ref{sec: high_level_planner} and Section~\ref{sec: low_level_control}, high-level planners are responsible for structuring and reasoning over task execution, while low-level controllers generate precise and stable actions. Although this abstraction is introduced in the context of basic manipulation, it naturally generalizes across a wide range of manipulation settings, including robotic foundation models that jointly couple high-level reasoning with low-level control.

We position our survey relative to existing literature and clarify its contributions as follows.  
\textbf{First, we adopt a perspective centered on planning and learning abstractions, rather than on individual modeling paradigms.}  
Recent surveys often focus on specific classes of models, such as vision–language–action frameworks~\cite{ma2024survey, zhong2025survey, xiang2025parallels, li2025survey}, diffusion-based policies~\cite{wolf2025diffusion}, or generative approaches~\cite{zhang2025generative}. While these paradigms have driven significant progress, they are typically treated as separate lines of work. In contrast, our perspective situates these methods within a unified abstraction, viewing them as different instantiations of high-level planning mechanisms, low-level learning strategies, or their combinations.

\textbf{Second, we introduce a systematic framework that reorganizes robot manipulation methods through the lens of planning and learning abstractions.}  
At the high level, we broaden the notion of planning (Section~\ref{sec: high_level_planner}) to encompass reasoning over language, code, motion, affordances, and 3D representations. At the low level, we propose a training-paradigm-oriented taxonomy for learning-based control (Section~\ref{sec: low_level_control}), decomposing existing approaches into input modeling, latent representation learning, and policy learning. This abstraction-driven organization facilitates principled comparison across methods and clarifies the relationships between different learning and planning strategies.

\textbf{Finally, building on this structured analysis, we identify emerging research trends and outline four prospective directions for future work.}  
These directions include the development of general-purpose architectures for robotic foundation models, addressing data bottlenecks in robot learning, advancing multimodal perception and interaction with complex objects, and ensuring safety in human–robot coexistence. Together, they highlight the key challenges that must be addressed to enable robust and scalable robotic manipulation in real-world environments.







==> sections/2-background.tex <==
% -------------------- 2-Background --------------------
\section{Background}
\label{sec: background}

\subsection{Manipulation Tasks}


\subsection{Generalization Tasks}
\label{subsec: generalization}

==> sections/2-background_2.tex <==
% -------------------- 2-Background --------------------
\section{Background}
\label{sec: background}

In this section, we first introduce the hardware types currently used for robot manipulation (Section~\ref{subsec: hardeare}). We then present the main categories of control strategies, \textit{i.e.}, non-learning and learning-based approaches (Section~\ref{subsec: control}). Next, we review the robotic models commonly employed in learning-based control (Section~\ref{subsec: robotics_models}). Finally, we discuss the evaluation protocols for learning-based models (Section~\ref{subsec: eval}).

% ---------- 机械臂的硬件类型 ----------
\subsection{Hardware Platforms for Manipulation}
\label{subsec: hardeare}

\input{figures/2_background/hardware}

\noindent \textbf{Single Arm.}
% Commonly used 6-DoF or 7-DoF single-arm robots include the KUKA LBR iiwa\footnote{\url{https://www.kuka.com/}}, Franka Emika Panda~\cite{haddadin2024franka}\footnote{\label{fn:franka}\url{https://franka.de/}}, UR5/UR10\footnote{\url{https://www.universal-robots.com/}}, Kinova Gen3\footnote{\url{https://www.kinovarobotics.com/}}, and xArm6/xArm7\footnote{\url{https://www.ufactory.us/}}. 
% These are typically equipped with 2-DoF grippers such as the Robotiq 2F\footnote{\url{https://robotiq.com/}}.
% There are also some specialized 2-DoF grippers like the DexWrist~\cite{peticco2025dexwrist}.
% Recently, there has been a growing interest in compact robotic arms to facilitate academic research, with platforms such as LeRobot\footnote{\url{https://github.com/huggingface/lerobot}} gaining popularity for their accessibility and ease of use.
Commonly used 6-DoF or 7-DoF single-arm robots include the 
KUKA LBR iiwa\supref{https://www.kuka.com/}{1}, 
Franka Emika Panda~\cite{haddadin2024franka}\supref{https://franka.de/}{2}, 
UR5/UR10\supref{https://www.universal-robots.com/}{3}, 
Kinova Gen3\supref{https://www.kinovarobotics.com/}{4}, 
and xArm6/xArm7\supref{https://www.ufactory.us/}{5}. 
These are typically equipped with 2-DoF grippers such as the 
Robotiq 2F\supref{https://robotiq.com/}{6}. 
There are also some specialized 2-DoF grippers like the DexWrist~\cite{peticco2025dexwrist}. 
Recently, there has been a growing interest in compact robotic arms to facilitate academic research, 
with platforms such as LeRobot\supref{https://github.com/huggingface/lerobot}{7} gaining popularity 
for their accessibility and ease of use.

\noindent \textbf{Bimanual Arms.}
% Common bimanual robotic systems primarily include the Franka Panda Dual Arm\footref{fn:franka}, ALOHA~\cite{fu2025mobile}, and ABB YuMi\footnote{\url{https://new.abb.com/}}.
% These systems enable coordinated dual-arm manipulation, making them suitable for complex tasks such as bi-manual assembly, handovers, and tool usage that require greater dexterity than single-arm setups.
Common bimanual robotic systems primarily include the 
Franka Panda Dual Arm\supref{https://franka.de/}{2}, 
ALOHA~\cite{fu2025mobile}, 
and ABB YuMi\supref{https://new.abb.com/}{8}. 
These systems enable coordinated dual-arm manipulation, making them suitable for complex tasks such as bi-manual assembly, handovers, and tool usage that require greater dexterity than single-arm setups.

\noindent \textbf{Dexterous Hands.}
% Dexterous hands commonly used in robotic manipulation research include the Robotiq Dexterous Gripper, Allegro Hand\footnote{\url{https://www.allegrohand.com/}}, Shadow Hand\footnote{\url{https://shadowrobot.com/}}, D’Kitty and D'Claw~\cite{ahn2020robel}, and others~\cite{shaw2024demonstrating, wan2025rapid}.
% These robotic hands vary in complexity and degrees of freedom, enabling a range of manipulation tasks from simple grasping to highly intricate dexterous operations.
Dexterous hands commonly used in robotic manipulation research include the Robotiq Dexterous Gripper, 
Allegro Hand\supref{https://www.allegrohand.com/}{9}, 
Shadow Hand\supref{https://shadowrobot.com/}{10}, 
D’Kitty and D'Claw~\cite{ahn2020robel}, 
and others~\cite{shaw2024demonstrating, wan2025rapid}.
These robotic hands vary in complexity and degrees of freedom, enabling a range of manipulation tasks from simple grasping to highly intricate dexterous operations.

\noindent \textbf{Soft Hands.}
% Soft hands commonly studied in robotic manipulation research include the RBO Hand 3~\cite{puhlmann2022rbo}, Festo BionicSoft Hand\footnote{\url{https://github.com/Festo-se/festo-bionicsofthand-main}}, and SpiRobs~\cite{wang2025spirobs}. 
% These soft robotic hands leverage compliant materials and innovative actuation mechanisms, such as pneumatic networks and tendon-driven designs, to achieve adaptable and safe grasping of diverse objects.
Soft hands commonly studied in robotic manipulation research include the RBO Hand 3~\cite{puhlmann2022rbo}, 
Festo BionicSoft Hand\supref{https://github.com/Festo-se/festo-bionicsofthand-main}{11}, 
and SpiRobs~\cite{wang2025spirobs}. 
These soft robotic hands leverage compliant materials and innovative actuation mechanisms, such as pneumatic networks and tendon-driven designs, to achieve adaptable and safe grasping of diverse objects.

\noindent \textbf{Mobile Robots.}
% Mobile manipulators, which combine a mobile base with an articulated arm, are widely adopted in research as versatile testbeds for real-world robotics. Representative platforms include the Hello Robot Stretch 3\footnote{\url{https://hello-robot.com/}}, PR2\footnote{\url{https://github.com/pr2}}, and TIAGo\footnote{\url{https://pal-robotics.com/robot/tiago/}}. By integrating mobility with manipulation, these robots can operate in unstructured environments and carry out complex tasks, such as navigation, object fetching, and human–robot interaction.
Mobile manipulators, which combine a mobile base with an articulated arm, are widely adopted in research as versatile testbeds for real-world robotics. Representative platforms include the 
Hello Robot Stretch 3\supref{https://hello-robot.com/}{12}, 
PR2\supref{https://github.com/pr2}{13}, 
and TIAGo\supref{https://pal-robotics.com/robot/tiago/}{14}. 
By integrating mobility with manipulation, these robots can operate in unstructured environments and carry out complex tasks, such as navigation, object fetching, and human–robot interaction.

\noindent \textbf{Quadruped Robots.}
% Representative quadruped robots commonly used in research include the Unitree GO2\footnote{\label{fn:unitree}\url{https://www.unitree.com/}}, B1, and Aliengo, as well as the Boston Dynamics Spot\footnote{\label{fn:boston}\url{https://bostondynamics.com/}}. 
% These platforms offer agile locomotion and can be equipped with robotic arms, enabling them to perform mobile manipulation tasks in unstructured or dynamic environments. 
Representative quadruped robots commonly used in research include the 
Unitree GO2, 
B1, and Aliengo\supref{https://www.unitree.com/}{15}, as well as the 
Boston Dynamics Spot\supref{https://bostondynamics.com/}{16}. 
These platforms offer agile locomotion and can be equipped with robotic arms, enabling them to perform mobile manipulation tasks in unstructured or dynamic environments. 

\noindent \textbf{Humanoid Robots.}
% Representative humanoid robots include Optimus Gen 2\footnote{\url{https://www.tesla.com/en_eu/AI}}, Atlas\footref{fn:boston}, Figure 02 \footnote{\url{https://www.figure.ai/}}, Neo\footnote{\url{https://www.1x.tech/neo}}, and Unitree G1\footref{fn:unitree}. These platforms are designed with bipedal locomotion and human-like morphology, aiming to perform complex tasks in environments originally built for humans.
Representative humanoid robots include 
Optimus Gen 2\supref{https://www.tesla.com/en_eu/AI}{17}, 
Atlas\supref{https://bostondynamics.com/}{16}, 
Figure 02\supref{https://www.figure.ai/}{18}, 
Neo\supref{https://www.1x.tech/neo}{19}, 
and Unitree G1\supref{https://www.unitree.com/}{15}. 
These platforms are designed with bipedal locomotion and human-like morphology, aiming to perform complex tasks in environments originally built for humans.


% ---------- 机械臂如何运动 ----------
\subsection{Non-Learning vs. Learning-based Control Paradigms for Robotic Manipulation}
\label{subsec: control}

Similar to how humans rely on explicit rules (e.g., stopping at red lights) or acquire adaptive skills through repeated practice (e.g., learning to ride a bicycle), robotic control paradigms span from classical, non-learning, model-based planning to learning-based policies. The former offers interpretability and safety in well-defined settings, while the latter provides flexible generalization in complex or uncertain environments.

\subsubsection{Non-Learning-based Control}
Non-learning-based control methods generate robot motions using classical control and optimization techniques without relying on data-driven or learning algorithms. We include them here for completeness, as some studies employ such methods for low-level control within deep learning frameworks. However, they are not the focus of our method section.

\noindent \textbf{Interpolation-based Planning.}
Classical manipulators often employ interpolation-based planning~\cite{duysinx2006introduction, tian2004effective}, where smooth joint-space trajectories are generated, typically offline, by fitting polynomial curves (e.g., cubic splines) between predefined start and goal states. These methods are computationally lightweight and straightforward to deploy, which makes them prevalent in repetitive, well-structured industrial tasks. However, they provide limited adaptability to dynamic or uncertain environments, constraining their applicability in unstructured settings.

\noindent \textbf{Sampling-based Planning.}
Sampling-based planners~\cite{elbanhawi2014sampling, kim2006sampling, schmitt2017optimal, huh2018constrained} construct feasible paths by sampling the configuration space and incrementally building a graph or tree of collision-free states, rather than explicitly computing the free space or solving large global optimizations. Canonical algorithms include Rapidly-exploring Random Trees (RRT)~\cite{kim2006sampling, huh2018constrained} and Probabilistic Roadmaps (PRM)~\cite{schmitt2017optimal}, with asymptotically optimal variants such as RRT*. They scale well to high-dimensional problems, but often yield suboptimal or non-smooth paths that require post-processing.

\noindent \textbf{Optimization-based Planning.}
Optimization-based planners cast manipulation as a constrained optimization problem over trajectories or control sequences, minimizing a task-specific cost while enforcing dynamics, kinematics, and collision-avoidance constraints.

\textit{Offline optimization-based planners} solve the trajectory planning problem prior to execution. They optimize the entire motion path as a batch process, often using gradient-based or stochastic optimization techniques. Representative methods include CHOMP (Covariant Hamiltonian Optimization for Motion Planning)~\cite{zucker2013chomp}, TrajOpt (Trajectory Optimization)~\cite{dai2018improving}, and STOMP (Stochastic Trajectory Optimization for Motion Planning)~\cite{kalakrishnan2011stomp}. These approaches generate smooth, collision-free trajectories, but typically require substantial computation time and do not adapt to unexpected changes during execution.

\textit{Online optimization-based planners}, such as Model Predictive Control (MPC)~\cite{kouvaritakis2016model, bhardwaj2022storm}, repeatedly solve a finite-horizon optimization problem at each control step using the current state as the initial condition. MPC leverages predictive models to anticipate future states and compute optimal control actions in a receding horizon manner. This real-time re-optimization enables adaptation to disturbances and dynamic environments, making MPC a popular choice for robust and precise robot manipulation control.

\subsubsection{Learning-based Control}

The motion of robotic manipulators is typically formulated as a Markov Decision Process (MDP), a formal framework that models sequential decision-making under uncertainty. An MDP is typically formulated as a five-tuple:
\begin{equation}
\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \gamma), 
\end{equation}

\noindent where
\begin{itemize}
  \item $\mathcal{S}$: state space, the set of all possible environment states;
  \item $\mathcal{A}$: action space, the set of all possible actions available to the agent;
  \item $P(s' \mid s, a)$: state transition probability, the probability of moving to state $s'$ when the agent takes action $a$ in state $s$;
  \item $R(s, a)$: reward function, the expected immediate reward obtained by executing action $a$ in state $s$;
  \item $\gamma \in [0, 1]$: discount factor, which trades off short‑term and long‑term rewards.
\end{itemize}

This formulation enables the design and evaluation of control policies that map states to actions with the objective of maximizing expected cumulative rewards. It serves as the foundation for a wide range of learning-based approaches in robot manipulation, including reinforcement learning and imitation learning.

\paragraph{Reinforcement Learning (RL)}
The goal of reinforcement learning is to learn an optimal policy $\pi^{*}: S \rightarrow A$ that maximizes the expected cumulative discounted reward (also known as return)~\cite{han2023survey}:
\begin{equation}
\pi^*=\arg \max _\pi \mathbb{E}\left[\sum_{t=0}^{\infty} \gamma^t R\left(s_t, a_t\right)\right], \quad \text { where } a_t \sim \pi\left(\cdot | s_t\right).
\end{equation}

This formalism provides the theoretical foundation for reinforcement learning and serves as a unifying framework for various algorithms, including Q-learning~\cite{watkins1992q, haarnoja2018composable}, policy gradient methods~\cite{sutton1999policy, peters2006policy}, and actor-critic approaches~\cite{grondman2012survey, haarnoja2018soft}. Unlike supervised learning/behavioral cloning in imitation learning, RL methods can be categorized based on data sources into: Offline RL~\cite{levine2020offline, chen2021decision}, which is trained entirely on pre-collected static datasets; Online RL~\cite{schulman2017proximal, haarnoja2018soft}, which requires continuous interaction with the environment to explore new data distributions; and Offline-to-Online approaches~\cite{lee2022offline, nakamoto2023cal} that combine both paradigms.

\paragraph{Imitation Learning (IL)}
Imitation Learning is typically divided into three categories: Behavior Cloning (BC), Inverse Reinforcement Learning (IRL), and Generative Adversarial Imitation Learning (GAIL).

\noindent \textbf{BC} can be formulated as the MDP framework, which is often defined without an explicitly specified reward function, to model sequential action mapping/generation problems~\cite{torabi2018behavioral, bai2025rethinking}. The concept of rewards is replaced with supervised learning, and the agent learns by mimicking expert actions.
Formally, the state $s_t$ at each timestep consists of visual observations, the robot’s proprioceptive state, and optionally a language instruction.
Let $x_t = (o_t, s_t, l)$ represent the overall state. 
The policy $\pi$ maps a sequence of states to an action.
The optimization process can be formulated as:
\begin{equation}\begin{aligned}\label{func: vanilla_bc}
\pi^* = \operatorname{argmin}_\pi \mathbb{E}_{(s_t) \sim \mathcal{D}_e}\left[\mathcal{L}\left(\pi\left(x_{t}\right), a_t\right)\right],
\end{aligned}\end{equation}
where $\mathcal{D}_e$ is expert trajectory dataset and $a_t$ is action labels. 
In vanilla BC, $\mathcal{L}$ is typically the cross-entropy (CE) for discrete action spaces, and either mean squared error (MSE) or $L_1$ loss for continuous action spaces.

\noindent \textbf{IRL} aims to recover the underlying reward function that explains the expert's behavior, rather than directly mimicking actions. By inferring this reward function, the agent can learn a policy that generalizes better to unseen states and tasks~\cite{arora2021survey, das2021model}. 
Formally, IRL assumes the expert acts optimally with respect to an unknown reward function $R(s,a)$ within the MDP framework. Given expert demonstrations $\mathcal{D}_e$, the goal is to find a reward function $R^*$ such that the expert policy $\pi_e$ maximizes the expected cumulative reward:
\begin{equation}\begin{aligned}\label{func: irl}
R^* = \operatorname{argmax}_{R} \mathbb{E}_{\pi_e}\left[ \sum_{t=0}^\infty \gamma^t R(s_t, a_t) \right] - \mathbb{E}_{\pi}\left[ \sum_{t=0}^\infty \gamma^t R(s_t, a_t) \right],
\end{aligned}\end{equation}
where $\pi$ is the policy induced by the learned reward $R$, and $\gamma \in [0,1)$ is the discount factor.
After estimating $R^*$, the agent solves a reinforcement learning problem to find the optimal policy $\pi^*$ that maximizes the expected return under $R^*$. This two-step process allows the agent to infer intentions behind expert behaviors, potentially improving robustness and adaptability in complex manipulation tasks.

\noindent \textbf{GAIL} frames imitation as distribution matching between the learner’s and the expert’s discounted occupancy measures, thereby bypassing explicit reward modeling. Define the discounted occupancy measure (i.e., the discounted state–action visitation distribution) induced by a policy $\pi$ as
\begin{equation}\label{eq: occupancy}
\rho_{\pi}(s,a) \;=\; (1-\gamma)\sum_{t=0}^{\infty}\gamma^t\,
\Pr\!\left(s_t=s,\, a_t=a \mid \pi, \mathcal{P}\right),
\end{equation}
where $\gamma\in[0,1)$ is the discount factor; $\mathcal{P}$ denotes the MDP transition kernel $P(s'\mid s,a)$; $\Pr(\cdot)$ denotes probability under the trajectory distribution induced by $(\pi,\mathcal{P})$; and the prefactor $(1-\gamma)$ normalizes $\rho_{\pi}$ on the infinite horizon.
Then, a standard adversarial objective is
\begin{equation}\begin{aligned}\label{eq: gail}
\min_{\pi}\;&\max_{D:\mathcal{S}\times\mathcal{A}\to(0,1)}\;
\mathbb{E}_{(s,a)\sim \rho_E}\!\big[\log D(s,a)\big] + \\
&\;\mathbb{E}_{(s,a)\sim \rho_{\pi}}\!\big[\log\!\big(1-D(s,a)\big)\big]
\;-\;\lambda\,\mathcal{H}(\pi).
\end{aligned}\end{equation}
where $D$ is a discriminator over state–action pairs, $\rho_{\pi}$ and $\rho_E$ are the learner’s and expert’s discounted occupancy measures, $\mathcal{H}(\pi)=\mathbb{E}_{(s,a)\sim \rho_{\pi}}[-\log \pi(a\mid s)]$ is the policy entropy, and $\lambda\!\ge\!0$ its weight. At the discriminator optimum, Eq.~\eqref{eq: gail} amounts to minimizing the divergence between $\rho_E$ and $\rho_{\pi}$. In practice, $\pi$ is optimized by policy-gradient updates using a discriminator-induced pseudo-reward, i.e., without relying on an environment-defined task reward.


% ---------- 机器人模型 ----------
\subsection{Robotics Models}
\label{subsec: robotics_models}

% TODO: 重心放回机器人模型，重改

\noindent \textbf{Vision Models.}
To perceive the environment, robotic models typically incorporate vision models to extract informative visual features. Common choices for visual encoders include models trained purely on visual data, such as the ResNet family~\cite{he2016deep}, Vision Transformers (ViT)~\cite{vaswani2017attention}, and self-supervised models like DINO~\cite{zhang2023dino}. For 3D perception tasks, point cloud-based encoders such as PointNet~\cite{qi2017pointnet} and PointTransformer~\cite{zhao2021point} are widely used. Additionally, vision-language pre-trained encoders, such as the image encoders of CLIP~\cite{radford2021learning} or SigLIP~\cite{zhai2023sigmoid}, are employed to obtain semantically enriched representations that align visual observations with linguistic inputs.
Some models leverage additional visual information, including object detection results (such as bounding boxes)~\cite{carion2020end}, visual tracking outputs~\cite{karaev2024cotracker}, to improve perception and support downstream tasks more effectively.

\noindent \textbf{Language Models.}
In recent years, especially since around 2020, language has emerged as a more natural and human-friendly modality, leading to a growing integration of language models into robotics. 
To understand human instructions, language embedding models are commonly employed for extracting textual features, such as BERT~\cite{devlin2019bert} and the language encoder of CLIP. 
With the leap from autoregressive models like GPT-2~\cite{radford2019language} to GPT-3~\cite{brown2020language}, large language models (LLMs) have demonstrated remarkable advances in text understanding and generalization. 
To further leverage the powerful generalization capabilities of LLMs~\cite{touvron2023llama, chowdhery2023palm}, many recent robotic models adopt LLMs as backbones, where textual inputs are processed through tokenization.

\noindent \textbf{Text-conditioned Vision Models and Vision-Language Models (VLMs).}
Robotic models also adopt VLMs such as LLaVA~\cite{liu2023visual}, PaLM-E~\cite{driess2023palm}, and Prism~\cite{karamcheti2024prismatic} as backbones, building upon their architectures to enhance multimodal understanding and control. 
In addition, some works leverage text-conditioned image editing~\cite{brooks2023instructpix2pix} and video generation models~\cite{liu2024sora} to guide action generation through visual imagination and goal specification.

\noindent \textbf{Vision-Action Models and Vision-Language-Action Models.}
Early approaches relied on visual servoing for control~\cite{hutchinson2002tutorial} and gradually incorporated RL or IL methods that map states or images to actions~\cite{jing2023exploring, chi2023diffusion}, giving rise to vision–action (VA) models. Over time, VA architectures have evolved from simple MLPs to more advanced diffusion-based frameworks~\cite{chi2023diffusion}, accompanied by diverse policy designs.
The concept of VLA models was introduced by RT-2~\cite{zitkovich2023rt}. 
In the narrow sense, VLAs refer to models that are fine-tuned from foundation VLMs using robotic trajectory data, enabling them to take human instructions and visual observations as input and directly generate robot actions in an end-to-end manner. 
In a broader sense, any model that takes both visual and language inputs and outputs robot actions through an end-to-end pipeline can be considered a VLA model.


% ---------- Evaluation ----------
\subsection{Evaluation}
\label{subsec: eval}

\noindent \textbf{Evaluation Metrics.}
The most commonly used metric for evaluating robotic performance is the success rate, which measures whether a given task is completed successfully. For long-horizon tasks~\cite{mees2022calvin}, this has been extended to metrics such as average success length, which captures the average number of consecutive tasks completed within a sequence of up to n tasks. Beyond success-based measures, efficiency metrics such as task completion time and action frequency are also employed to assess how quickly and effectively a robot accomplishes a task. In RL settings, return is also widely used as an overall measure of performance.

\noindent \textbf{Model Selection.}
Evaluation strategies vary depending on the experimental setting. A common approach is to evaluate the model every k epochs and select the checkpoint with the highest success rate. Alternatively, for more stable comparisons, one can average the results of the top-n checkpoints from the final training phase. These strategies are frequently employed in single-task settings. In contrast, multi-task settings often adopt a simpler approach by reporting performance at the final training epoch or step, which enables more straightforward and consistent cross-task comparisons. Another widely used strategy is to select the checkpoint that achieves the highest validation performance for subsequent testing.



==> sections/3-benchmarks.tex <==
% -------------------- 3-Tasks, datasets and Benchmarks --------------------
\section{Benchmarks and Datasets}
\label{sec: benchmarks}

\input{figures/3_benchmarks/benchmark}
% \input{sections/3-benchmarks/3.1}
\input{sections/3-benchmarks/3.2}
\input{sections/3-benchmarks/3.3}
\input{sections/3-benchmarks/3.4}
% \input{sections/3-benchmarks/3.5}

% % ---------- Grasping Datasets ----------
% \subsection{Grasping Datasets}
% \label{subsec: grasping_datasets}

% \input{tables/3_benchmarks/grasping_dataset}

% This paper primarily focuses on grasp detection and generation tasks, where the goal is to predict viable grasp configurations directly from sensory inputs. While some works explore grasping as a downstream outcome of broader manipulation objectives, our discussion is centered on methods that explicitly target grasp prediction rather than those that infer grasps from manipulation trajectories or task goals.  
% Data annotations are typically categorized into two formats: rectangle-based and 6-DoF-based. The rectangle-based format labels each grasp using a 5-dimensional grasp rectangle representation, defined by the center position $(x,y)$, the gripper's width and height, and the orientation angle relative to the horizontal axis. In contrast, the 6-DoF format directly annotates the end-effector’s six-degree-of-freedom pose, including position $(x,y,z)$, orientation (e.g., Euler angles or quaternions), and may also include additional information such as the approach direction and a grasp quality score.
% We provide a comprehensive summary of existing grasping datasets in Table~\ref{tab: grasping_datasets} and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_grasping_datasets}.

% Grasping datasets have undergone significant evolution along several dimensions, each contributing to the advancement of the field. 
% First, annotation has shifted from manual labeling to model-based automation, greatly reducing human effort and enabling scalable data generation. 
% Second, the amount of annotated data has increased from small to large-scale datasets, allowing for more robust and data-driven learning. 
% Third, grasp representations have evolved from simple 2D rectangles~\cite{jiang2011efficient, depierre2018jacquard, zhang2022regrad, vuong2024grasp, vuong2024language} to full 6-DoF~\cite{fang2020graspnet, eppner2021acronym, gilles2022metagraspnet, gilles2023metagraspnetv2, nguyen2024graspanything6d} and dexterous hand~\cite{wang2023dexgraspnet, ye2025dex1b} poses, enabling a more accurate modeling of the complexity inherent in real-world grasping.
% Fourth, task settings have expanded from single-object scenarios to multi-object and cluttered environments, offering more realistic and challenging conditions. 
% Lastly, the input modalities have progressed from purely vision-based inputs to language-conditioned instructions, facilitating more flexible and semantically rich manipulation. 
% These changes collectively support the development of generalizable and intelligent grasping systems.



% % ---------- Manipulation Simulator Benchmarks for Robot Arm ----------
% \subsection{Single-Embodiment Manipulation Simulators and Benchmarks}

% \input{tables/3_benchmarks/manipulation_simultor_benchmark}

% Single-embodiment manipulation benchmarks focus on a fixed robotic platform, such as a single-arm manipulator. Based on the categorization of manipulation tasks introduced in Section~\ref{sec: manipulation_tasks}, we provide a comprehensive overview of existing single-embodiment manipulation simulators and benchmarks in Table~\ref{tab: manipulation_simulator_benchmark}, and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_of_single-embodiment_benchmarks}.


% \noindent \textbf{Basic Manipulation Benchmarks.}
% These benchmarks primarily focus on relatively simple tabletop tasks performed using single- or dual-arm manipulators, such as pick-and-place, sorting, pushing, inserting, opening, closing, and pouring.
% Early benchmarks primarily focused on learning trajectories for single-task settings using RL or IL~\cite{yu2020meta, gupta2020relay}. 
% More recent efforts have shifted toward evaluating models under increasingly complex scenarios. 
% These include supporting long-horizon tasks that require robots to complete multi-step operations sequentially~\cite{mees2022calvin, zhang2024vlabench}, incorporating language prompts to guide trajectory generation~\cite{jiang2022vima, zheng2022vlmbench, liu2023libero}, testing generalization under visual distractions~\cite{pumacay2024colosseum, garcia2025towards}, or unseen tasks~\cite{fang2025intention}, proposing fairer evaluation protocols tailored to VLAs~\cite{li2025evaluating, zhang2024vlabench}, and expanding from single-arm to more capable dual-arm manipulation settings~\cite{grotz2024peract2, mu2025robotwin, chen2025robotwin}. 
% Recent benchmarks have also started placing greater emphasis on tactile feedback to enhance policy learning in contact-rich manipulation scenarios~\cite{xu2023efficient, akinola2025tacsl, luu2025manifeel}.

% \noindent \textbf{Dexterous Manipulation Benchmarks.}
% Benchmarks for dexterous manipulation advance both algorithmic methods and hardware platforms. On the algorithmic side, learning frameworks that integrate deep reinforcement learning with demonstrations enable high-dimensional hands to acquire complex skills more efficiently~\cite{rajeswaran2018learning}. On the hardware side, open-source platforms such as TriFinger provide low-cost, reproducible, and community-driven testbeds for dexterity research~\cite{wuthrich2021trifinger}. Together, these benchmarks facilitate systematic evaluation and have accelerated progress in learning-based dexterous manipulation.

% \noindent \textbf{Deformable Object Manipulation Benchmarks.}
% Benchmarks for deformable object manipulation provide structured environments for evaluating robotic systems on tasks involving non-rigid objects such as cloth, rope, and fluids~\cite{huang2021plasticinelab, lin2021softgym}. They are essential for developing algorithms capable of reasoning over high-dimensional, continuous, and underactuated dynamics. By offering reproducible settings, diverse tasks, and well-defined evaluation metrics, these benchmarks enable systematic comparison of methods and foster progress in visuo-tactile perception, planning, and control under complex physical interactions.

% \noindent \textbf{Mobile Manipulation Benchmarks.}
% Mobile manipulation benchmarks evaluate systems that integrate locomotion and manipulation~\cite{ehsani2021manipulathor, yenamandra2023homerobot, li2023behavior}. Typical tasks involve coordinating a mobile base (wheeled or legged) with an onboard manipulator to transport objects, navigate to target locations, and interact within cluttered or spatially extended environments. These benchmarks are critical for studying perception, planning, and control challenges faced by embodied agents operating in dynamic and unstructured settings.

% \noindent \textbf{Quadrupedal Manipulation Benchmarks.}
% Wang et al. introduced ODYSSEY~\cite{wang2025odyssey}, a benchmark and framework for open-world quadruped robots that unifies exploration and manipulation in long-horizon tasks. By integrating vision-language planning with whole-body control, ODYSSEY addresses key challenges in instruction decomposition, locomotion–manipulation coordination, and generalization across diverse open-world scenarios, with validation in both simulation and the real world.

% \noindent \textbf{Humanoid Manipulation Benchmarks.}
% Humanoid manipulation benchmarks evaluate the capabilities of robots with human-like body structures such as arms, hands, and legs~\cite{chernyadev2025bigym, sferrazza2024humanoidbench, jing2025humanoidgen}. Tasks typically involve upper-body operations including grasping, lifting, assembling, or tool use, and may also extend to full-body motions such as bending or balancing. These benchmarks aim to assess dexterity, stability, and coordination in executing human-relevant manipulation tasks across structured and unstructured environments.

% \input{tables/3_benchmarks/cross_embodiment_simulator_benchmark}

% \input{tables/3_benchmarks/trajectory_dataset}


% % ---------- Cross-Embodiment Manipulation Simulator and Benchmarks ----------
% \subsection{Cross-Embodiment Manipulation Simulators and Benchmarks}

% Cross-embodiment manipulation benchmarks support a diverse range of robotic platforms, including single-arm, dual-arm, mobile, quadrupedal, and humanoid robots. These settings are designed to evaluate whether a single model can consistently perform similar tasks across robots with varying morphologies, degrees of freedom, and control constraints.
% Some benchmarks integrate multiple embodiment-specific benchmarks, each with different simulator backends and without a unified interface~\cite{majumdar2023we}. Others consolidate various simulator backends and provide a unified API for consistent interaction~\cite{kumar2023robohive, geng2025roboverse}. Additionally, there are benchmarks that rely on a single simulator backend, within which different embodiments are supported through carefully designed environments~\cite{zhu2020robosuite, mittal2023orbit, nasiriany2024robocasa, genesis2024genesis, tao2025maniskill3, zhang2026agentworld}.
% We present a comprehensive overview of existing cross-embodiment simulators and benchmarks in Table~\ref{tab: cross_embodiment_simulator_benchmark}, and provide detailed descriptions of representative benchmarks in Appendix~\ref{appendix: details_of_cross-embodiment_benchmarks}.



% % ---------- Trajectory Datasets ----------
% \subsection{Trajectory Datasets}

% Trajectory datasets are structured collections of time-ordered data that capture the sequential states, actions, and sensory observations of an agent interacting with an environment. In the context of robotics and embodied AI, these datasets typically include robot joint states, end-effector poses, control inputs, and multimodal observations (e.g., RGB images, depth maps, force-torque readings) collected during the execution of specific tasks.
% In addition to trajectory datasets included in benchmarks, some works focus on building dedicated datasets that vary in scale, quality, and diversity. These datasets range from small collections to large-scale repositories with millions of samples, and from low-fidelity teleoperated data to high-quality expert demonstrations. They also differ in embodiment types, control modes, and data sources such as human teleoperation, scripted agents, or learned policies. Many high-quality datasets include semantic labels, task definitions, and multimodal observations, making them valuable for learning general manipulation policies across tasks and robot types.
% We provide a comprehensive summary of existing trajectory datasets in Table~\ref{tab: trajectory_datasets} and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_of_trajectory_datasets}.


% % ---------- Embodied QA and Affordance Datasets ----------
% \subsection{Embodied QA and Affordance Datasets}

% \input{tables/3_benchmarks/embodied_qa_and_affordance_dataset}

% \input{tables/3_benchmarks/learning_vs_non-learning}

% While EQA and affordance understanding both require visual-semantic and spatial reasoning, EQA emphasizes high-level question answering based on environmental context, whereas affordance understanding targets low-level functional interaction with objects, such as grasping or tool use.
% These datasets empower robotic models with the ability to perceive and understand the physical world, and we categorize their capabilities into three core task types. 
% First, Visual Perception Tasks focus on the static recognition of visual information, enabling robots to identify what an object is, what color or material it has, and what state it is in (e.g., open or closed). This includes object recognition, attribute recognition, object state recognition~\cite{majumdar2024openeqa}, and keypoint selection to determine actionable locations for manipulation~\cite{zhao2025manipbench}. 
% Second, Spatial Reasoning Tasks involve understanding object positions, spatial relationships, and reachability. They encompass 2D/3D object detection~\cite{huang2024manipvqa}, object localization~\cite{majumdar2024openeqa}, and reasoning about spatial relations between the robot and its environment~\cite{chen2025robo2vlm, zhou2025roborefer}, such as determining the relative direction between a gripper and a target object. 
% Finally, Functional and Commonsense Reasoning Tasks address the robot’s understanding of affordances~\cite{gundawar2025pac} and functional uses~\cite{majumdar2024openeqa} of objects—for instance, recognizing that a dish wand is used for cleaning utensils or that a knife should be grasped by its handle. These tasks bridge perception with actionable, context-aware behavior grounded in physical interaction knowledge.
% Table~\ref{tab: embodied_qa_and_affordance_datasets} and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_of_embodied_qa_and_affordance_datasets}.



==> sections/3-benchmarks/3.1.tex <==
% ---------- Grasping Datasets ----------
\subsection{Grasping Datasets}
\label{subsec: grasping_datasets}

\input{tables/3_benchmarks/grasping_dataset}

This paper primarily focuses on grasp detection and generation tasks, where the goal is to predict viable grasp configurations directly from sensory inputs. While some works explore grasping as a downstream outcome of broader manipulation objectives, our discussion is centered on methods that explicitly target grasp prediction rather than those that infer grasps from manipulation trajectories or task goals.  
Data annotations are typically categorized into two formats: rectangle-based and 6-DoF-based. The rectangle-based format labels each grasp using a 5-dimensional grasp rectangle representation, defined by the center position $(x,y)$, the gripper's width and height, and the orientation angle relative to the horizontal axis. In contrast, the 6-DoF format directly annotates the end-effector’s six-degree-of-freedom pose, including position $(x,y,z)$, orientation (e.g., Euler angles or quaternions), and may also include additional information such as the approach direction and a grasp quality score.
We provide a comprehensive summary of existing grasping datasets in Table~\ref{tab: grasping_datasets} and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_grasping_datasets}.

Grasping datasets have undergone significant evolution along several dimensions, each contributing to the advancement of the field. 
First, annotation has shifted from manual labeling to model-based automation, greatly reducing human effort and enabling scalable data generation. 
Second, the amount of annotated data has increased from small to large-scale datasets, allowing for more robust and data-driven learning. 
Third, grasp representations have evolved from simple 2D rectangles~\cite{jiang2011efficient, depierre2018jacquard, zhang2022regrad, vuong2024grasp, vuong2024language} to full 6-DoF~\cite{fang2020graspnet, eppner2021acronym, gilles2022metagraspnet, gilles2023metagraspnetv2, nguyen2024graspanything6d} and dexterous hand~\cite{wang2023dexgraspnet, ye2025dex1b} poses, enabling a more accurate modeling of the complexity inherent in real-world grasping.
Fourth, task settings have expanded from single-object scenarios to multi-object and cluttered environments, offering more realistic and challenging conditions. 
Lastly, the input modalities have progressed from purely vision-based inputs to language-conditioned instructions, facilitating more flexible and semantically rich manipulation. 
These changes collectively support the development of generalizable and intelligent grasping systems.



==> sections/3-benchmarks/3.2.tex <==
\subsection{Single-Embodiment Manipulation Simulators and Benchmarks}

\input{tables/3_benchmarks/manipulation_simultor_benchmark}

Single-embodiment manipulation benchmarks focus on a fixed robotic platform, such as a single-arm manipulator. We provide a comprehensive overview of existing single-embodiment manipulation simulators and benchmarks in Table~\ref{tab: manipulation_simulator_benchmark}.


\noindent \textbf{Basic Manipulation Benchmarks.}
These benchmarks primarily focus on relatively simple tabletop tasks performed using single- or dual-arm manipulators, such as pick-and-place, sorting, pushing, inserting, opening, closing, and pouring.
Early benchmarks primarily focused on learning trajectories for single-task settings using RL or IL~\cite{yu2020meta, gupta2020relay}. 
More recent efforts have shifted toward evaluating models under increasingly complex scenarios. 
These include supporting long-horizon tasks that require robots to complete multi-step operations sequentially~\cite{mees2022calvin, zhang2024vlabench}, incorporating language prompts to guide trajectory generation~\cite{jiang2022vima, zheng2022vlmbench, liu2023libero}, testing generalization under visual distractions~\cite{pumacay2024colosseum, garcia2025towards}, or unseen tasks~\cite{fang2025intention}, proposing fairer evaluation protocols tailored to VLAs~\cite{li2025evaluating, zhang2024vlabench}, and expanding from single-arm to more capable dual-arm manipulation settings~\cite{grotz2024peract2, mu2025robotwin, chen2025robotwin}. 
Recent benchmarks have also started placing greater emphasis on tactile feedback to enhance policy learning in contact-rich manipulation scenarios~\cite{xu2023efficient, akinola2025tacsl, luu2025manifeel}.

\noindent \textbf{Dexterous Manipulation Benchmarks.}
Benchmarks for dexterous manipulation advance both algorithmic methods and hardware platforms. On the algorithmic side, learning frameworks that integrate deep reinforcement learning with demonstrations enable high-dimensional hands to acquire complex skills more efficiently~\cite{rajeswaran2018learning}. On the hardware side, open-source platforms such as TriFinger provide low-cost, reproducible, and community-driven testbeds for dexterity research~\cite{wuthrich2021trifinger}. Together, these benchmarks facilitate systematic evaluation and have accelerated progress in learning-based dexterous manipulation.

\noindent \textbf{Deformable Object Manipulation Benchmarks.}
Benchmarks for deformable object manipulation provide structured environments for evaluating robotic systems on tasks involving non-rigid objects such as cloth, rope, and fluids~\cite{huang2021plasticinelab, lin2021softgym}. They are essential for developing algorithms capable of reasoning over high-dimensional, continuous, and underactuated dynamics. By offering reproducible settings, diverse tasks, and well-defined evaluation metrics, these benchmarks enable systematic comparison of methods and foster progress in visuo-tactile perception, planning, and control under complex physical interactions.

\noindent \textbf{Mobile Manipulation Benchmarks.}
Mobile manipulation benchmarks evaluate systems that integrate locomotion and manipulation~\cite{ehsani2021manipulathor, yenamandra2023homerobot, li2023behavior}. Typical tasks involve coordinating a mobile base (wheeled or legged) with an onboard manipulator to transport objects, navigate to target locations, and interact within cluttered or spatially extended environments. These benchmarks are critical for studying perception, planning, and control challenges faced by embodied agents operating in dynamic and unstructured settings.

\noindent \textbf{Quadrupedal Manipulation Benchmarks.}
Wang et al. introduced ODYSSEY~\cite{wang2025odyssey}, a benchmark and framework for open-world quadruped robots that unifies exploration and manipulation in long-horizon tasks. By integrating vision-language planning with whole-body control, ODYSSEY addresses key challenges in instruction decomposition, locomotion–manipulation coordination, and generalization across diverse open-world scenarios, with validation in both simulation and the real world.

\noindent \textbf{Humanoid Manipulation Benchmarks.}
Humanoid manipulation benchmarks evaluate the capabilities of robots with human-like body structures such as arms, hands, and legs~\cite{chernyadev2025bigym, sferrazza2024humanoidbench, jing2025humanoidgen}. Tasks typically involve upper-body operations including grasping, lifting, assembling, or tool use, and may also extend to full-body motions such as bending or balancing. These benchmarks aim to assess dexterity, stability, and coordination in executing human-relevant manipulation tasks across structured and unstructured environments.

\input{tables/3_benchmarks/cross_embodiment_simulator_benchmark}

\input{tables/3_benchmarks/trajectory_dataset}



==> sections/3-benchmarks/3.3.tex <==
\subsection{Cross-Embodiment Manipulation Simulators and Benchmarks}

Cross-embodiment manipulation benchmarks support a diverse range of robotic platforms, including single-arm, dual-arm, mobile, quadrupedal, and humanoid robots. These settings are designed to evaluate whether a single model can consistently perform similar tasks across robots with varying morphologies, degrees of freedom, and control constraints.
Some benchmarks integrate multiple embodiment-specific benchmarks, each with different simulator backends and without a unified interface~\cite{majumdar2023we}. Others consolidate various simulator backends and provide a unified API for consistent interaction~\cite{kumar2023robohive, geng2025roboverse}. Additionally, there are benchmarks that rely on a single simulator backend, within which different embodiments are supported through carefully designed environments~\cite{zhu2020robosuite, mittal2023orbit, nasiriany2024robocasa, genesis2024genesis, tao2025maniskill3, zhang2026agentworld}.
We present a comprehensive overview of existing cross-embodiment simulators and benchmarks in Table~\ref{tab: cross_embodiment_simulator_benchmark}.
% , and provide detailed descriptions of representative benchmarks in Appendix~\ref{appendix: details_of_cross-embodiment_benchmarks}.




==> sections/3-benchmarks/3.4.tex <==
\subsection{Trajectory Datasets}

Trajectory datasets are structured collections of time-ordered data that capture the sequential states, actions, and sensory observations of an agent interacting with an environment. In the context of robotics and embodied AI, these datasets typically include robot joint states, end-effector poses, control inputs, and multimodal observations (e.g., RGB images, depth maps, force-torque readings) collected during the execution of specific tasks.
In addition to trajectory datasets included in benchmarks, some works focus on building dedicated datasets that vary in scale, quality, and diversity. These datasets range from small collections to large-scale repositories with millions of samples, and from low-fidelity teleoperated data to high-quality expert demonstrations. They also differ in embodiment types, control modes, and data sources such as human teleoperation, scripted agents, or learned policies. Many high-quality datasets include semantic labels, task definitions, and multimodal observations, making them valuable for learning general manipulation policies across tasks and robot types.
We provide a comprehensive summary of existing trajectory datasets in Table~\ref{tab: trajectory_datasets}.
% and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_of_trajectory_datasets}.



==> sections/3-benchmarks/3.5.tex <==
\subsection{Embodied QA and Affordance Datasets}

\input{tables/3_benchmarks/embodied_qa_and_affordance_dataset}

\input{tables/3_benchmarks/learning_vs_non-learning}

While EQA and affordance understanding both require visual-semantic and spatial reasoning, EQA emphasizes high-level question answering based on environmental context, whereas affordance understanding targets low-level functional interaction with objects, such as grasping or tool use.
These datasets empower robotic models with the ability to perceive and understand the physical world, and we categorize their capabilities into three core task types. 
First, Visual Perception Tasks focus on the static recognition of visual information, enabling robots to identify what an object is, what color or material it has, and what state it is in (e.g., open or closed). This includes object recognition, attribute recognition, object state recognition~\cite{majumdar2024openeqa}, and keypoint selection to determine actionable locations for manipulation~\cite{zhao2025manipbench}. 
Second, Spatial Reasoning Tasks involve understanding object positions, spatial relationships, and reachability. They encompass 2D/3D object detection~\cite{huang2024manipvqa}, object localization~\cite{majumdar2024openeqa}, and reasoning about spatial relations between the robot and its environment~\cite{chen2025robo2vlm, zhou2025roborefer}, such as determining the relative direction between a gripper and a target object. 
Finally, Functional and Commonsense Reasoning Tasks address the robot’s understanding of affordances~\cite{gundawar2025pac} and functional uses~\cite{majumdar2024openeqa} of objects—for instance, recognizing that a dish wand is used for cleaning utensils or that a knife should be grasped by its handle. These tasks bridge perception with actionable, context-aware behavior grounded in physical interaction knowledge.
Table~\ref{tab: embodied_qa_and_affordance_datasets} and offer detailed descriptions of representative datasets in Appendix~\ref{appendix: details_of_embodied_qa_and_affordance_datasets}.



==> sections/4-manipulation_tasks.tex <==
% 以任务分类
\section{Manipulation Tasks}
\label{sec: manipulation_tasks}

Early grasping methods primarily focused on identifying stable grasp configurations through geometric analysis, force closure conditions, or task-specific heuristics. Candidate grasp poses were analytically generated from object geometry, contact normals, or predefined grasp templates, and then executed using inverse kinematics (IK) and motion planning. Building on such established grasps, early approaches to dexterous, deformable, mobile, quadrupedal, and humanoid manipulation typically assumed a known target pose or a task-specific goal. The emphasis was on optimizing motion trajectories or control commands to achieve these goals under physical and kinematic constraints, rather than learning end-to-end action generation from raw sensory input as in modern RL or IL methods. The comparison is summarized in Table~\ref{tab: method_comparison}.

Among these, basic manipulation is by far the most extensively studied, supported by a rich body of literature that enables fine-grained categorization of methods. We therefore dedicate Sections~\ref{sec: high_level_planner} and \ref{sec: low_level_control} to a detailed discussion of high-level planners and low-level learning-based control in the context of basic manipulation, while for other task categories we summarize representative methods within their respective subsections. Beyond the tasks covered in this survey, niche domains such as aerial manipulation~\cite{khamseh2018aerial, ruggiero2018aerial, suarez2020benchmarks} and underwater manipulation~\cite{lane1997amadeus, morgan2022autonomous, liu2025self} will be incorporated in future updates.

\input{figures/4_manipulation_tasks/grasp_methods}

% Grasping
\subsection{Grasping}

In the narrow sense considered in this work, grasping specifically refers to the tasks of grasp detection and grasp generation. These tasks involve identifying feasible grasp configurations from sensor inputs such as images or point clouds, allowing robotic end-effectors to securely pick up objects. The primary focus is on predicting the position and orientation of the gripper to ensure stable and reliable grasps, even in the presence of diverse object shapes, varying poses, and cluttered environments.

\noindent \textbf{Non-Learning-based Grasp.} 
Early methods generate grasp poses by explicitly analyzing object geometry~\cite{jones1990planning}, performing contact-driven force analysis~\cite{miller2004graspit}, or applying task-specific rules~\cite{stoytchev2005behavior}, in combination with the gripper model. 
However, due to their limited generalization ability in handling complex shapes, occlusions, and unseen objects, these approaches have gradually been replaced by data-driven, learning-based methods, as discussed below. The taxonomy of learning-based grasping approaches is illustrated in Figure~\ref{fig: grasp_methods}.

\noindent \textbf{Rectangle-based Grasp.}
Grasping rectangles were first introduced by Jiang et al.~\cite{jiang2011efficient}. While they are visually similar to bounding boxes, their representational semantics are fundamentally different. A grasping rectangle is defined as a 5-dimensional representation, as previously described in Section~\ref{subsec: grasping_datasets}. 
Subsequent methods have progressively incorporated deep learning techniques, ranging from basic convolutional neural networks (CNNs)~\cite{redmon2015real, kumra2017robotic, morrison2018closing} to more advanced architectures such as ResNet~\cite{carion2020end}, GR-ConvNet~\cite{kumra2020grconvnet} and Transformer~\cite{wang2022transformer}, and further to CLIP-based models that integrate textual information through feature fusion methods~\cite{nguyen2024lightweight}. More recently, diffusion models have also been employed~\cite{vuong2024language}. Over time, the models have evolved from simple to complex, and the modalities have shifted from unimodal to increasingly multimodal.

\noindent \textbf{6-DoF Grasp.}
Two-dimensional rectangle-based representations, which typically assume parallel-jaw grippers executing top-down grasps, are limited to 2 or 3 degrees of freedom (DoF). This restricts the gripper’s orientation and reduces applicability in unstructured or complex environments. To address these limitations, researchers have proposed 6-DoF grasp representations~\cite{yan2018learning} that define a grasp as a complete 6-dimensional pose in 3D space. This formulation enables the robot to grasp objects from arbitrary orientations, significantly improving flexibility and robustness. The 6-DoF representation is especially beneficial in cluttered scenes, non-planar object poses, and scenarios involving complex geometries.

Apart from a few early 2D-based approaches~\cite{zhai2023monograspnet}, the majority of recent methods adopt 3D representations. In particular, methods based on point cloud inputs have explored a wide range of architectures, ranging from mapping convolutional networks~\cite{fang2023anygrasp} and transformer-based models~\cite{fan2025miscgrasp}, to generative autoencoders~\cite{yan2018learning}, variational autoencoders~\cite{mousavian20196dof, iwase2025zerograsp}, and UNet-style frameworks~\cite{xie2025rethinking}. 
To improve efficiency, various methods have been proposed, including applying instance segmentation or heatmap to focus on task-relevant manipulation regions~\cite{murali20206, chen2023efficient}, reducing the grasp search space by representing grasp poses with contact points on the object surface~\cite{sundermeyer2021contact}, incorporating graph neural networks for geometric reasoning on point cloud data~\cite{moghadam2023grasp}, and adopting an economic supervision paradigm that selects key annotations and leverages focal representation to reduce training cost and improve performance~\cite{wu2024economic}.
Some works further address structural distortions commonly found in real-world point cloud data by introducing completion or denoising modules to convert the input into a clean and consistent style~\cite{cheng2025pcf, cai2025real}. 
Several methods also address the SE(3)-equivariance problem~\cite{lim2025equigraspflow, hu2025orbitgrasp} by modeling grasp generation as a continuous normalizing flow over SE(3) with equivariant vector fields, or by predicting per-point grasp quality over the orientation sphere using spherical harmonic basis functions.
Meanwhile, several methods also leverage 3D representations such as SDF~\cite{breyer2021volumetric, song2025implicit, jauhri2024learning}, NeRF~\cite{rashid2023language, dai2023graspnerf}, and 3DGS~\cite{zheng2024gaussiangrasper, ji2025graspsplats, yu2024sparsegrasp} to extract geometric features or to sample grasp points for downstream prediction.

\noindent \textbf{Language-Driven Grasp.}
In recent years, language-driven grasping has gained increasing attention, aiming to achieve object-specific and instruction-guided manipulation. Existing approaches can be broadly categorized into three groups. The first adopts multimodal feature fusion~\cite{xu2023joint, nguyen2024language}, where textual and visual modalities are jointly encoded, often via cross-attention mechanisms. The second leverages existing grasp models to generate large numbers of grasp candidates, followed by ranking or scoring with LLMs or VLMs to select the most confident grasps. For instance, LLMs can generate task-specific descriptions~\cite{tang2023graspgpt}, while VLMs are used for visual grounding to compute grasp confidence scores~\cite{qian2025thinkgrasp, tang2025affordgrasp}. Representative methods include VL-Grasp, which employs VLMs to attend to the target object and generate grasps~\cite{lu2023vl}; OWG, which leverages VLM-based semantic priors for planning under occlusion~\cite{tziafas2025towards}; and Reasoning-Grasping, which integrates visual-linguistic inference for improved object-level understanding~\cite{jin2025reasoning}. Other efforts adapt MLLMs for environment-aware error correction~\cite{luo2025roboreflect}, or learn object-centric attributes to enable rapid grasp adaptation across tasks~\cite{yang2024attribute}. Affordance-driven approaches also ground grasp generation in language and vision cues~\cite{dong2025rtagrasp, song2025learning, deshpande2025graspmolmo}. The third line of work directly fine-tunes MLLMs on grasp foundation models with large-scale grasp datasets~\cite{xu2024rt}.

\noindent \textbf{Challenges.}
Firstly, the aforementioned grasp detection and generation methods were originally designed for 2-DoF parallel-jaw grippers. 
However, with the increasing use of dexterous hands, research has shifted toward dexterous grasping, which requires more complex annotations such as hand joint angles and contact force maps. To handle the high dimensionality of this task, various generative approaches—including diffusion-based models—have been proposed~\cite{xu2024dexterous, weng2024dexdiffuser, wei2024grasp}. Some approaches represent grasp configurations via contact points or maps~\cite{li2023gendexgrasp}, or leverage interaction-based representations like D(R, O)~\cite{wei2024d} to infer grasps from geometric relationships.
Second, traditional grasping strategies typically rely on a single end-effector (e.g., suction or parallel grippers), which limits adaptability to diverse object geometries. To address this, several works have explored bimanual grasping using dual-arm or dual-gripper configurations~\cite{mahler2019learning, yamada2025combo}.
Lastly, grasping transparent objects also remains a significant challenge, as depth sensors often fail to detect or localize such materials accurately. Recent efforts address this limitation by incorporating alternative modalities, such as LiDAR~\cite{deng2025fusegrasp} or 3D reconstruction~\cite{duisterhof2024residual, shi2024asgrasp, kim2025t}, to infer the geometry of transparent or reflective objects.


% Basic Manipulation
\subsection{Basic Manipulation}
Basic manipulation refers to relatively simple tabletop tasks performed by single- or dual-arm manipulators, such as pick-and-place, sorting, pushing, inserting, opening, closing, and pouring. 
Most current research remains focused on this category, as illustrated in Figure~\ref{fig: cat_basic} and further discussed in Sections~\ref{sec: high_level_planner}--\ref{sec: low_level_control}, where the majority of methods and benchmarks are developed around object-centric interactions in structured environments.
While these sections classify approaches within the scope of basic manipulation, the proposed taxonomy is general in nature and can be readily extended to other categories of manipulation tasks.


\input{tables/4_manipulation_tasks/manipulation_tasks}

\input{figures/4_manipulation_tasks/case_dexterous}


% Dexterous Manipulation
\subsection{Dexterous Manipulation}
Dexterous manipulation refers to the capability of robotic systems equipped with multi-fingered or anthropomorphic hands to achieve precise and coordinated object control through complex contact interactions. It involves in-hand reorientation, fine force modulation, and multi-point contact, enabling actions such as twisting, grasping, and rotating, as illustrated in Figure~\ref{fig: case_dex}. This capability is critical for tasks requiring high precision and adaptability, such as tool use, assembly, and manipulation of small or irregular objects. Human hand models typically include 20–25 DoF, with each finger modeled by 4 DoF, the thumb by 4–5 DoF, and additional DoF from the palm and wrist for enhanced realism~\cite{welte2025interactive}.

\noindent \textbf{Non-Learning-based Methods.}
Early work on dexterous manipulation predominantly employed non-learning approaches, including optimization- and control-based techniques such as heuristic search and constrained optimization~\cite{bai2014dexterous}. These methods typically assume access to known dynamics and object models, and focus on trajectory planning under physical constraints.

\noindent \textbf{Learning-based Methods.} 
With the advent of RL, both model-based and model-free paradigms have been applied to dexterous manipulation. Model-based methods such as PDDM~\cite{nagabandi2020deep} exploit learned dynamics for efficient planning and control, while model-free approaches directly optimize policies from interaction~\cite{rajeswaran2018learning}, sometimes enhanced with few-shot imitation to accelerate learning on real hands~\cite{zhu2019dexterous}. More recently, human-in-the-loop frameworks such as HIL-SERL~\cite{luo2025precise} combine demonstrations, online corrections, and reinforcement learning to achieve sample-efficient training of precise and dexterous skills directly on real robots.
IL has gained attention for its data efficiency, exemplified by DexMV~\cite{qin2022dexmv}, which employs kinematic retargeting from human videos to robot hands. Extensions incorporate auxiliary tasks such as contact prediction~\cite{liang2025dexhanddiff, fu2025cordvip} and inverse dynamics modeling~\cite{radosavovic2021state}, enabling better generalization and action consistency.
Hybrid IL–RL approaches aim to combine these strengths, typically using IL for policy initialization followed by RL refinement~\cite{kumar2016learning, arunachalam2023dexterous}. Integration can vary: DexMV applies IL first and fine-tunes with RL, whereas ViViDex~\cite{chen2025vividex} performs RL in a privileged state space before distilling policies via IL.

Recent advances in VLA models further expand generalization. DexGraspVLA~\cite{zhong2025dexgraspvla} integrates semantic reasoning with diffusion-based policies for grasping in cluttered scenes, while OFA~\cite{li2025object}, LBM~\cite{barreiros2025careful}, and Being-H0~\cite{luo2025being} leverage multimodal prompts and human videos to generate dexterous motions and follow language instructions.

Human guidance provides another supervision source: Chen et al.~\cite{chen2025object} use object and wrist trajectories from videos to guide RL, and Mandi et al.~\cite{mandi2025dexmachina} introduce functional retargeting to transition from demonstrations to autonomous control. Affordance reasoning further supports grasp-specific strategies~\cite{kannan2023deft, agarwal2023dexterous}, guiding object selection under semantic constraints.
Finally, recent works emphasize robustness and autonomy. Task decomposition reduces complexity by structuring subtasks~\cite{dasari2023learning}, while recovery mechanisms such as REBOOT~\cite{hu2023reboot} introduce IL-trained reset policies to handle failures in long-horizon settings.

\noindent \textbf{Challenges.} 
Beyond high-dimensional control and contact dynamics, dexterous manipulation faces broader challenges.
First, many real-world tasks are long-horizon and compositional, requiring sequential execution of fine-grained skills. Chen et al.~\cite{chen2023sequential} address this by decomposing tasks into discrete skills trained with RL and linking them via a high-level policy.
Second, sim-to-real transfer remains a bottleneck due to discrepancies in perception, dynamics, and actuation. CyberDemo~\cite{wang2024cyberdemo} mitigates this through data augmentation, improving robustness under domain shift.
Third, accurate perception is difficult in cluttered or partially observed scenes, where occlusion hampers object tracking. DexPoint~\cite{qin2023dexpoint} leverages point cloud completion to recover missing geometry and enhance spatial awareness.


\input{figures/4_manipulation_tasks/case_soft}

% Soft Robotics Manipulation
\subsection{Soft Robotics Manipulation}
Soft manipulators, built with compliant materials or structures, are well-suited for human–robot collaboration, operation in uncertain environments, and safe, adaptive grasping, as illustrated in Figure~\ref{fig: case_soft}. They overcome the limitations of rigid manipulators when handling delicate or deformable objects~\cite{chen2022review}. To this end, a wide range of designs have been developed to support diverse applications~\cite{ansari2017towards, thuruthel2018stable, puhlmann2022rbo, liu2022touchless, wang2025spirobs}.

\noindent \textbf{Non-Learning-based Methods.}
For soft manipulator control, analytical kinematic models based on the constant-curvature assumption map shape parameters to end-effector poses via virtual rigid-link chains and Denavit–Hartenberg transformations~\cite{jones2006kinematics}. Similarly, three-dimensional continuum manipulators can be approximated as rigid-jointed robots, with computed-torque control achieving closed-loop dynamics~\cite{wang2020dynamic}. Other approaches employ model predictive control with Koopman operators~\cite{bruder2019modeling, lv2025multi}, or rely on accurate Lagrangian models combined with adaptive dynamic sliding mode control to enhance robustness~\cite{kazemipour2022adaptive}. Hybrid schemes also integrate learning into non-learning frameworks: forward dynamics can be approximated with machine learning and combined with trajectory optimization for open-loop control~\cite{thuruthel2017learning}, while feedback-driven strategies exploit learned models to stabilize and restore system states~\cite{thuruthel2018stable}.

\textbf{Learning-based Methods.} 
RL and IL have been widely applied to soft manipulator control. 
Model-free RL avoids explicit physical modeling by training policies in simulation for closed-loop endpoint control~\cite{you2017model}. Forward dynamics learned with recurrent networks can be integrated into trajectory optimization to generate samples and train predictive controllers~\cite{thuruthel2018model}, while LSTM-based dynamics models enable feedback policy learning~\cite{centurelli2022closed}. Domain randomization combined with incremental offline training has improved task-space accuracy and adaptability~\cite{li2022towards}, and wavelet-based dynamics approximations paired with LSTM and TD3 controllers further enhance generalization under variability~\cite{zhou2024cable}.
IL approaches include Soft DAgger~\cite{nazeer2023soft}, which employs dynamic behavior mapping for online expert-like action generation, and KineSoft~\cite{yoo2025kinesoft}, which integrates kinesthetic teaching with diffusion-based policy learning. Hybrid methods also emerge, such as SS-ILKC~\cite{meng2025sensor}, which combines multi-objective RL with adversarial IL to learn goal-directed control strategies in sensor space, supported by sim-to-real pre-calibration for zero-shot transfer.

\noindent \textbf{Challenges.} 
Soft-hand-based manipulation faces several challenges, including modeling highly nonlinear and underactuated dynamics, achieving precise force and pose control with deformable or fragile objects, ensuring robustness under environmental uncertainty and sensor noise, and lowering the cost and complexity of data collection and teleoperation for policy training. To improve sample efficiency, Soft DAgger~\cite{nazeer2023soft} enables online imitation learning from limited demonstrations through dynamic behavior mapping. To reduce hardware complexity in teleoperation, Liu et al.~\cite{liu2022touchless} propose a flexible bimodal sensory interface that combines vision-based perception with wearable sensors, enabling intuitive and low-cost control without bulky equipment.


\input{figures/4_manipulation_tasks/case_deformable}


% Deformable Object Manipulation
\subsection{Deformable Object Manipulation}
Deformable object manipulation (DOM) requires robots to perceive and control non-rigid objects whose shapes vary under applied forces. Unlike rigid-body manipulation, it demands reasoning over high-dimensional, continuous state spaces, coping with uncertain deformation dynamics, and interpreting subtle visual or tactile cues. As illustrated in Figure~\ref{fig: case_deformable}, tasks such as cloth folding, rope and cable tying, and food handling involve diverse deformations—including tension, compression, and bending—making DOM a complex yet crucial challenge in robotic manipulation~\cite{sanchez2018robotic, blanco2024t, gu2023survey}.

\noindent \textbf{Non-Learning-based Methods.}
Traditional approaches to DOM, such as path planning~\cite{saha2007manipulation} and model-based control~\cite{luque2024model}, often rely on simplified physical models or analytical solutions. However, these methods typically struggle with generalization and real-time adaptability in complex environments, leading to a shift toward data-driven techniques such as RL, IL, and hybrid learning-control frameworks.

\noindent \textbf{Learning-based Methods.}
Jan et al.~\cite{matas2018sim} propose a deep RL method based on a modified DDPG algorithm that learns from visual and robot state inputs and achieves zero-shot sim-to-real transfer via domain randomization. In contrast, IL methods directly exploit demonstrations: DexDeform~\cite{li2023dexdeform} extracts latent skills from human demonstrations and fine-tunes them with limited robot data, DefGoalNet~\cite{thach2024defgoalnet} predicts goal configurations from few-shot demonstrations conditioned on state and context, and MPD~\cite{scheikl2024movement} generates movement primitives with diffusion models. To combine both paradigms, DMfD~\cite{salhotra2022learning} incorporates expert data into RL through advantage-weighted BC loss, expert-initialized replay buffers, and reset-to-state initialization, achieving stable and efficient policy optimization.

Beyond learning paradigms, DOM has explored diverse strategies spanning geometric modeling, affordance prediction, and structure-aware perception. DeformGS~\cite{duisterhof2024deformgs} represents deformable objects with canonical Gaussians and learns a time-conditioned deformation field for temporally consistent 3D pose tracking. Affordance-based approaches include DeformerNet~\cite{hu20193}, which predicts end-effector displacements from partial point clouds, Foresightful Affordance~\cite{wu2023learning}, which integrates dense per-pixel affordances with long-horizon value estimation, and APS-Net~\cite{luan2025learning}, which ranks standardized folding and flattening trajectories guided by affordance heatmaps. Language-conditioned affordance prediction has also been explored~\cite{deng2024learning}.
Finally, estimating object-specific physical properties has emerged as a complementary direction~\cite{caporali2024deformable, kuroki2024gendom}. GenDOM~\cite{kuroki2024gendom} learns a parameter-conditioned policy and leverages a single human demonstration with differentiable simulation to infer unseen object properties, enabling generalization to novel deformable instances.

\noindent \textbf{Challenges.}
Deformable objects lack a fixed pose, and key deformation regions are often occluded during manipulation. To improve visibility and perception, recent work jointly optimizes camera and manipulator motion, guided by structure-of-interest cues~\cite{weng2024interactive}. Deformation dynamics also exhibit delayed responses, complicating real-time control; this is addressed by encoding states into latent spaces and predicting their dynamics. For example, DeformNet~\cite{li2024deformnet} encodes object geometry with PointNet and a conditional NeRF, and models temporal evolution with a recurrent state-space model for latent-level MPC. An even greater challenge is modeling topological changes. DoughNet~\cite{bauer2024doughnet} extends latent-space modeling to jointly capture geometric and topological variations from point clouds, enabling long-horizon planning with CEM for tool selection and manipulation.


\input{figures/4_manipulation_tasks/case_mobile}


% Mobile Manipulation
\subsection{Mobile Manipulation}
Mobile manipulation is a robotic paradigm that combines navigation and manipulation capabilities within a single system. It allows robots to physically interact with objects beyond a fixed workspace by actively navigating the environment. This integration poses significant challenges in perception, planning, and control, as it requires coordinating whole-body motion, handling long-horizon tasks, and dealing with dynamic, partially observable scenes. 
Several studies have focused on designing robots specifically for mobile manipulation~\cite{holmberg2000development, hebert2015mobile, fu2025mobile}.
As illustrated in Figure~\ref{fig: case_mobile}, mobile manipulation is critical for real-world applications such as household assistance, warehouse automation, and service robotics~\cite{thakar2023survey}.

\noindent \textbf{Non-Learning-based Methods.}
Traditionally, mobile manipulation is decomposed into two separate problems: navigation and manipulation. Navigation is typically handled by classic path planners, such as grid-based methods (e.g., Dijkstra) and sampling-based planners (e.g., RRT). Manipulation is often addressed using grasp models, motion primitives, or trajectory planning based on point clouds.
Some control methods perform joint optimization of navigation and manipulation. For example, Berenson et al.~\cite{berenson2008optimization} optimize full-body configurations and grasp poses simultaneously, then plan motions via sampling. Chitta et al.~\cite{chitta2012mobile} coordinate base-arm planning with ROS-based navigation and point cloud grasping. Others embed manipulation goals directly into MPC cost functions~\cite{pankert2020perceptive}.

\noindent \textbf{Learning-based Methods.}
These methods have emerged to learn policies for whole-body control. 
For RL, Wang et al.~\cite{wang2020learning} use RGB-D inputs to estimate object pose and train a policy that jointly predicts base velocity, arm trajectories, and gripper actions. HarmonicMM~\cite{yang2024harmonic} extends this by integrating visual and pose information into a unified RL framework, while Wu et al.~\cite{wu2020spatial} propose spatial Q-value learning at the map level for navigation guidance. To improve reward signals, Honerkamp et al.~\cite{honerkamp2021learning} design dense rewards based on end-effector reachability, and Causal MoMa~\cite{hu2023causal} introduces causality-aware modeling of control–reward relations to stabilize policy optimization.
For IL, MOMA-Force~\cite{yang2023moma} learns motion and force policies from visual-force demonstrations, while HoMeR~\cite{sundaresan2025homer} decomposes tasks into global keypose prediction and local refinement to map end-effector targets to whole-body actions. Wang et al.~\cite{zhicheng2025object} leverage SAM2-based perception for object-centric IL, and Skill Transformer~\cite{huang2023skill} treats manipulation as a skill prediction problem, learning both skill categories and corresponding low-level actions.
Hybrid methods combine IL with RL to enhance generalization. For example, Xiong et al.~\cite{xiong2024adaptive} initialize policies via behavior cloning and refine them through online RL to handle unseen articulated objects.

Beyond learning paradigms, recent work integrates high-level reasoning and multimodal representations. VLA-based methods such as MoManipVLA~\cite{wu2025momanipvla} process multimodal instructions to predict end-effector waypoints while delegating base motion to a trajectory optimizer. LLM-driven frameworks, including MoMa-LLM~\cite{honerkamp2024language} and SayPlan~\cite{rana2023sayplan}, combine open-vocabulary language, scene graphs, and reasoning for object search and high-level task planning. Complementary efforts in \textit{3D scene modeling} guide manipulation through active perception: ActPerMoMa~\cite{jauhri2024active} optimizes viewpoint selection and grasp reachability via incremental TSDF mapping, while TaMMa~\cite{hou2025tamma} employs sparse Gaussian localization and depth completion to generate accurate target poses.

\noindent \textbf{Challenges.}
In addition to perception–action coordination, dynamic obstacles, and long-horizon decision-making, mobile manipulation faces several additional challenges.
A first challenge is enabling effective human–robot collaboration. Ciocarlie et al.~\cite{ciocarlie2012mobile} developed an assistive system that combines user interfaces, shared control, and autonomy to transform a PR2 robot into an in-home assistant. Extending this line of work, Robi Butler~\cite{xiao2025robi} introduces a closed-loop household control framework that supports multimodal interaction, where high-level planners such as LLMs and VLMs enable natural language and gesture-based commands for intuitive and remote collaboration.
A second challenge is real-time manipulation during navigation, where robots must coordinate mobility and manipulation under environmental constraints. Whole-body motion control frameworks~\cite{haviland2022holistic, burgess2023architecture} address this problem by enabling reactive planning and execution for on-the-move manipulation.


\input{figures/4_manipulation_tasks/case_quadrupedal}


% Quadrupedal Manipulation
\subsection{Quadrupedal Manipulation}
Quadrupedal manipulation is an emerging paradigm that combines the agile mobility of quadruped robots with the ability to physically interact with objects. Unlike traditional manipulators or mobile bases, quadrupeds can traverse complex and unstructured terrains while maintaining dynamic stability, making them particularly suitable for applications such as search and rescue, field robotics, and autonomous exploration. Representative tasks are illustrated in Figure~\ref{fig: case_mobile}.
Manipulation can be realized through several embodiments: whole-body loco-manipulation~\cite{jeon2023learning, huang2024hilma, ouyang2024long, ding2024quar, song2024germ, zhao2025more}; leg-as-manipulator designs that repurpose one or more legs for interaction~\cite{cheng2023legs, arm2024pedipulate, he2024learning}; back-mounted arms~\cite{wolfslag2020optimisation, fu2023deep, arcari2023bayesian, ferrolho2023roloma, yokoyama2023asc, qiu2024learning, mendonca2025continuously, zhang2024gamma, liu2025visual, jiang2024learning, wang2025quadwbg, pan2025roboduet, zhi2025learning, hou2025efficient}; and grippers integrated into front legs for simultaneous locomotion and manipulation~\cite{lin2024locoman}. Each embodiment introduces unique challenges in whole-body coordination, dynamic control, and perception-driven planning.

\noindent \textbf{Non-Learning-based Methods.}
Recent advances in quadrupedal manipulation have explored diverse control strategies, ranging from model-based optimization to learning-based approaches. Optimization-based methods provide interpretable and physically grounded control with strong task generalization. For example, Arcari et al.~\cite{arcari2023bayesian} combine MPC with Bayesian multi-task error learning for real-time dynamics adaptation. Wolfslag et al.~\cite{wolfslag2020optimisation} incorporate SUF stability metrics and contact constraints into a quadratic programming framework for robust, support-leg-aware planning, a concept further extended by RoLoMa~\cite{ferrolho2023roloma} to improve trajectory robustness. LocoMan~\cite{lin2024locoman} demonstrates a hardware–control co-design approach, equipping quadrupeds with lightweight front-leg manipulators and employing unified WBC to achieve agile locomotion and precise manipulation.

\noindent \textbf{Learning-based Methods.}
In the realm of RL, recent research has focused on developing structured and informative control representations. Jeon et al.~\cite{jeon2023learning} introduce a hierarchical RL framework that encodes interaction experience, robot morphology, and action history into latent representations to facilitate effective policy learning. Fu et al.~\cite{fu2023deep} decouple leg and arm rewards in the policy gradient formulation to enhance coordination between locomotion and manipulation, while Zhi et al.~\cite{zhi2025learning} present a unified force–position controller that estimates forces from perception instead of sensors. Hou et al.~\cite{hou2025efficient} incorporate explicit arm kinematics and feasibility-based rewards to promote physically plausible behaviors. Two-stage training schemes have also been explored: RoboDuet~\cite{pan2025roboduet} sequentially trains locomotion and arm policies with reward adaptation for coordination. GAMMA~\cite{zhang2024gamma} improves grasp precision by conditioning policies on grasp poses, while Wang et al.~\cite{wang2025quadwbg} propose GORM, a metric for grasp reachability under varying base poses, guiding base movements for optimal grasping. Teacher–student frameworks have further advanced base–arm coordination, as in VBC~\cite{liu2025visual} and Jiang et al.~\cite{jiang2024learning}, where visual or pose-tracking guidance is distilled into student policies. Other works combine hierarchical and hybrid designs, such as HiLMa-Res~\cite{huang2024hilma}, which uses high-level RL to control Bézier parameters and base motion while relying on hybrid CPG–Bézier controllers for leg movements, and Pedipulate~\cite{arm2024pedipulate}, which demonstrates end-to-end RL for single-foot manipulation.
In the IL domain, Human2LocoMan~\cite{niu2025human2locoman} enables cross-embodiment transfer from XR-driven human demonstrations using a modular Transformer policy, effectively transferring human manipulation skills to quadrupeds.
Hybrid IL–RL frameworks further improve efficiency and generalization. He et al.~\cite{he2024learning} employ BC to train a high-level planner for grasp trajectories, while a low-level RL controller coordinates leg and single-leg manipulation. WildLMa~\cite{qiu2024wildlma} builds an IL-based skill library from VR demonstrations, sequencing and composing tasks under LLM guidance.

VLA-based frameworks have also emerged for high-level semantic reasoning. QUAR-VLA~\cite{ding2024quar} pioneers the application of VLA models to quadrupeds, while GeRM~\cite{song2024germ} and MoRE~\cite{zhao2025more} integrate mixture-of-experts architectures with offline RL to learn generalist visuomotor policies and Q-functions with enhanced generalization and decision quality. QUART-Online~\cite{tong2024quart} advances this line by introducing action-chunk discretization and semantic alignment training, enabling latency-free inference for quadrupedal VLA tasks.

Finally, advances in 3D semantic perception and high-level planning extend quadrupedal capabilities. GeFF~\cite{qiu2024learning} performs real-time NeRF-based reconstruction with semantic relevance fields to guide locomotion, while manipulation is executed via learned grasp models. At the task level, LLMs have been combined with policy libraries: Ouyang et al.~\cite{ouyang2024long} propose a hierarchical framework where LLMs parse long-horizon, multi-skill instructions into structured subgoals executed by RL-based skills, bridging symbolic reasoning and continuous control.

\noindent \textbf{Challenges.}
In addition to common challenges such as balance–manipulation coupling, terrain adaptability, and perception delays, real-world deployment remains difficult due to the sim-to-real gap caused by modeling inaccuracies and sensor noise. To mitigate this, fully autonomous RL pipelines have been developed. Mendonca et al.~\cite{mendonca2025continuously} propose a framework that integrates on-policy data collection with continuous training, while ASC~\cite{yokoyama2023asc} addresses long-horizon tasks by decomposing them into modular skills trained via RL, coordinating them through a skill-switching policy jointly trained with IL and RL, and introducing a corrective policy to improve robustness during deployment.
Long-horizon task execution itself poses another significant challenge. Cheng et al.~\cite{cheng2023legs} propose a stage-wise RL framework that independently learns locomotion and single-leg manipulation skills, which are later composed via a behavior tree to accomplish temporally extended tasks.


\input{figures/4_manipulation_tasks/case_humanoid}


% Humanoid Manipulation
\subsection{Humanoid Manipulation}
Humanoid manipulation involves robotic platforms with human-like morphology, typically including a torso, two arms, and either simplified 2-DoF or fully dexterous hands, with the lower body implemented as either a mobile base or bipedal legs. These systems are designed to perform object interaction tasks in human environments.
These systems seek to replicate or extend human manipulation capabilities, enabling actions such as grasping, lifting, tool use, and coordinated bimanual operations, as illustrated in Figure~\ref{fig: case_human}. While the humanoid form offers natural compatibility with tools and environments built for humans, it also introduces challenges in balance control, whole-body coordination, and fine motor skills, making humanoid manipulation a central research focus in robotics and embodied intelligence.

\noindent \textbf{Non-Learning-based Methods.}
Early humanoid control primarily relied on traditional approaches such as rule-based and analytical controllers~\cite{harada2006dynamics, bouyarmane2012humanoid}. Some works also explored the integration of learning-based models into control frameworks. For example, OKAMI~\cite{li2025okami} leverages 3D human pose estimation from a single human video to infer joint positions and derive executable actions for humanoid robots via inverse kinematics.

\noindent \textbf{Learning-based Methods.}
The recent trend in humanoid manipulation has shifted from hand-tuned controllers toward fully learning-based models. As highlighted in~\cite{gu2025humanoid}, the field remains underexplored, with existing methods falling broadly into RL, IL, and VLA frameworks.

For RL-based approaches, FLAM~\cite{zhang2025flam} leverages a pre-trained human motion foundation model to score the stability of humanoid poses, using this score as an auxiliary reward to encourage balanced behaviors. Xie et al.~\cite{xie2023hierarchical} combine diffusion-based motion generation with reinforcement learning to achieve whole-body humanoid manipulation.
In the domain of IL, TRILL~\cite{seo2023deep} directly maps RGB images to pose commands, while OmniH2O~\cite{he2025omnih2o} abstracts unified motion goals from diverse modalities (e.g., language, RGB, MoCap, VR) using a diffusion policy. iDP3~\cite{ze2025generalizable} adapts the classic DP3 diffusion policy from third-person to egocentric views, enabling teleoperation of the head, torso, and arms. Qiu et al.~\cite{qiu2025humanoid} leverage large-scale egocentric demonstrations to align human and robot actions in a shared representation space, and TACT~\cite{murooka2025tact} incorporates tactile feedback to improve manipulation robustness.
Hybrid RL+IL strategies have also been proposed. For example, André et al.~\cite{schakkal2025hierarchical} decouple locomotion and manipulation by training a mid-level trajectory generator with IL to specify motion goals, while using RL to optimize a low-level tracking policy for accurate execution.

Finally, VLA methods aim to develop end-to-end language-conditioned policies for joint locomotion and manipulation. HumanVLA~\cite{ding2025humanoid} encodes images and language separately, concatenates features, and decodes actions through an MLP. GR00T N1~\cite{bjorck2025gr00t} further integrates visual and tokenized language features via a VLM before feeding them into a diffusion-based head. Humanoid-VLA~\cite{xu2024humanvla} aligns language and action spaces using cross-attention to fuse visual features, while TrajBooster~\cite{liu2025trajbooster} introduces a loco-manipulation VLA trained with retargeted data from real-world to simulation.

\noindent \textbf{Challenges.}
In addition to challenges such as multimodal perception, balance–manipulation coupling, and high degrees of freedom, humanoid manipulation also struggles with enabling multi-agent collaboration. For instance, CooHOI~\cite{gao2024coohoi} exploits object dynamics as an implicit communication channel to achieve coordinated manipulation across multiple agents. To further address the sim-to-real gap, Lin et al.~\cite{lin2025sim} introduce a generalizable reward formulation and a decoupled RL architecture, which improve sample efficiency through staged training.


==> sections/5_high-level_planner/affordance_learning.tex <==
% Affordance
% \section{Affordance Learning}
% \label{subsec: affordance_learning}

% A unified understanding of robot manipulation requires moving beyond asking what things are to discerning what can be done with them. The concept of affordance, originating from psychologist J.J. Gibson, provides a powerful framework for this shift~\cite{gibson2014theory}. In robotics, an affordance represents the potential for interaction an object or environment offers relative to a robot's capabilities—a door affords opening, a surface affords placing. By intrinsically linking perception to action, affordances serve as a foundational bridge for building more general and intelligent manipulation systems.

% The study of affordances has evolved from early model-based geometric reasoning to modern data-driven paradigms. The rise of deep learning, in particular, now enables robots to learn functional properties directly from raw sensory data, often through self-supervised interaction. This chapter explores the central role of affordance in this modern context, dissecting the concept from four critical perspectives.

% \subsection{Articulated Object Affordance}
% A significant frontier in robot manipulation is the interaction with articulated objects. Unlike their rigid counterparts, the affordances of objects like cabinets, laptops, and drawers are not merely defined by their static surface properties but are governed by their underlying, often unobservable, kinematic structures. This introduces the challenge of perceiving kinematic affordance: the potential for motion dictated by joints, axes, and constraints. A unified understanding of manipulation must therefore encompass the ability to infer these latent physical properties and translate them into effective interaction strategies.

% A foundational approach to uncovering these hidden kinematics is through physical interaction. By observing an object's state change before and after a manipulation attempt, a robot can infer its articulation model. Ditto~\cite{jiang2022ditto} exemplifies this principle by employing interactive perception to build interactive `digital twins' of real-world objects. From a pair of point cloud observations, Ditto jointly reconstructs part-level geometry and estimates the articulation model (e.g., revolute or prismatic joints), creating a fully-fledged virtual representation that can be instantiated in a physics simulator. This line of work establishes that interaction is a key modality for grounding a robot's understanding of an object's physical possibilities.

% The advent of Large Language and Vision-Language Models (LLMs and VLMs) has catalyzed a paradigm shift, moving from purely geometric reasoning to a synthesis of semantics, physics, and language. These models offer the potential to reason about manipulation in a more human-like, conceptual manner. A key insight is the need to bridge human-defined semantic parts with their physical functionalities. SAGE~\cite{geng2024sage} explicitly addresses this by distinguishing between an object's semantic parts (e.g., a `container') and its actionable parts (e.g., a `pressable button'), fusing the general knowledge of a VLM with the predictions of a domain-specific model to ground instructions. Building on this, other works explore how to effectively communicate kinematic knowledge to LLMs. The framework of Kinematic-aware Prompting~\cite{xia2024kinematic} proposes a unified parser that translates an object's kinematic structure into a structured textual description. This description is then used to prompt an LLM, guiding it to generate a sequence of low-level 3D waypoints for the robot, effectively converting abstract physical knowledge into concrete actions.

% This integration of language and reasoning has paved the way for learning robot-agnostic, object-centric representations that encapsulate affordances more directly. Instead of learning robot-specific actions, these methods aim to predict an intrinsic, actionable model of the object itself. A3VLM~\cite{huang2025a3vlm} pioneers this by training a VLM to predict a compact triad—(Bounding Box, Axis, Semantic Label)—from a single RGB image. This object-centric representation contains all the necessary information for a robot to derive a manipulation policy using simple action primitives. Pushing this concept towards greater generality, UniAff~\cite{yu2025uniaffunifiedrepresentationaffordances} introduces a unified affordance representation for both articulated objects and tools, demonstrating that a single VLM can learn a common functional vocabulary that spans diverse object categories and manipulation tasks.

% Finally, for any manipulation framework to be truly robust in the real world, it must be able to learn from and recover from failure. Recent work has focused on closing the loop through interactive correction. AIC MLLM~\cite{xiong2025autonomous} introduces a system that leverages failed interactions to improve subsequent attempts. When an action fails to produce the desired motion, a feedback module extracts information about the failure—for instance, by generating a visual mask over an unmovable part. This feedback is then used to prompt the MLLM to correct its next SE(3) pose prediction. By incorporating mechanisms for self-reflection and correction, such as Test-Time Adaptation (TTA), the system becomes more resilient and adaptive. This ability to reason about and learn from failure is a crucial component of a unified understanding of manipulation, enabling robots to operate more robustly in complex and unstructured environments.

% \subsection{Part-based Object Affordance}

% A central tenet for achieving a unified understanding of manipulation is the principle of compositionality. Humans effortlessly generalize manipulation skills to novel objects not by memorizing every object's function, but by understanding that objects are assemblies of functional parts. A handle affords grasping, a lid affords opening, and a container affords holding, regardless of whether these parts belong to a mug, a pot, or a novel kitchen gadget. This part-based reasoning is fundamental to generalization, allowing an agent to compose known part-level skills to interact with a virtually infinite variety of unseen objects.

% The formalization of this idea in robotics was significantly advanced by the concept of Generalizable and Actionable Parts (GAParts), introduced in GAPartNet~\cite{geng2023gapartnet}. This work established a large-scale dataset and a clear taxonomy for parts that are not only visually similar across different object categories (generalizable) but also share consistent manipulation strategies (actionable). By defining canonical coordinate frames and interaction semantics for classes like `hinge doors' or `line handles,' GAPartNet provided a foundational vocabulary for part-based affordance learning. Building upon this, PartManip~\cite{geng2023partmanip} demonstrated how to learn cross-category manipulation policies by first training a state-based expert with access to ground-truth part information and then distilling this knowledge into a vision-based student that operates on raw point clouds. This progression illustrates a concrete pathway from conceptual part definitions to learned, vision-driven manipulation skills.

% The utility of part-based understanding is greatly amplified when connected to natural language, enabling robots to perform more fine-grained, instruction-driven tasks. While manipulating a `handle' is a primitive skill, following a command like `pick up the bottle and show me the cap' requires a deeper reasoning about the relationship between parts and the user's intent. The PartInstruct benchmark~\cite{yin2025partinstruct} was created to drive research in this direction, providing a large-scale dataset of part-level instructions and expert demonstrations for complex, multi-step tasks. Concurrently, works like 3DAPNet~\cite{nguyen2024language} have focused on grounding open-vocabulary language labels (e.g., `grasp to pour') directly to specific part regions and their corresponding 6-DoF interaction poses, effectively creating a language-conditioned affordance-pose detector.

% Beyond recognizing and acting on individual parts, a more advanced form of compositional reasoning involves decomposing entire actions into a set of relationships between parts. Composable Part-based Manipulation (CPM)~\cite{liu2023composable} introduces the novel idea that a functional action can be represented as a composition of part-part functional correspondences. For example, the `pouring' action is not a monolithic skill but a combination of constraints:
% align, rim\_source, rim\_target, tilt, body\_source, body\_target, and facing-up, handle\_source, body\_target.
% CPM employs a collection of composable diffusion models, each trained to capture a primitive correspondence. At inference time, these models are combined to generate manipulation parameters that satisfy all constraints simultaneously. This approach provides a powerful generative framework for manipulation, enabling zero-shot generalization to novel object categories by composing learned, primitive part-level relationships. This shift from part-centric affordances to inter-part relations represents a significant step towards a more flexible and unified understanding of manipulation.



% \subsection{Spatial Affordance}

% While understanding the affordances of individual objects is crucial, intelligent manipulation in unstructured environments requires reasoning that extends beyond the object to the scene itself. This gives rise to the concept of spatial affordance, which concerns the interactive possibilities defined by the spatial layout of a scene and the relationships between its entities. It addresses questions not of what an object can do, but where an action can take place—where an item can be placed, which gap can be traversed, or how objects can be arranged relative to one another. A unified understanding of manipulation must therefore account for this contextual, scene-level reasoning.

% A primary challenge has been that standard VLMs, trained on internet-scale 2D image-caption pairs, inherently lack a robust understanding of 3D space. Foundational work has thus focused on injecting this basic spatial knowledge into VLMs through large-scale data synthesis. Frameworks like SpatialVLM~\cite{chen2024spatialvlm} and SpatialBot~\cite{cai2025spatialbot} pioneered this data-centric approach. By leveraging off-the-shelf vision models (e.g., for metric depth estimation) to lift 2D images into 3D, they automatically generated massive Visual Question Answering (VQA) datasets. Training on these datasets, which contain millions of questions about metric distances, sizes, and relative positions, endows VLMs with a foundational vocabulary for spatial reasoning.

% With this basic vocabulary established, the next step is to tailor spatial understanding for robotic action. The ROBO SPATIAL~\cite{song2025robospatial} benchmark was designed for this purpose, defining three core categories of robotics-relevant spatial queries: spatial configuration (e.g., "Is the mug to the left of the laptop?"), spatial compatibility (e.g., "Can the chair fit in front of the table?"), and spatial context (e.g., "Point to a vacant space on the counter."). Critically, this work emphasizes the importance of reasoning across multiple reference frames—ego-centric, world-centric, and object-centric—a capability essential for any embodied agent that must interpret commands from different perspectives.

% Even with a conceptual understanding of where an action is possible, a robot requires a precise target for execution. A significant leap in bridging high-level reasoning and low-level control has been the move towards precise, point-based outputs. RoboPoint~\cite{yuan2025robopoint} trains a VLM to predict a specific pixel coordinate as a "spatial affordance point" that directly grounds a language instruction. Instead of outputting a text answer, the model points to the exact location where an action, such as placing or grasping, should occur. This directly translates abstract spatial language into an actionable target. A parallel line of work, Robotic Visual Instruction (VIEW)~\cite{li2025robotic}, addresses the precision problem from the input side, proposing a paradigm where users communicate spatial intent through unambiguous, hand-drawn sketches like arrows and circles, which are then decoded into robot actions.

% Ultimately, a robust and generalizable spatial understanding system must flexibly integrate diverse forms of spatial information. Recent work has begun to analyze the spectrum of spatially-grounded mid-level representations that bridge high-level perception and low-level action~\cite{yang2025bridging}. This research categorizes representations along dimensions such as object-centricity, motion-centricity, pose-awareness, and depth-awareness, finding that different manipulation tasks benefit from different types of grounding. To leverage this insight, they propose a Mixture-of-Experts (MoE) policy architecture that dynamically combines multiple specialized models, each trained on a distinct mid-level representation. This approach acknowledges that there is no single "best" spatial representation; rather, a unified understanding emerges from the ability to synthesize the right spatial information for the task at hand. This progression—from learning basic spatial concepts to reasoning about actionable possibilities and finally to flexibly combining precise, multi-faceted spatial representations—is critical for enabling robots to operate intelligently and reliably in complex human environments.



% \subsection{Visual Affordance}
% Visual affordance learning serves as the critical bridge connecting raw perceptual input to executable robot actions. It is fundamentally a grounding problem: how to transform high-dimensional sensor data, such as pixels or point clouds, into a representation that encodes interaction possibilities. The evolution of visual affordance representations—from dense spatial maps to sparse keypoints, and from static 2D views to dynamic 3D understanding—charts a clear path towards a more unified and capable framework for robot manipulation.

% A foundational paradigm in this area was established by Transporter Networks~\cite{zeng2021transporter}, which reformulated manipulation as a visual correspondence problem. By learning dense, pixel-aligned feature maps from top-down orthographic images, this approach could predict affordance heatmaps for "picking" and "placing" through spatial feature matching (cross-correlation). The inherent SE(2) equivariance of this formulation made it remarkably data-efficient and established a powerful "where" pathway for action, grounding manipulation directly in the visual space without explicit object models.

% While spatially precise, this initial paradigm lacked semantic understanding. The subsequent integration of pre-trained vision-language models (VLMs) was a pivotal step. CLIPort~\cite{shridhar2022cliport} ingeniously combined the semantic prowess of CLIP with the spatial accuracy of Transporter Networks, introducing a two-stream architecture. A semantic "what" pathway interprets the language instruction, while a spatial "where" pathway identifies the precise location for interaction. This decoupling of "what" and "where" proved highly effective. Further research demonstrated that such visual affordance maps need not rely solely on expert demonstrations; they can be learned in a self-supervised manner from unstructured "play" data, as shown by VAPO~\cite{borjadiaz2022affordance}, and can be used to guide hierarchical policies, as in HULC++~\cite{mees2023grounding}.

% Despite their success, dense heatmaps can lack the precision required for fine-grained tasks. This led to a shift towards sparser, more object-centric representations. KITE~\cite{sundaresan2023kite} championed this shift by grounding language instructions not to a dense map, but to a discrete set of 2D keypoints. This representation offers superior precision and cleanly decouples the problem into a grounding module, which identifies the exact point of interaction, and an acting module, which executes a keypoint-conditioned skill. This focus on sparse, semantically meaningful points marked a significant refinement in visual affordance representation.

% Furthermore, most early methods were constrained by their reliance on canonical, often top-down, 2D camera views, limiting their applicability in mobile manipulation. SLAP~\cite{parashar2023spatiallanguageattentionpoliciesefficient} addressed this by transitioning the visual input modality from 2D images or voxels to 3D point cloud "tokens". This inherently view-invariant representation allows the policy to reason about affordances from arbitrary, egocentric viewpoints, a crucial capability for robots operating in dynamic, real-world environments.

% More recently, the role of foundation models has evolved from passive feature extractors to active reasoning engines that communicate visually. This is exemplified by the paradigm of visual prompting. MOKA~\cite{liu2024moka} introduced a method where a VLM generates explicit visual "marks" (e.g., colored dots) on an image to unambiguously guide a low-level policy. Taking this a step further, PIVOT~\cite{nasiriany2024pivot} proposed an iterative process where a VLM suggests a visual action, a verifier assesses its feasibility, and the VLM refines its proposal based on the feedback. This transforms visual affordance prediction from a single-shot inference into a closed-loop, deliberative reasoning process.


\subsection{Affordance Learning}
\label{sec:affordance_learning}

A unified understanding of robot manipulation requires moving beyond asking \textit{what} things are to discerning \textit{what can be done} with them. The concept of affordance, originating from psychologist J.J. Gibson, provides a powerful framework for this shift~\cite{gibson2014theory}. In robotics, an affordance represents the potential for interaction an object or environment offers relative to an agent's capabilities—a door affords opening, a surface affords placing. By intrinsically linking perception to action, affordances serve as a foundational bridge for building more general and intelligent manipulation systems.

The study of affordances has evolved from early model-based geometric reasoning to modern data-driven paradigms. The rise of deep learning, in particular, now enables robots to learn functional properties directly from raw sensory data, often through self-supervised interaction or by leveraging the vast knowledge embedded in foundation models. This chapter explores the central role of affordance in this modern context, dissecting the concept from four critical perspectives based on the primary source of information: geometric, visual, semantic, and multimodal.

\subsubsection{Geometric Affordance}
\label{subsec:geometric_affordance}

Geometric affordance posits that an object's functional possibilities are fundamentally dictated by its three-dimensional shape, structure, and kinematics. Research in this area often focuses on inferring an object's kinematic model—its parts, joints, and movement constraints—directly from its 3D geometry~\cite{jiang2022ditto, geng2023gapartnet, geng2023partmanip}. For example, interactive approaches like Ditto~\cite{jiang2022ditto} discover articulation models by physically probing an object and observing its response.

A key principle for generalizing geometric affordances is \textit{compositionality}, where the function of a complex object is understood as the sum of its functional parts~\cite{geng2023gapartnet, geng2023partmanip, liu2023composable}. Landmark efforts such as GAPartNet~\cite{geng2023gapartnet} established taxonomies of cross-category parts, enabling policies to learn skills for ``any handle'' rather than ``a specific mug's handle''. More advanced frameworks like CPM~\cite{liu2023composable} take this further by representing complex actions not as monolithic skills, but as a composition of geometric constraints between the constituent parts of interacting objects.

\subsubsection{Visual Affordance}
\label{subsec:visual_affordance}

Visual affordance focuses on directly learning interaction possibilities from 2D visual data, such as RGB or RGB-D images. This paradigm typically formulates manipulation as a visual correspondence problem, learning to produce dense, pixel-wise affordance maps that indicate where an action can be performed~\cite{zeng2021transporter, borjadiaz2022affordancelearningplaysampleefficient, geng2022endtoendaffordancelearningrobotic, tang2025functofunctioncentriconeshotimitation, kim2025screwsplatendtoendmethodarticulated}.

The seminal Transporter Networks~\cite{zeng2021transporter} established this approach by using a spatially equivariant architecture to predict pick-and-place heatmaps via feature matching. This powerful ``where'' pathway grounds manipulation directly in the pixel space without needing explicit object models. The scalability of this idea was later enhanced by methods like VAPO~\cite{borjadiaz2022affordancelearningplaysampleefficient}, which demonstrated that such visual affordance maps could be learned in a self-supervised manner from unstructured ``play'' data, significantly reducing the reliance on expert demonstrations.

\subsubsection{Semantic Affordance}
\label{subsec:semantic_affordance}

Semantic affordance explores the connection between high-level, symbolic concepts and an agent's actions. Before the widespread adoption of modern foundation models, this line of research focused on how human-defined semantic labels, such as object categories or part names, could guide robot behavior. This perspective represents an early effort to bridge symbolic reasoning with physical interaction, providing a historical context for the multimodal approaches that dominate the field today.

For example, pioneering research in affordance-based imitation learning~\cite{4399517} investigated how a robot could learn to manipulate objects by associating semantic properties with observed human actions. By identifying object parts like ``handles'' or ``lids'' and linking them to specific manipulation trajectories, the robot could generalize its learned skills to new objects that shared similar semantic attributes. While often limited by the need for pre-defined semantic categories, these methods established the critical principle that abstract, human-understandable knowledge is a powerful prior for guiding robot learning.

\subsubsection{Multimodal Affordance}
\label{subsec:multimodal_affordance}

The current frontier of affordance learning lies in the fusion of multiple information modalities, driven by the powerful reasoning and grounding capabilities of Vision-Language Models (VLMs) and Large Language Models (LLMs). This multimodal perspective moves beyond any single source of information, aiming to create a holistic understanding of interaction potential by synthesizing visual appearance, linguistic instruction, spatial context, and geometric structure.

A dominant research thrust is the fusion of natural language with visual perception, allowing robots to ground high-level instructions in the scene~\cite{shridhar2022cliport, mees2023grounding, yin2025partinstruct, geng2024sage, huang2025a3vlm}. Landmark architectures like CLIPort~\cite{shridhar2022cliport} introduced a two-stream model, effectively creating a semantic "what" pathway to interpret language and a spatial "where" pathway to localize the action. This principle has been extended to ground language to ever-finer details, such as specific object parts~\cite{yin2025partinstruct, geng2024sage}.

Another critical fusion involves endowing models with an explicit understanding of 3D space, enabling them to reason about metric properties like distance, orientation, and layout~\cite{chen2024spatialvlm, cai2025spatialbot, song2025robospatial, yuan2025robopoint}. To make this spatial understanding directly actionable, methods like RoboPoint~\cite{yuan2025robopoint} train models to output a precise pixel coordinate as a "spatial affordance point," translating abstract spatial language into a concrete target.

Furthermore, the interaction paradigm itself is evolving into a multimodal dialogue, incorporating new input modalities and enabling models to reason and recover from failure~\cite{liu2024moka, li2025robotic, huang2024copageneralroboticmanipulation, xiong2025autonomous}. For instance, visual prompting approaches like MOKA~\cite{liu2024moka} allow a VLM to generate explicit visual ``mark'' on an image to unambiguously guide a policy, while frameworks like AIC-MLLM~\cite{xiong2025autonomous} enable the model to learn from its own failures through interactive correction.

Finally, a key goal is to learn unified and generalizable affordance representations that transfer to novel objects and tasks~\cite{yu2025uniaff, tang2025uad, kuang2025ram}. This is pursued by learning unified representations for diverse object types, such as tools and articulated objects~\cite{yu2025uniaff}, or by developing methods for unsupervised or retrieval-based affordance transfer to unseen objects~\cite{tang2025uad, kuang2025ram}. This convergence of modalities is paving the way for robots that can reason about and act upon a much richer and more nuanced understanding of the world.


\subsection{3D Representation as Planner}
Although 3D representations such as Gaussian Splatting and Neural Descriptor Fields do not directly produce control signals, they function as planning modules by generating structured action proposals (e.g., 6-DoF grasps, relational rearrangements, or optimization costs). In this sense, they serve as mid-level planners that bridge perception and action, and are therefore included under the high-level planning category.

Recent work on manipulation has converged on mid-level 3D scene representations that turn perception into actionable proposals (e.g., 6-DoF grasps, keyframes, or cost fields) rather than full task plans. Two trends drive this line: (i) editable, real-time Gaussian splatting (GS) variants that fuse geometry with semantics/motion and enable scene editing, and (ii) implicit/descriptor fields that distill features from 2D foundation models into 3D for correspondence and language grounding.

\textbf{Gaussian-splatting scene representations and editing.}
Splat-MOVER builds a modular stack (ASK/SEE/Grasp-Splat) for open-vocabulary manipulation by distilling semantics/affordances into a 3DGS “digital twin,” then proposing grasp candidates for planning~\cite{shorinwa2025splat}. 
Object-Aware GS adds object-centric, 30 Hz dynamic reconstruction with semantics~\cite{li2024object}. 
Physically Embodied GS couples particles (physics) to 3DGS (vision) for a real-time, visually-correctable world model~\cite{abou2025physically}. 
MSGField uses 2DGS with attached motion/semantic attributes for language-guided manipulation in dynamic scenes~\cite{sheng2024msgfield}. 
RoboSplat directly edits 3DGS reconstructions to synthesize diverse demonstrations (objects, poses, views, lighting, embodiments), substantially boosting one-shot visuomotor policy generalization~\cite{yang2025novel}.

\textbf{Implicit/descriptor fields.}
NDF learns SE(3)-equivariant descriptors for few-shot pose transfer~\cite{simeonov2022neural}; R-NDF extends to relational rearrangement across objects~\cite{simeonov2023se}; F3RM distills CLIP features into 3D fields for few-shot, language-conditioned grasp/place~\cite{shen2023distilled}; $D^3$Fields builds dynamic 3D descriptor fields that support zero-shot rearrangement via image-specified goals~\cite{wang2025d}.

\textbf{Generative world models.}
Imagination Policy “imagines” target point clouds and converts them to keyframe actions via rigid registration—turning action inference into a local generative task with strong real-robot result~\cite{huang2025imagination}.

\textbf{Structured scene graphs.}
RoboEXP incrementally constructs an action-conditioned scene graph (ACSG) via interactive exploration, enriching the state with action-relevant relations for downstream manipulation~\cite{jiang2025roboexp}.

==> sections/7-bottlenecks.tex <==
\section{Bottlenecks in Robot Manipulation}
\label{sec: bottleneacks}

Despite the remarkable progress of robot manipulation in recent years, achieving general-purpose, real-world deployment in unstructured environments remains constrained by fundamental bottlenecks. Among these, two stand out as the most critical. The first lies in data, since the quality, diversity, and utilization of data directly determine the scalability of imitation and reinforcement learning methods. The second is generalization, which is essential for transferring skills across unseen environments, novel tasks, and diverse embodiments. Addressing these two dimensions—data and generalization—represents a central challenge for advancing robot manipulation toward robust and adaptable real-world performance.

\input{sections/7-bottlenecks/data}

\input{sections/7-bottlenecks/generalization}

==> sections/7-bottlenecks/data.tex <==
% 以收集和利用数据分类

\input{tables/7-bottlenecks/data}

\subsection{Data Collection and Utilization}
\label{subsec: data}

Data lies at the core of imitation learning and embodied intelligence, as its quality, diversity, and scale fundamentally determine the effectiveness and generalization of learned policies. Unlike conventional machine learning, robotic learning requires data that reflects not only perception but also action and embodiment, making data both the most valuable resource and the main bottleneck for progress in the field.
This section focuses on two key aspects. Data collection defines how demonstrations and interaction experiences are acquired, including human teleoperation, human-in-the-loop enhancement, synthetic generation, and crowdsourced collection. Data utilization addresses how collected data are leveraged through processes such as selection, retrieval, augmentation, expansion, and reweighting to improve robustness and efficiency. Together, collection and utilization form the foundation for training, evaluating, and scaling imitation learning methods toward real-world embodied intelligence.

\subsubsection{Data Collection}
\label{subsubsec:data_collect}
Data collection for robot learning spans multiple paradigms that differ in cost, scalability, embodiment alignment, and reliance on humans. 
Broadly, existing approaches can be grouped into four categories. 
First, \textbf{human teleoperation and demonstration} systems provide direct supervision through diverse interfaces. 
Second, \textbf{human-in-the-loop} methods allow selective correction or guidance to improve efficiency and robustness. 
Third, \textbf{synthetic or automatic} data generation leverages models or simulation to scale beyond human effort. 
Finally, \textbf{crowdsourcing frameworks} distribute the collection process across a wide base of contributors, lowering cost and broadening coverage. 
The following paragraphs summarize representative efforts within each category.

\paragraph{Human Teleoperation and Demonstration}
Human teleoperation remains the most direct and widely used paradigm for robot data collection. 
Existing systems can be broadly categorized by their interface design and embodiment alignment, 
each offering different trade–offs in scalability, fidelity, and ease of deployment.

\noindent \textbf{Cost–Effective and Scalable Teleoperation.}
Several systems~\cite{young2021visual, qin2023anyteleop, wu2024gello, chi2024universal, iyer2025open} target low cost and ease of deployment to scale data collection across platforms.
Young et al.~\cite{young2021visual} use everyday reacher–grabber tools to build a simple interface that acquires large visual imitation datasets and transfers to real robots.
AnyTeleop~\cite{qin2023anyteleop} offers a unified, modular vision–based stack that supports diverse robots, hands, and cameras in simulation and the real world.
GELLO~\cite{wu2024gello} provides a low–cost replica–arm framework that makes human control intuitive and scalable.
UMI~\cite{chi2024universal} supplies a portable framework that collects dexterous bimanual demonstrations and unifies data collection with policy learning for cross–platform deployment.
OPEN TEACH~\cite{iyer2025open} further leverages consumer VR headsets to gather natural hand–gesture demonstrations across morphologies.

\noindent \textbf{Feedback–Rich Teleoperation for Contact and Dexterity.}
Other work~\cite{kim2023training, kobayashi2025alpha, xue2025reactive, ding2024bunny} augments interfaces with force, tactile, or haptics to capture contact–rich behavior.
M2R~\cite{kim2023training} introduces a master–to–robot controller with force/torque sensing so that demonstrations encode interaction forces without expensive bilateral rigs.
ALPHA–BiACT~\cite{kobayashi2025alpha} combines bilateral force and position control for richer bimanual data.
RDP~\cite{xue2025reactive} integrates tactile–feedback teleoperation with slow–fast policy learning to improve contact–heavy manipulation.
Bunny–VisionPro~\cite{ding2024bunny} adds real–time VR hand tracking with low–cost haptics to enable fine dexterous demonstrations.

\noindent \textbf{Egocentric and XR Interfaces Aligning Viewpoints.}
XR and egocentric capture align human and robot observations to reduce the sim–to–human gap.
Zhang et al.~\cite{zhang2018deep} use consumer VR with motion controllers to place operators in the robot observation–action space on PR2.
EgoMimic~\cite{kareer2025egomimic} records egocentric AR video and hand motion for viewpoint–aligned teleoperation.
ARCap~\cite{chen2024arcap} overlays AR guidance and haptics so non–experts can record robot–feasible demonstrations.
Dhouioui et al.~\cite{dhouioui2024perspective} apply immersive VR to collect expert–quality demonstrations for molecular manipulation tasks.
In addition, active perception has been used to improve visibility in cluttered scenes, exemplified by AV-ALOHA~\cite{chuang2024active}, which adds an auxiliary camera arm to reduce occlusion and yield cleaner demonstrations.
  
\noindent \textbf{Embodiment Alignment via Exoskeletons and Replica Arms.}
A complementary line aligns human kinematics with robot embodiment to simplify mapping and increase precision.
AirExo~\cite{fang2024airexo} presents an affordable dual–arm exoskeleton that bridges human–robot kinematic differences and travels easily for in–the–wild collection.
DexUMI~\cite{xu2025dexumi} combines a wearable exoskeleton for motion alignment with a software pipeline for visual domain adaptation, yielding high–fidelity dexterous data.
Tilde~\cite{si2024tilde} introduces a TeleHand–DeltaHand pair for precise one–to–one in–hand teleoperation and data capture.
TeleMoMa~\cite{dass2024telemoma} extends to whole–body mobile manipulation with a modular multimodal teleoperation stack.

Together, these teleoperation systems illustrate a spectrum of design choices that balance scalability, fidelity, and embodiment alignment, forming the foundation for large-scale robot data collection.


\paragraph{Human-in-the-Loop Enhancement}
Human-in-the-loop approaches introduce targeted interventions and multi-round checks. 
By allowing humans to retrospectively verify outcomes or correct trajectories in real time, these methods improve data reliability. 
RoboCat~\cite{bousmalis2023robocat} introduces a self-improving generalist agent that finetunes on a small set of human demonstrations and then self-generates new trajectories, which are retrospectively labeled for success by humans, enabling automated evaluation and continual learning with minimal direct supervision.
DexCap\cite{wang2024dexcap} introduces a human-in-the-loop motion correction mechanism that combines residual correction and teleoperation, allowing real-time human intervention during policy execution.
IntervenGen\cite{hoque2024intervengen} introduces a novel data generation system that can autonomously produce a large set of corrective interventions with rich coverage of the state space from a small number of human interventions.
CR-DAgger\cite{xu2025compliant} introduces a compliant intervention interface and residual policy design that enable efficient use of minimal human corrections.


\paragraph{Synthetic and Automatic Data Generation}
Human demonstrations are costly and limited in coverage. 
Synthetic and automatic methods address this by reducing annotation effort and scaling data diversity through multi-round generation. 

% 基于llm vlm
\noindent \textbf{Leverage LLM/VLM for Generation.}
A recent branch of research~\cite{xiao2023robotic, ha2023scaling, zhang2024sprint, duan2025manipulate, zhou2025autonomous, blank2025scaling, jia2023seil} attempts to leverage LLMs for task decomposition, followed by planning or reinforcement learning to parse subtasks and generate demonstrations.
DIAL~\cite{xiao2023robotic} augments unlabeled demonstrations with automatically generated language instructions from pretrained vision–language models, enabling efficient training of language-conditioned policies and generalization without costly annotation.
Ha et al.~\cite{ha2023scaling} use LLM-guided planning and sampling to scale language-annotated data generation, then distill it into a robust multitask visuomotor policy with language-conditioned diffusion models, supporting retry-aware learning.
SPRINT~\cite{zhang2024sprint} relabels and composes instructions with large language models and applies language-conditioned offline reinforcement learning to chain skills across trajectories, improving downstream efficiency.
Manipulate-Anything~\cite{duan2025manipulate} generates self-correcting demonstrations with vision–language models without privileged information or hand-crafted skills, enabling zero-shot execution and robust policy training.
Other work advances autonomous improvement with foundation models (SOAR~\cite{zhou2025autonomous}), zero-shot natural-language annotation of long-horizon videos (NILS~\cite{blank2025scaling}), and symmetry-aware augmentation that mixes expert trajectories with simulated transitions (SEIL~\cite{jia2023seil}).

% 基于Synthetic
\noindent \textbf{Synthetic Sub-Trajectory Generation.} Another research direction is represented by MimicGen~\cite{mandlekar2023mimicgen} and its extensions\cite{jiangdexmimicgen, garrett2025skillmimicgen, hoque2024intervengen, jiangdexmimicgen}.
MimicGen\cite{mandlekar2023mimicgen} adapts a set of human-collected source demonstrations to novel object configurations by synthesizing corresponding execution plans. In principle, this approach is applicable to a wide range of manipulation skills and object types. For example, DexMimicGen~\cite{jiangdexmimicgen} extends the MimicGen strategy to support bimanual platforms equipped with dexterous hand end-effectors. However, the execution plans generated by MimicGen and its extensions~\cite{garrett2025skillmimicgen, hoque2024intervengen, jiangdexmimicgen} rely on costly physical robot deployments.
To address this, DemoGen~\cite{xue2025demogen} replaces expensive robot-collected demonstrations with an efficient, fully synthetic generation process, which leverages TAMP-based trajectory adaptation and 3D point cloud editing to produce diverse demonstrations.


\input{figures/7_bottlenecks/data_collect}


\paragraph{Crowdsourcing-based Data Collection}
Crowdsourcing reduces the cost and expertise barriers of robot demonstration collection, enabling large-scale and diverse data acquisition beyond what expert operators alone can provide.
A growing line of work leverages crowdsourcing to scale robot demonstration collection and reduce cost~\cite{chung2014accelerating, mandlekar2018roboturk, david2024unpleasantness, tung2021learning, duan2023ar2, liu2025egozero}.
RoboTurk~\cite{mandlekar2018roboturk} builds a smartphone teleoperation platform with a cloud backend. The design lowers entry barriers for remote workers, standardizes task setup and logging, and supports rapid collection of diverse manipulation trajectories at scale.  
David et al.~\cite{david2024unpleasantness} extend crowdsourced teleoperation from simulation to physical robots. The system addresses latency, safety, and reset logistics so that large numbers of real-robot demonstrations can be collected remotely across varied tasks.  
AR2-D2~\cite{duan2023ar2} removes the need for real robots during collection by using an iOS AR application to capture human–object interactions and scene geometry, which are later retargeted to robots to reduce hardware and supervision requirements.
Other work established the feasibility of platform-based collection~\cite{chung2014accelerating}, scaled to multi-arm settings by assigning one arm per worker~\cite{tung2021learning}, and enabled in-the-wild egocentric demonstrations with lightweight smart glasses~\cite{liu2025egozero}.


\subsubsection{Data Utilization}
Effectively utilizing existing data is essential for improving robot policy performance, especially under constraints of limited data collection budgets. Recent research has explored various strategies for selecting, retrieving, augmenting, expanding, and reweighing data to maximize its utility in training generalizable and robust manipulation policies.

\paragraph{Data Selection}
Raw robot datasets often contain noise, redundancy, or domain imbalance. To address this issue, recent work~\cite{gandhi2023eliciting, zheng2023extraneousness, belkhale2023data, dasari2023unbiased, kuhar2023learning, yue2024leverage, hejna2025remix, saxena2025matters} studies how to select, filter, and adjust data for robot learning, including trajectory filtering, preference-based pruning, domain-mixture curation, and the choice of pretraining sources.

EIL~\cite{zheng2023extraneousness} filters extraneous segments by learning action-conditioned embeddings with temporal cycle consistency and applying an unsupervised voting-based alignment procedure. This yields cleaner demonstration sets that better match task intent.
L2D~\cite{kuhar2023learning} evaluates heterogeneous human demonstrations with latent trajectory representations and preference learning, then selects higher-quality examples for offline imitation learning, improving robustness under mixed-quality data.
Re-Mix~\cite{hejna2025remix} formulates dataset curation as minimax reweighting over domain mixtures using excess behavior-cloning loss, automatically upweighting helpful domains while downweighting harmful ones to boost generalist policy performance.
Other work, EAD~\cite{gandhi2023eliciting} elicits aligned demonstrations via compatibility signals; DC-IL~\cite{belkhale2023data} defines action divergence and transition diversity as data-quality metrics to curb distribution shift; UVP~\cite{dasari2023unbiased} shows pretraining image distribution can matter more than dataset size; ILID~\cite{yue2024leverage} selects state–action pairs by scoring resultant states with a state-only discriminator; and MimicLabs~\cite{saxena2025matters} finds composition and retrieval that prioritize camera-pose and spatial diversity can outperform full-dataset training.


\paragraph{Data Retrieval}
Retrieval-based approaches address the data bottleneck in robot learning by mining task-relevant demonstrations or sub-trajectories from large prior corpora, thereby reducing sample complexity and improving transferability~\cite{pari2022surprising, nasiriany2023learning, du2023behavior, di2024effectiveness, di2024dinobot, zhu2024retrieval, yin2024offline, lin2025flowretrieval, memmel2025strap, kumar2025collage}.

A first line of work couples representation learning with non-parametric retrieval. VINN~\cite{pari2022surprising} learns a self-supervised visual encoder and performs nearest-neighbor search in the latent space, yielding a strong policy without gradient-based fine-tuning. SAILOR~\cite{nasiriany2023learning} organizes prior experience into a latent space of short-horizon skills and retrieves high-similarity sub-trajectories as reusable motion primitives, accelerating few-shot adaptation. Behavior Retrieval~\cite{du2023behavior} further introduces a variational encoder to score state–action similarity, seeding queries with limited expert rollouts and jointly training on both expert and retrieved data to reduce reliance on labeled trajectories.

Beyond representation-driven methods, more recent studies emphasize adaptation and integration. Di Palo and Johns~\cite{di2024effectiveness} retrieve and replay demonstrations through a three-stage decide–align–execute framework. DINOBot~\cite{di2024dinobot} adapts demonstrations to novel objects via pixel-level alignment on DINO-ViT features. RAEA~\cite{zhu2024retrieval} integrates trajectories from a multimodal memory directly into action prediction. GSR~\cite{yin2024offline} organizes prior interactions as a graph over pretrained embeddings to imitate high-value behaviors identified by search. FlowRetrieval~\cite{lin2025flowretrieval} leverages optical flow to mine cross-task motion segments, while STRAP~\cite{memmel2025strap} retrieves sub-trajectories with visual foundation models and time-invariant alignment. COLLAGE~\cite{kumar2025collage} fuses multiple similarity signals with adaptive weighting to curate high-quality training subsets from large datasets.
Together, these approaches demonstrate that effective retrieval, whether through robust representation spaces or advanced adaptation mechanisms, can serve as a powerful alternative or complement to direct policy learning, enabling efficient few-shot learning and improved generalization across tasks.

\paragraph{Data Augmentation}
We categorize augmentation strategies into three families: label and trajectory relabeling, physics- and geometry-consistent augmentation, and generative augmentation across visuals, viewpoints, and embodiments. These categories capture complementary aspects of how demonstrations can be reinterpreted, physically transformed, or perceptually diversified to improve learning.

\noindent \textbf{Label and Trajectory Relabeling.}
This family focuses on reinterpreting existing demonstrations by modifying goals, segmenting sequences, or generating counterfactuals. DAAG~\cite{di2025diffusion} relabels trajectories in a temporally and geometrically consistent way using diffusion models, aligning them with new instructions to improve sample efficiency and transfer. S2I~\cite{chen2025towards} segments demonstrations, applies contrastive selection, and optimizes trajectories to better leverage mixed-quality data. Related efforts include goal relabeling in GoalGAIL~\cite{ding2019goal} and counterfactual sample generation with variational inference in OILCA~\cite{he2023offline}.

\noindent \textbf{Physics- and Geometry-consistent Augmentation.}
This emphasis is on creating physically valid demonstrations through transformations consistent with real-world dynamics. Mitrano and Berenson~\cite{mitrano2022data} treat augmentation as an optimization problem, applying rigid-body transformations to generate diverse but valid manipulation examples. Wang et al.~\cite{wang2023identifying} first isolate high-quality rollouts, then exploit environmental symmetries to construct principled augmentations.

\noindent \textbf{Generative Visual, Viewpoint, and Embodiment Augmentation.}
This category uses generative models to expand perceptual diversity and embodiment coverage. GenAug~\cite{chen2023genaug} applies pretrained generative models for semantic scene edits that preserve behavior while enhancing visual variation. RoVi-Aug~\cite{chen2025rovi} employs diffusion-based image-to-image translation to synthesize demonstrations across robots and camera viewpoints, enabling zero-shot transfer to unseen embodiments. RoboPearls~\cite{tang2025robopearls} leverages 3D Gaussian Splatting to create editable, photorealistic reconstructions for language-guided demonstration synthesis. Additional efforts include text-guided masking in ROSIE~\cite{zhu2024retrieval}, deformable-eye novel view synthesis in DMD~\cite{zhang2024diffusion}, single-image 3D-aware view generation in VISTA~\cite{tian2025view}, and multi-rate sensory alignment in DABI~\cite{kobayashi2025dabi}.


\paragraph{Data Expansion}
We categorize expansion methods into two complementary families. The first focuses on synthesis and imagination, where generative models, planners, or simulators create new experiences beyond the collected data. The second emphasizes reuse and correction, where existing demonstrations are transformed, recombined, or augmented with targeted corrective data to enrich training.

\noindent \textbf{Synthesis and Imagined Rollouts.}
Generative Predecessor Models~\cite{schroecker2019generative} learn distributions over predecessor states and sample synthetic state–action pairs that converge into expert trajectories, thereby densifying the space of successful behaviors and improving reachability.
Self-Imitation by Planning~\cite{luo2021self} leverages planners to produce higher-quality rollouts from the same tasks and appends them to the dataset, forming an iterative improve–add–imitate loop that bootstraps policy performance.
Category-Level Manipulation~\cite{shen2022learning} applies adversarial self-imitation to generate novel category-level trajectories, augmenting raw demonstrations and strengthening generalization across object categories.
SAFARI~\cite{di2020safari} synthesizes imagined rollouts that respect safety constraints and corrective intent, creating counterfactual demonstrations that are otherwise costly or infeasible to collect.
TASTE-Rob~\cite{zhao2025taste} produces task-oriented hand–object interaction videos as demonstrations, enriching both visual and interaction diversity without requiring privileged labels.

\noindent \textbf{Reuse and Corrective Expansion.}
Scalable Multi-Task Imitation Learning~\cite{singh2020scalable} relabels collected trajectories across tasks so that each demonstration supervises multiple goals, enabling large-scale cross-task reuse.
JUICER~\cite{ankile2024juicer} decomposes demonstrations into reusable motion segments and recomposes them into new task sequences, achieving combinatorial growth of training data from a limited skill library.
Diff-DAgger~\cite{lee2025diff} estimates policy uncertainty with diffusion models and selectively collects or synthesizes corrective demonstrations only in uncertain regions, focusing supervision where failures are most likely.


\paragraph{Data Reweighting}
Data reweighting methods assign different importance to demonstrations based on quality, feasibility, or preference signals, rather than treating all data equally. This strategy mitigates the negative impact of suboptimal or inconsistent demonstrations and enhances policy learning by emphasizing high-value samples.
Beliaev~\cite{beliaev2022imitation} et al. propose an imitation learning approach that estimates each demonstrator’s expertise and uses it to weight the demonstration data.
FABCO~\cite{takahashi2025feasibility} presents a feasibility-aware imitation learning framework that assesses each human demonstration’s feasibility via the robot’s dynamics models and uses the estimated feasibility as a weight during policy learning.
PLARE~\cite{luu2025policy} introduces a method that dispenses with explicit reward modeling by querying a large vision-language model for preference labels on pairs of trajectory segments and then training the policy directly on these preference signals using a contrastive learning objective.
Together, these methods highlight how reweighting demonstrations based on expertise, feasibility, or preference signals can enhance policy learning by emphasizing high-quality data and mitigating the impact of suboptimal examples.

==> sections/7-bottlenecks/generalization.tex <==
% 以泛化任务利用分类
\subsection{Generalization}
\label{subsec: generalization_tasks}

\input{figures/7_bottlenecks/generalization}

Robotic manipulation generalization can be broadly categorized into three dimensions: environment generalization, task generalization, and cross-embodiment generalization. Environment generalization concerns robustness to variations in conditions such as Sim2Real transfer, spatial transformations, lighting, and background or distractor changes. Task generalization emphasizes maintaining performance across different task configurations, including long-horizon tasks, few-shot or meta-learning, continual learning, and skill composition. Cross-embodiment generalization focuses on transferring skills across robots with diverse morphologies, kinematics, dynamics, or sensing modalities, which is crucial for building general-purpose embodied agents. In what follows, we structure our survey along these three perspectives.

\subsubsection{Environment Generalization}

\paragraph{Sim2Real and Real2Sim2Real Generalization} 
Simulation offers a scalable alternative for training and evaluating manipulation policies, alleviating the high cost, operational risks, and safety concerns of large-scale real-world data collection. However, discrepancies in dynamics, sensing, and environmental complexity often result in poor transferability, commonly referred to as the sim-to-real gap~\cite{lyu2024scissorbot}. We categorize existing approaches into three paradigms based on how simulation and real-world data are leveraged to improve policy generalization: Simulation-Only Training, Real-World Adaptation, and Sim–Real Interaction.

\noindent \textbf{Simulation-Only Training.}
This paradigm assumes that policies trained with sufficient variability in simulation can directly transfer to the real world without further tuning. A common technique is domain randomization, where physical parameters (e.g., mass, friction, damping)~\cite{chen2021understanding} and perceptual cues (e.g., textures~\cite{tobin2017domain}, lighting~\cite{tremblay2018training}, object pose~\cite{ren2019domain}) are systematically perturbed to promote robustness. Peng et al.~\cite{peng2018sim} showed that randomized dynamics improve sim-to-real transfer, while more recent efforts such as DexScale~\cite{liu2025dexscale} scale up augmentation and randomization to further boost generalization. However, these approaches rely on the assumption that simulated variability adequately captures real-world complexity, which often fails for tasks requiring fine-grained sensing or multimodal interaction.

\noindent \textbf{Real-World Adaptation.}
This paradigm refines simulation-trained policies using real-world data, typically through fine-tuning, imitation, or online reinforcement learning. For instance, Josifovski et al.~\cite{josifovski2025safe} introduced safe continual adaptation under deployment constraints, whereas alternative methods employ pseudo-labeling or distillation to exploit real sensory streams with minimal annotation. Such methods offer greater robustness than simulation-only approaches but are limited by the cost and risk of real-world interaction, which constrains scalability in high-stakes domains.

\noindent \textbf{Sim–Real Interaction.}
Rather than treating adaptation as a post hoc correction, this paradigm reconstructs simulation directly from real-world data to close the sim-to-real loop~\cite{torne2024reconciling, dan2025x, yu2025real2render2real}. Advances such as 3D scanning enable the creation of high-fidelity digital twins. For example, RialTo~\cite{torne2024reconciling} builds task-specific scenes from minimal sensing and uses inverse distillation to learn transferable policies. Although requiring more infrastructure, this approach combines realism and scalability, enabling safer and more efficient learning in complex tasks where direct trial-and-error in the real world is impractical.

\paragraph{SE(3) and SIM(3)-Equivariance Generalization} 
A complementary strategy for environment generalization is to embed geometric equivariance into policy architectures. These methods enforce SE(3) or SIM(3)-equivariance so that representations stay consistent under viewpoint, pose, or scale changes. By doing so, policies can adapt to new perspectives and scene layouts without large amounts of retraining. Representative works include EquiBot \cite{yang2024equibot} and ET-SEED \cite{tie2024seed}, which design equivariant diffusion policies for robust manipulation. Adapt3R \cite{wilcox2025adapt3r} extends this idea with adaptive 3D scene representations. Recent work on active viewpoint control \cite{nakagawa2025imitation} also shows that imitation learning with neck motion can push manipulation beyond the initial field of view. Together, these works highlight geometric equivariance as a powerful inductive bias that complements sim2real pipelines.

\paragraph{Others}
Lighting, background, and distractor variations also present fundamental challenges for visual generalization in robotic manipulation, as policies often overfit to training conditions. Recent work tackles this issue through augmentation, representation learning, and context-robust imitation. Physically-based augmentation methods explicitly perturb lighting to improve robustness under illumination shifts~\cite{jin2025physically}. Object-centric and factorized representations aim to disentangle task-relevant features from background clutter, thereby narrowing the generalization gap~\cite{chapin2025object, xie2024decomposing}. Other approaches emphasize cross-context imitation, either by regularizing position-invariant features~\cite{yin2023spatial} or by learning from demonstrations collected under inconsistent or varying contexts~\cite{yang2020cross, qian2023robot}. At scale, foundation-model-based policies such as SwitchVLA~\cite{li2025switchvla} and Diffusion-VLA~\cite{wen2024diffusion} demonstrate improved resilience to distractors by leveraging large multimodal priors. Collectively, these studies highlight that addressing visual shifts is crucial for bridging the gap between controlled training settings and deployment in cluttered, dynamic environments.


\subsubsection{Task Generalization}

\paragraph{Generalization for Long-horizon Tasks}
Long-horizon robotic manipulation represents a core challenge for embodied intelligence. Unlike short-horizon tasks that typically involve single-skill execution, long-horizon problems demand the coordination of multiple sub-skills, hierarchical reasoning, and temporally abstract decision-making. Robust generalization requires agents not only to plan and execute extended action sequences but also to adapt across variations in task structure, object arrangement, and dynamic environments. Recent advances approach this challenge along three interconnected axes: skill compositionality, semantic task decomposition, and structure-aware representation learning.

\noindent \textbf{Skill Compositionality.}
At the foundation lies the ability to compose and reuse modular skills~\cite{chenu2022divide,lee2021adversarial,zhu2022bottom,belkhale2023hydra,agia2022stap,zhang2023bootstrap,liu2024learning}. STAP~\cite{agia2022stap} addresses sequencing by optimizing the feasibility of action chains. Generative frameworks such as BOSS~\cite{zhang2023bootstrap} and BLADE~\cite{liu2024learning} leverage large language models to autonomously expand skill libraries and incorporate semantic grounding into action spaces, thereby enabling flexible skill reuse and extension.

\noindent \textbf{Semantic Task Decomposition.}
Beyond static skill composition, multimodal semantics have been introduced to parse and decompose tasks into modular components~\cite{mu2025look, myers2024policy, dalal2025local, lin2024hierarchical, sundaresan2024s, mao2024dexskills}. PALO~\cite{myers2024policy} employs vision-language models to translate high-level task descriptions into reusable sub-tasks, enabling rapid adaptation with minimal supervision. ManipGen~\cite{dalal2025local} integrates local policies that encode invariances in pose, skill order, and scene layout, combining them with foundational models in vision and motion planning to generalize across unseen long-horizon sequences.

\noindent \textbf{Structure-Aware Representation Learning.}
A finer level of generalization is achieved through task-level abstraction and representation learning~\cite{triantafyllidis2023hybrid, tanwani2021sequential, wu2020squirl, chen2025backbone, chen2025robohorizon, yang2025bootstrapping}. TBBF~\cite{chen2025backbone} decomposes complex tasks into primitive therbligs, facilitating efficient action-object mappings and trajectory synthesis. RoboHorizon~\cite{chen2025robohorizon} formalizes a Recognize-Sense-Plan-Act pipeline by fusing LLMs with multi-view world models, addressing sparse reward supervision and perceptual complexity. HD-Space~\cite{yang2025bootstrapping} identifies atomic sub-task boundaries from demonstrations, improving sample efficiency and policy robustness with limited data.

\paragraph{Compositional Generalization}
Compositional generalization in robotic manipulation emphasizes the ability to solve novel tasks by systematically recombining known skills, objects, and instructions. Recent research explores diverse strategies to achieve this capability. One line of work focuses on data-driven efficiency, where targeted data collection strategies are designed to maximize coverage of compositional variations with minimal demonstrations, enabling scalable policy training~\cite{gao2024efficient}. Another approach grounds policies in programmatic or symbolic structures, allowing robots to leverage modular task representations for systematic recomposition and generalization to unseen task combinations~\cite{wang2023programmatically}. Complementary efforts investigate policy architectures that explicitly factorize control into entities or modules, facilitating the recombination of learned components to improve adaptability in complex environments~\cite{zhou2022policy}. Together, these methods illustrate a growing effort to move beyond rote memorization of tasks toward systematic generalization, enabling robots to flexibly adapt to combinatorial task spaces.

\paragraph{Few-shot Learning}
Few-shot learning enables robots to acquire skills from only a handful of demonstrations~\cite{chen2025vidbot, valassakis2022demonstrate, jain2024cobt, heppert2024ditto, li2025elastic}, alleviating the high cost of large-scale data collection. Research in this area can be broadly grouped into two directions: embedding structured priors and leveraging semantic transfer. 
One line of work embeds structured inductive biases into perception and control to maximize the utility of limited demonstrations. Domain-invariant constraints, including spatial equivariance, 3D geometry, or action continuity, are incorporated to reduce data requirements and improve generalization. For example, Ren et al.~\cite{ren2024learning} combine point cloud representations with a diffusion-based policy, achieving robust generalization from as few as ten demonstrations.
A complementary line of research emphasizes semantic transfer and compositional generalization. These methods extract transferable knowledge from alternative sources, such as human demonstrations or previously solved tasks, and adapt it to new objectives. For instance, YOTO~\cite{zhou2025you} maps human hand motions from video to dual-arm robotic skills, while TOPIC~\cite{song2025few} constructs task prompts and a dynamic relation graph to systematically reuse prior experience for new policy learning.

\paragraph{Meta Learning}
While closely related to few-shot learning, meta learning distinguishes itself by focusing on the ability to \emph{amortize} task adaptation. Instead of relying directly on structural priors or semantic transfer to generalize from a handful of demonstrations, meta learning trains over a distribution of tasks so that the model acquires a generic adaptation procedure. This paradigm equips robots with rapid adaptability to unseen tasks, even under extremely limited supervision~\cite{duan2017one,james2018task,di2023one,zhang2024one,bing2022meta,haldar2023teach,biza2023one}.

\noindent \textbf{Task-Conditioned Meta-Representations.}
One direction focuses on learning task-conditioned embeddings that serve as meta-representations. Early approaches such as Duan et al.~\cite{duan2017one} and TecNets~\cite{james2018task} encode demonstrations into low-dimensional vectors for policy conditioning. Later works extend this idea with relational graph networks~\cite{di2023one} or invariance-based objectives~\cite{zhang2024one}, enforcing structural consistency across tasks. These embedding-based approaches highlight the importance of compact task representations in accelerating policy adaptation.

\noindent \textbf{Cross-Modal and Instruction-Driven Adaptation.}
Another direction emphasizes the integration of additional modalities and task instructions into the adaptation process. MILLION~\cite{bing2022meta} incorporates natural language into the meta-learning loop, enabling semantically guided adaptation. FISH~\cite{haldar2023teach} demonstrates versatile skill acquisition from just one minute of demonstrations, while interaction-warping~\cite{biza2023one} aligns novel trajectories with past interaction structures to facilitate transfer. Collectively, these works establish meta learning as a principled framework for scalable and data-efficient generalization.

\paragraph{Lifelong, Continual and Incremental Learning}
Endowing robots with the ability to learn continuously is a key milestone toward building adaptive and autonomous embodied agents. This capability requires retaining previously acquired skills without forgetting while avoiding the need for complete retraining. In robotic manipulation, two closely related paradigms have emerged to address this challenge: lifelong learning (continual learning) and incremental learning. Although they differ in focus, both aim to support sustained performance in real-world scenarios.

\noindent \textbf{Lifelong and Continual Learning.} This paradigm emphasizes the retention and reuse of knowledge across sequential tasks~\cite{yao2025think, roy2025m2distill, gao2021cril, lei2025dynamic}. For instance, PPL~\cite{yao2025think} encodes reusable motion primitives as prompts, while DMPEL~\cite{lei2025dynamic} employs a modular ensemble of experts with coefficient replay. These approaches show that structured modularity, through either prompt-based reuse or expert specialization, facilitates forward transfer of knowledge while alleviating catastrophic forgetting.

\noindent \textbf{Incremental Learning.} In contrast, incremental learning addresses settings where robots acquire new atomic skills one task at a time. iManip~\cite{zheng2025imanip} formalizes this problem with a benchmark built on RLBench~\cite{james2020rlbench} and introduces an extendable PerceiverIO model that adapts action prompts for new primitives. By combining incremental model expansion with replay-based training, it supports effective skill accumulation while avoiding catastrophic forgetting. This paradigm underscores the importance of modular architectures and continual update mechanisms in enabling long-term learning for robotic manipulation.


\subsubsection{Cross-Embodiment Generalization}
Cross-embodiment generalization refers to the ability of robotic policies or representations to transfer across embodiments with different morphologies, kinematics, dynamics, or sensing modalities. This capability is critical for developing general-purpose embodied agents that operate seamlessly across diverse platforms, including arms, mobile manipulators, and humanoid robots.

\noindent \textbf{Latent Alignment.}
The latent alignment paradigm aims to achieve cross-embodiment generalization by mapping heterogeneous robot morphologies into a shared latent representation space, enabling policy transfer without explicit correspondence in state or action dimensions.
Early work such as XSkill~\cite{xu2023xskill} introduces an unsupervised framework that discovers embodiment-agnostic skills by disentangling latent motion factors, enabling reusable skill primitives across robots. Wang et al.~\cite{wang2024cross} extend this idea via latent space alignment, jointly optimizing a shared embedding to preserve action equivalence between morphologies and support transfer under mismatched kinematics. Latent Action Diffusion~\cite{bauer2025latent} advances this direction by employing diffusion-based generative modeling to interpolate and align latent actions across embodiments, achieving smooth and consistent transfer in high-dimensional manipulation tasks. Large-scale frameworks such as OmniMimic~\cite{yang2024pushing} and CrossFormer~\cite{doshi2024scaling} demonstrate that training on diverse embodiments within a unified latent action space produces scalable, general-purpose controllers capable of zero-shot transfer across manipulation, navigation, and locomotion. Similarly, HPT~\cite{wang2024scaling} integrates heterogeneous pre-trained visual and proprioceptive Transformers into a shared latent fusion module, improving robustness and coordination across embodiments. Together, these works position latent alignment as a scalable and principled foundation for bridging morphology-specific policies toward unified embodied intelligence.

\noindent \textbf{Skill Extension.}
The skill extension paradigm focuses on scaling and transferring manipulation abilities across embodiments, such as adapting single-arm policies to bimanual coordination or transferring skills between morphologically distinct manipulators. AnyBimanual~\cite{lu2025anybimanual} enables unimanual-to-bimanual transfer through shared latent representations and motion consistency constraints, decomposing dual-arm actions into coordinated single-arm primitives for flexible adaptation. Modularity through Attention~\cite{zhou2023modularity} employs an attention-based modular policy architecture that learns composable, language-conditioned skill representations, supporting efficient reuse across embodiments and tasks. These works collectively show that modular and structured representations provide a scalable foundation for skill extension and cross-embodiment transfer.

\noindent \textbf{Hierarchical Skill Library.}
The hierarchical skill library paradigm focuses on scalable frameworks that organize and coordinate manipulation skills across diverse embodiments through structured abstraction and modular design. RoboOS~\cite{tan2025roboos} introduces a hierarchical embodied framework that unifies cross-embodiment and multi-agent collaboration within an operating system–like architecture, abstracting perception, control, and communication into standardized APIs for shared skill reuse and adaptability. By integrating high-level task orchestration with low-level motion primitives, this hierarchical organization bridges engineering infrastructure and embodied intelligence, enabling large-scale, interoperable skill reuse across diverse robotic platforms.

\noindent \textbf{Other Strategies.}
Recent research on cross-embodiment learning explores complementary paradigms such as data augmentation, reinforcement learning, and SE(3)-equivariant control to address distinct transfer challenges. Mirage~\cite{chen2024mirage} uses cross-painting to re-render source observations for zero-shot transfer between robots. In RL, Human2Sim2Robot~\cite{lum2025crossing} bridges the human–robot gap with a single demonstration, while X-Sim~\cite{dan2025x} reconstructs high-fidelity simulations for real-to-sim-to-real policy reuse. LEGATO~\cite{seo2025legato} introduces an SE(3)-equivariant imitation framework that unifies perception and control using a shared grasping tool, enabling consistent transfer across morphologies. Collectively, these approaches advance robust cross-embodiment generalization through perceptual adaptation, RL-based alignment, and geometric consistency.

% \subsubsection{Others}
% A growing line of work argues that measuring ``generalization'' itself must be standardized, leading to taxonomies and benchmarks that emphasize visual, semantic, and behavioral axes \cite{gao2025taxonomy}. In parallel, The COLOSSEUM \cite{pumacay2024colosseum} establishes large-scale, reproducible benchmarks spanning diverse tasks and environments to stress robustness and transferability. Such standardized evaluations and datasets facilitate rigorous comparison across methods, promote reproducibility, and accelerate progress toward broadly generalizable robotic policies. 

% Beyond benchmark design, another line of research investigates algorithmic strategies for adaptation at deployment, particularly when robots encounter out-of-distribution (OOD) observations. Test-Time adaptation focuses on OOD observations encountered during deployment. Gupta et al. \cite{gupta2025adapting} propose a diffusion-based policy that queries human experts for functional analogies when encountering OOD inputs. The system substitutes unfamiliar observations with semantically similar training examples, enabling generalization without retraining. This approach demonstrates the effectiveness of interactive semantic alignment as a lightweight alternative to offline adaptation.



==> sections/8-applications.tex <==
% 以应用分类
\section{Applications}
\label{sec: applications}

Robotics research plays a central role in advancing intelligent systems with tangible real-world impact. Over the past decades, robots have evolved from rigid, hard-coded tools executing predefined routines into perceptive agents capable of interpreting and interacting with their environments, with vision as a primary modality. Today, empowered by large language models and multimodal foundation models, the field is rapidly progressing toward embodied intelligence, where robots integrate perception, planning, and control to accomplish complex tasks in dynamic and uncertain settings~\cite{zhang2025embodied, firoozi2025foundation}. This paradigm shift requires not only precise mechanical design but also robust and generalizable decision-making that enables robots to adapt flexibly across diverse tasks and user instructions. These advances are fueling applications in domestic, healthcare, industrial, and scientific domains. To illustrate these developments, Figure~\ref{fig: case_app} presents representative application domains and typical tasks across sectors. The remainder of this section focuses on these application scenarios, outlining how robots are being deployed in practice across different fields.


% \input{tables/8_applications/application}
\input{figures/8_applications/case_app}

\subsection{Household Assistance}
Robotic manipulation in household environments targets essential daily activities such as dressing, cooking, feeding, assisting, stowing, object rearrangement, and tool use. Dressing assistance has been studied through bimanual strategies and safe human-robot interaction with deformable garments~\cite{zhao2025bimanual, liu2024forcemimic, erickson2019multidimensional}. Cooking and feeding tasks emphasize contact-rich manipulation and adaptive policies for varied food types and configurations~\cite{liu2025forcemimic, liu2024adaptive, sundaresan2023learning}. Assistive care applications explore shared control and soft manipulators for elderly support~\cite{fu2025tasc, ansari2017towards}. Stowing and object rearrangement tasks leverage behavior primitives, language-guided planning, and vision-language models to enable flexible scene organization~\cite{chen2023predicting, jin2025paca, chang2024lgmcts, ding2023task, kapelyukh2023dall}. Finally, tool manipulation has emerged as a critical subdomain, where function-centric imitation, language grounding, and generative design support skill transfer across diverse household tasks~\cite{lin2025robotsmith, tang2025functo, chen2025tool, ren2023leveraging}.


\subsection{Agriculture}
Agriculture is an important yet highly challenging application domain for robotic manipulation, where robots must operate in unstructured environments characterized by dense canopies, variable lighting, irregular crop shapes, and the need for delicate handling. Recent works demonstrate progress across multiple crop types and farming conditions. For instance, robotic systems have been deployed for fruit and pepper harvesting in outdoor fields, showing the feasibility of autonomous harvesting under occlusion and cluttered backgrounds~\cite{subedi2025find,kim2025pepper,kim2025autonomous,li2025enhanced}. Other efforts address the safe manipulation of fragile bio-products, such as irregular poultry carcasses, by integrating customized grippers with learned control strategies~\cite{davar2025chicgrasp}. Beyond harvesting, new controllers have been designed for navigating dense plant canopies and adapting to complex interactions with foliage~\cite{parayil2025rice}. Together, these studies highlight the potential of robotics to enhance productivity, safety, and precision in agriculture, paving the way toward scalable automation in one of the most labor-intensive sectors.


\subsection{Industry}
In industrial contexts, robotic manipulation plays a crucial role in automating complex and large-scale processes such as assembly, logistics, and material handling. Early efforts emphasized enabling autonomous mobile manipulation in structured factory settings, laying the foundation for robots to navigate and interact in dynamic production environments~\cite{domel2017toward}. To support system design and deployment, modeling frameworks such as RobotML have been developed for simulating and validating industrial manipulation scenarios~\cite{kchir2016robotml}. More recent advances demonstrate how intelligent systems can enhance manufacturing flexibility, with reinforcement learning enabling adaptive assembly strategies that improve efficiency and reduce manual intervention~\cite{li2022flexible}. At the same time, specialized applications have emerged to address challenging settings, such as vision-based manipulation of transparent plastic bags, which are common in industrial packaging and logistics but difficult for traditional perception systems~\cite{adetunji2025vision}. Collectively, these applications illustrate how robotic manipulation is transitioning from fixed, rigid automation pipelines toward more adaptive, perception-driven systems capable of handling diverse tasks in real-world industrial environments.
It should be noted, however, that most learning-driven approaches are still evaluated in simulation or laboratory setups rather than on fully deployed factory lines, as industrial deployment demands strict reliability and safety, where rule-based systems remain the prevailing choice.


\subsection{AI4Science}
Robotic manipulation is increasingly being applied as a powerful enabler for scientific discovery, where precision, repeatability, and autonomy are critical. In medical science, robotic systems are advancing surgical assistance and minimally invasive procedures, ranging from autonomous intubation~\cite{tian2025learning}, capsule robot navigation~\cite{he2025capsdt}, and robotic spinal fixation~\cite{maroufi2025s3d}, to language-conditioned surgical planning~\cite{kim2025surgical, kim2025srt} and high-fidelity training simulators such as SonoGym for ultrasound-guided surgery~\cite{ao2025sonogym}. Beyond medicine, robotics also supports biology and life sciences, with platforms like RoboCulture~\cite{angers2025roboculture} enabling automated biological experimentation and robotic micromanipulation systems providing real-time spatiotemporal assistance in microscopy~\cite{mori2024real}.
In chemistry, the recently proposed robotic AI chemist~\cite{song2025multiagent} demonstrates how multi-agent robotic systems can autonomously conduct chemical experiments on demand, accelerating discovery by integrating automation with intelligent decision-making.
In aerospace, manipulation technologies extend to high-stakes environments, such as space assembly and in-orbit trajectory learning for robotic arms~\cite{mishra2025enhancing, shyam2020imitation}. More broadly, simulation frameworks like LabUtopia~\cite{li2025labutopia} establish standardized environments for training and benchmarking embodied scientific agents. Collectively, these applications highlight how robotics is becoming an essential tool in AI4Science, accelerating progress in medicine, biology, aerospace, and beyond.


\subsection{Art}
Robotic manipulation has also found applications in the artistic domain, where tasks such as music performance, calligraphy, drawing, and co-creative design showcase the expressive and demonstrative potential of embodied agents. In music, RP1M provides a large-scale motion dataset enabling robots to perform piano playing with bi-manual dexterous hands, highlighting how robotic systems can be trained to execute highly coordinated and nuanced actions beyond traditional industrial tasks~\cite{zhao2025rp1m}. In visual art, robotic calligraphy demonstrates how imitation learning can support the reproduction of culturally significant practices by planning precise brush trajectories in three-dimensional space~\cite{xie2023end, wang2023style}, while RoboCoDraw integrates GAN-based style transfer with time-efficient path optimization to allow robots to generate stylized portrait drawings~\cite{wang2020robocodraw}. Beyond performance, robotics has also been integrated into design and architecture through co-intelligent processes, where robots learn to translate design intent into executable construction paths, expanding their role as creative collaborators~\cite{buvs2024deepcraft}. Together, these studies illustrate how robotics can extend from functional manipulation to artistic expression, providing both a testbed for fine-grained motor control and a platform for human–robot collaboration in creative fields.


\subsection{Sports}
Robotic manipulation has also entered the domain of sports, where dynamic, high-speed interactions demand precise perception–action coordination. Recent advances demonstrate robots learning to perform complex athletic skills, such as legged manipulators executing coordinated badminton movements that couple locomotion with dexterous striking~\cite{ma2025learning}. In table tennis, robots have been trained to handle fast-paced rallies, from early efforts in sample-efficient reinforcement learning for controlled ball exchanges~\cite{tebbe2021sample} to more recent systems like SpikePingpong, which leverages spike-based vision sensors for real-time, high-frequency striking with enhanced precision~\cite{wang2025spikepingpong}. These applications not only showcase robotics as a platform for pushing the limits of real-time control and multimodal perception but also offer new opportunities for human–robot interaction, training, and performance augmentation in competitive sports.






==> sections/acknowledgments.tex <==
\section*{Acknowledgments}
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.

==> sections/biographynophoto.tex <==
\vspace{11pt}

\bf{If you include a photo:}

\vspace{-33pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}

\vfill

==> sections/header.tex <==
% The paper headers
% \markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2021}%
% {Shell \MakeLowercase{\textit{et al.}}: A Sample Article Using IEEEtran.cls for IEEE Journals}

% \IEEEpubid{0000--0000/00\$00.00~\copyright~2021 IEEE}

% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.

==> tables/3_benchmarks/cross_embodiment_simulator_benchmark.tex <==
\begin{table*}[t]
\centering
\caption{Summary of cross-embodiment Robotic manipulation benchmarks. S = segmentation, T = tactile sensing, and A = audio.}
\label{tab: cross_embodiment_simulator_benchmark}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Name} & \textbf{Year} & \textbf{Simulator} & \textbf{\#Objects} & \textbf{\#Tasks} & \textbf{\#Demos} & \textbf{Observation} & \textbf{\#Robot} & \textbf{Manip. Type} \\
\midrule
RoboSuite~\cite{zhu2020robosuite}     & 2020         & MuJoCo             & 20               & 9 tasks        & -              & RGB, D                & 10                        & Ba, Mo, Hu, Quad, Uni, Bi, Dex \\
CortexBench~\cite{majumdar2023we}   & NeurIPS 2023 & Multiple           & -                & 17 tasks & 850+      & RGB, D                & 6                         & Ba, Mo, Uni \\
RoboHive~\cite{kumar2023robohive}   & NeurIPS 2023 & Multiple           & -                & 17 tasks & 850+      & RGB, D                & 10+                         & Ba, Mo, Quad, Hu, Uni, Bi, Dex \\
ORBIT/Isaac Lab~\cite{mittal2023orbit} & RA-L 2023  & Isaac Sim          & -                & 5 types & -     & RGB, D, S             & 16                        & Ba, Mo, Hu, Uni, Bi, Dex \\
RoboCasa~\cite{nasiriany2024robocasa}      & RSS 2024     & MuJoCo/\cite{zhu2020robosuite}   & 2509             & 100 tasks      & 100K+           & RGB, D                & 4+                        & Ba, Mo, Hu, Quad, Uni, Bi, Dex \\
Genesis~\cite{genesis2024genesis}       & 2024         & Genesis Engine     & -                & -              & -              & RGB, D, T, A          & 6                         & Ba, Mo, Hu, Uni, Bi, Dex \\
ManiSkill3~\cite{tao2025maniskill3}    & RSS 2025     & SAPIEN             & 10K+             & 12 types  & 1M frames       & RGB, D, S             & 20+                       & Ba, Mo, Hu, Uni, Bi, Dex \\
AgentWorld~\cite{zhang2026agentworld}    & CoRL 2025     & Isaac Sim             & 9K             & -  & 1000+       & RGB, D             & 4                       & Mo, Hu, Uni, Bi, Dex \\
RoboVerse~\cite{geng2025roboverse}     & 2025         & MetaSim            & 5.5K             & 276 tasks      & 500K            & RGB, D                & 5                         & Ba, Mo, Hu, Uni, Bi, Dex \\
VIKI-Bench~\cite{kang2025viki}    & 2025         & \cite{nasiriany2024robocasa, tao2025maniskill3} & -             & 23,737 tasks   & -              & RGB, D                & 6                         & Ba, Mo, Hu, Uni, Bi, Dex \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/3_benchmarks/embodied_qa_and_affordance_dataset.tex <==
\begin{table*}[t]
\centering
\caption{Summary of embodied QA and affordance datasets.}
\label{tab: embodied_qa_and_affordance_datasets}
\vskip -0.05in
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc
>{\centering\arraybackslash}p{3.4cm}
>{\centering\arraybackslash}p{3.4cm}
>{\centering\arraybackslash}p{3.8cm}
}
\toprule
\textbf{Dataset} & \textbf{Year} & \textbf{Domain} & \textbf{Size} & \textbf{Visual Perception Tasks} & \textbf{Spatial Reasoning Tasks} & \textbf{Functional and Commonsense Reasoning Tasks} \\
\midrule
OpenEQA~\cite{majumdar2024openeqa} & CVPR 2024 & real & 1.6K & Object, Attribute and Object State Recognition & Object Localization, Spatial Reasoning & Functional Reasoning, World Knowledge \\
ManipVQA~\cite{huang2024manipvqa} & IROS 2024 & real + sim & 84K & Physically Grounded Understanding & Object Detection & -- \\
RefSpatial~\cite{zhou2025roborefer} & NeurIPS 2025 & real & 20M & - & Object Location, Orientation and Topological Reasoning & -- \\
ManipBench~\cite{zhao2025manipbench} & 2025 & real + sim & 12K+ & Keypoint Selection, Trajectory Understanding & Fabric Manipulation, Tool \& Drawer Contact & -- \\
PointArena~\cite{cheng2025pointarena} & 2025 & real & 982 & Pointing & Pointing & -- \\
Robo2VLM~\cite{chen2025robo2vlm} & 2025 & real & 684K+ & Scene Understanding, Multiple View & Object State, Spatial Relationship & Goal-conditioned Reasoning, Interaction Reasoning \\
PAC Bench~\cite{gundawar2025pac} & 2025 & real + sim & 30K+ & Properties & Constraints & Affordance \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/3_benchmarks/grasping_dataset.tex <==

\begin{table*}[t]
\centering
\caption{Summary of grasping datasets.}
\label{tab: grasping_datasets}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Dataset} & \textbf{Year} & \textbf{Grasp Type} & \textbf{Scene} & \textbf{\#Objects} & \textbf{Domain} & \textbf{Size} & \textbf{Visual Modality} & \textbf{w/ Language} \\
\midrule
Cornell~\cite{jiang2011efficient} & ICRA 2011 & rect. & single object & 240 & real & 1035 images, 8019 grasps & RGB-D & $\times$ \\
Jacquard~\cite{depierre2018jacquard} & IROS 2018 & rect. & single object & 11k & sim & 54k images, 1.1M grasps & RGB-D & $\times$ \\
GraspNet~\cite{fang2020graspnet} & CVPR 2020 & 6-DoF & cluttered & 88 & real & 97,280 images, $\sim$1.2B grasps & RGB-D & $\times$ \\
ACRONYM~\cite{eppner2021acronym} & ICRA 2021 & 6-DoF & multi-object & 8872 & sim & 17.7M grasps & RGB-D & $\times$ \\
Regrad~\cite{zhang2022regrad} & RA-L 2022 & rect. $\&$ 6-DoF & multi-object & 50K & sim & 1.02K images, 100M grasps & RGB-D & $\times$ \\
MetaGraspNet~\cite{gilles2022metagraspnet} & CASE 2022 & 6-DoF & cluttered & - & sim + real & 217k (sim) + 2.3k (real) images & RGB-D & $\times$ \\
Dexgraspnet~\cite{wang2023dexgraspnet} & ICRA 2023 & 6-DoF & single-object & 5355 & sim & 1.32M grasps & - & $\times$ \\
MetaGraspNet-V2~\cite{gilles2023metagraspnetv2} & TASE 2023 & 6-DoF & cluttered & - & sim + real & 296k (sim) + 3.2k (real) images & RGB-D & $\times$ \\
Grasp-Anything~\cite{vuong2024grasp} & ICRA 2024 & rect. & multi-object & 3M & syn & 1M images, $\sim$600M grasps & RGB & $\checkmark$ \\
Grasp-Anything++~\cite{vuong2024language} & CVPR 2024 & rect. & multi-object & 3M & syn & 1M images, 10M grasps & RGB & $\checkmark$ \\
Grasp-Anything-6D~\cite{jiang2011efficient} & ECCV 2024 & 6-DoF & multi-object & 3M & syn & 1M images, 200M grasps & RGB-D & $\checkmark$ \\
Dex1B~\cite{ye2025dex1b} & RSS 2025 & dexterous & single object & 1B & sim & 1B grasps & PC & $\times$ \\
GraspClutter6D~\cite{nguyen2024graspanything6d} & 2025 & 6-DoF & cluttered & 200 & real & 52K images, 9.3B grasps & RGB-D & $\times$ \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/3_benchmarks/learning_vs_non-learning.tex <==
\begin{table*}[t]
\centering
\caption{Comparison between non-learning and learning-based methods for grasping and manipulation. Here, grasping specifically refers to grasp detection and generation.}
\label{tab: method_comparison}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\textbf{Mani. Type} & \textbf{Control Type} & \textbf{Pose Generation} & \textbf{Trajectory Generation} & \textbf{Generalization} & \textbf{Interpretability \& Stability} \\
\midrule
\multirow{2}{*}{Grasping} 
  & Non-learning & Analytical: geometric rules, force-closure analysis & IK + motion planning & Low  & High \\
  & Learning      & Learned from data                                & IK + motion planning & High & Low  \\
\midrule
\multirow{2}{*}{Manipulation} 
  & Non-learning & Task-specific or predefined goal pose             & IK + motion planning & Low  & High \\
  & Learning      & Learned implicitly via RL or IL & Learned policies via RL or IL & High & Low \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/3_benchmarks/manipulation_simultor_benchmark.tex <==
\begin{table*}[t]
\centering
\caption{Summary of robot manipulation simulators and benchmarks. 
All benchmarks provide proprioceptive or pose observations by default, and most include additional modalities. 
% D denotes depth, S denotes segmentation, T denotes tactile sensing, P denotes particle-based state representations, and N denotes surface normals.
% Ba refers to basic manipulation, De to deformable object manipulation, Dex to dexterous manipulation, Mo to mobile manipulation, and Hu to humanoid manipulation. 
% Uni indicates single-arm settings, while Bi denotes bimanual configurations.
}
\label{tab: manipulation_simulator_benchmark}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\textbf{Name} & \textbf{Year} & \textbf{Simulator} & \textbf{\#Objects} & \textbf{\#Tasks} & \textbf{\#Demos} & \textbf{Observation} & \textbf{Robot Type} & \textbf{Mani. Type} \\
\midrule
MetaWorld~\cite{yu2020meta} & CoRL 2019 & MuJoCo & 80 & 50 & - & Pose & Sawyer & Ba, Uni \\
Franka Kitchen~\cite{gupta2020relay} & CoRL 2020 & MuJoCo & 10 & 7 & 513 & Pose & Franka Panda & Ba, Uni \\
RLBench~\cite{james2020rlbench} & RA-L 2020 & CoppeliaSim & 28 & 100 & - & RGB, D, S & Franka Panda & Ba, Uni \\
CALVIN~\cite{mees2022calvin} & RA-L 2021 & Pybullet & 28 & 34 & 40M & RGB, D & Franka Panda & Ba, Uni \\
Robomimic~\cite{mandlekar2022matters} & CoRL 2021 & MuJoCo & 15 & 8 & 6K & RGB, D & Franka Panda & Ba, Uni \\
Maniskill~\cite{mu2maniskill} & NeurIPS 2021 & SAPIEN & 100+ & 4 & 30K+ & RGB, D, S & Franka Panda & Ba, Uni \\
VLMbench~\cite{zheng2022vlmbench} & NeurIPS 2022 & CoppeliaSim/\cite{james2020rlbench} & 22 & 8 & 6K+ & RGB, D, S & Franka Panda & Ba, Uni \\
Maniskill2~\cite{gumaniskill2} & ICLR 2023 & SAPIEN & 2144 & 20 & 30K+ & RGB, D, S & Franka Panda & Ba, Mo, Uni, Bi \\
VIMA-Bench~\cite{jiang2022vima} & ICML 2023 & Pybullet/Ravens & 100+ & 17 & 600K+ & RGB, D, S & UR5 & Ba, Uni \\
ARNOLD~\cite{gong2023arnold} & ICCV 2023 & Isaac Sim & 40 & 8 & 10K+ & RGB, D, S & Franka Panda & Ba, Uni \\
LIBERO~\cite{liu2023libero} & NeurIPS 2023 & MuJoCo/\cite{zhu2020robosuite} & 67 & 130 & 6.5K & RGB, D & Franka Panda & Ba, Uni \\
COLOSSEUM~\cite{pumacay2024colosseum} & RSS 2024 & CoppeliaSim/\cite{james2020rlbench} & - & 20 & 2K & RGB, D & Franka Panda & Ba, Uni \\
SimplerEnv~\cite{li2025evaluating} & CoRL 2024 & SAPIEN & - & 10 & Bridge v2 & RGB, D & Google Robot, WidowX & Ba, Uni \\
GenSim2~\cite{hua2025gensim2} & CoRL 2024 & SAPIEN & 200 & 100 & - & RGB, D & Franka Panda & Ba, Uni \\
GemBench~\cite{garcia2025towards} & ICRA 2025 & CoppeliaSim & 20+ & 60 & - & RGB, D & Franka Panda & Ba, Uni \\
RoboTwin~\cite{mu2025robotwin} & CVPR 2025 & SAPIEN/\cite{tao2025maniskill3} & 10+ & - & 320 & RGB, D, S & Aloha-AgileX & Ba, Bi \\
GENMANIP~\cite{gao2025genmanip} & CVPR 2025 & Isaac Sim & 10K & 200 & 200K & RGB, D, S & Franka Panda & Ba, Uni \\
VLABench~\cite{zhang2024vlabench} & 2024 & MuJoCo & 2000+ & 100 & 5K & RGB, D & Franka Panda & Ba, Uni \\
AGNOSTOS~\cite{zhou2025agnostos} & 2025 & CoppeliaSim/\cite{james2020rlbench} & - & 41 & 3.6K & RGB, D, S & Franka Panda & Ba, Uni \\
RoboTwin 2~\cite{chen2025robotwin} & 2025 & SAPIEN/\cite{tao2025maniskill3} & 731 & 50 & 100K & RGB, D, S & Aloha, UR5, Franka, ARX-X5 & Ba, Uni, Bi \\
ROBOEVAL~\cite{wang2025roboeval} & 2025 & - & - & 8 & 3K+ & RGB, D & Franka Panda & Ba, Bi \\
INT-ACT~\cite{fang2025intention} & 2025 & SAPIEN/\cite{li2025evaluating} & - & 50 & Bridge v2 & RGB, D & Franka Panda & Ba, Uni \\
\midrule
TacSL~\cite{akinola2025tacsl} & T-RO 2025 & Isaac Gym & - & 3 & - & RGB, D, T & Franka Panda & Ba, Uni \\
ManiFeel~\cite{luu2025manifeel} & 2025 & Isaac Gym/\cite{akinola2025tacsl} & - & 6 & - & RGB, D, T & Franka Panda & Ba, Uni \\
\midrule
\cite{rajeswaran2018learning} & RSS 2018 & MuJoCo & - & 4 & 100 & RGB, D, T & ADROIT Hand & Dex, Uni \\
TriFinger~\cite{wuthrich2021trifinger} & CoRL 2021 & PyBullet & - & 2 & - & RGB & 3-DoF Hand & Dex, Uni \\
\midrule
PlasticineLab~\cite{huang2021plasticinelab} & ICLR 2021 & Taichi + DiffTaichi & 1 & 10 & - & RGB, D, P & Rigid End-Effector & De \\
SoftGym~\cite{lin2021softgym} & CoRL 2021 & NVIDIA FleX & 4 & 10 & - & RGB, D, P & Sawyer, Franka & De, Uni \\
DaXBench~\cite{chen2023daxbench} & ICLR 2023 & DaX & 4 & 9 & - & RGB, D, P & - & De \\
\midrule
ManipulaTHOR~\cite{ehsani2021manipulathor} & CVPR 2021 & Unity/AI2-THOR & 2.6K+ & - & - & RGB, D, N & Kinova Gen3 on Mobile Base & Mo, Uni \\
HomeRobot~\cite{yenamandra2023homerobot} & CoRL 2023 & AI Habitat & 7892 & - & - & RGB, D & Hello Robot Stretch & Mo, Uni \\
BEHAVIOR-1K~\cite{li2023behavior} & CoRL 2023 & OmniGibson & 5215 & 1K & - & RGB, D & Mobile Manipulator & Mo, Uni \\
\midrule
ODYSSEY~\cite{wang2025odyssey} & 2025 & Isaac Sim & 105 & 12 & - & RGB & 3-DoF Hand & Quad, Uni \\
\midrule
BiGym~\cite{chernyadev2025bigym} & CoRL 2024 & MuJoCo & 10+ & 40 & 2K & RGB, D & Unitree H1 & Hu, Bi \\
HumanoidBench~\cite{sferrazza2024humanoidbench} & 2024 & MuJoCo & ~15 & 27 & - & RGB, LiDAR & Unitree H1 + Shadow-Hand & Hu, Bi, Dex \\
HumanoidGen~\cite{jing2025humanoidgen} & 2025 & SAPIEN & - & 20 & - & RGB, D & Unitree & Hu, Bi, Dex \\
\bottomrule
\end{tabular}
}
\\[1ex]
\hfill {\footnotesize D = depth, S = segmentation, T = tactile sensing, P = particle-based state representations, N = normals}
\\[0ex]
\hfill {\footnotesize Ba = basic, De = deformable object, Dex = dexterous, Mo = mobile, Quad = quadrupedal, Hu = humanoid manipulation}
\\[0ex]
\hfill {\footnotesize Uni = single arm, Bi = bimanual arms}
\end{table*}


==> tables/3_benchmarks/trajectory_dataset.tex <==
\begin{table*}[ht]
\centering
\caption{Summary of trajectory datasets.}
\label{tab: trajectory_datasets}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Dataset} & \textbf{Year} & \textbf{Domain} & \textbf{\#Demos} & \textbf{\#Verb} & \textbf{Robot Type} & \textbf{Observation} \\
\midrule
MINE~\cite{sharma2018multiple} & CoRL 2018 & real & 8.3k & 20 & Baxter Robot & RGB, D \\
BridgeData~\cite{ebert2021bridge} & 2021 & real & 7.2k & 4 & WidowX250 & RGB, D \\
BC-Z~\cite{jang2022bc} & CoRL 2021 & real & 26k & 3 & Google Robot & RGB \\
RT-1~\cite{brohan2023rt} & RSS 2023 & real & 130k & 2 & Google Robot & RGB, D \\
RH20T~\cite{fang2023rh20t} & RSSW 2023 & real & 110k & 33 & Flexiv, UR5, Franka & RGB, D, T \\
BridgeData V2~\cite{walke2023bridgedata} & CoRL 2023 & real & 60.1k & 24 & WidowX 250 & RGB, D \\
RoboSet~\cite{bharadhwaj2024roboagent} & ICRA 2024 & real & 98.5k & 11 & Franka Panda & RGB, D \\
Open X-Embodiment~\cite{o2024open} & ICRA 2024 & real & 1.4M & 217 & 22 Embodiments & RGB, D \\
DROID~\cite{khazatsky2024droid} & RSS 2024 & real & 76k & 86 & Franka Panda & RGB, D \\
AgiBot World Dataset~\cite{bu2025agibot} & IROS 2025 & real & 1M+ & 87 &	Agibot & RGB, D, T \\
ARIO~\cite{wang2024all} & 2024 & real + sim & 3M & 20 & AgileX, UR5, Cloud Ginger XR-1 & RGB, D, T, A \\
RoboMind~\cite{wu2024robomind} & 2024 & real & 107k & 38 & Franka Panda, Tien Kung, AgileX, UR5 & RGB, D \\
RoboFAC~\cite{lu2025robofac} & 2025 & sim (SAPIEN/ManiSkill) & 9.44k & 12 & Franka Panda & RGB, D \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/4_manipulation_tasks/manipulation_tasks_2.tex <==
\begin{table*}[t]
\centering
\caption{Representative methods across manipulation types and learning paradigms.}
\label{tab: manipulation_methods}
\vskip -0.05in
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Mani. Type & RL & IL & RL+IL & VLA \\
\midrule
Basic & See Table~\ref{tab: rl} & See Figure~\ref{fig: il} & See Table~\ref{tab: rl-il} & See Figure~\ref{fig: vla-taxonomy} \\
Dexterous & PDDM~\cite{nagabandi2020deep}, \cite{rajeswaran2018learning}, \cite{zhu2019dexterous} & DexHandDiff~\cite{liang2025dexhanddiff}, CordViP~\cite{fu2025cordvip} & REBOOT~\cite{hu2023reboot}, ViViDex~\cite{chen2025vividex} & OFA~\cite{li2025object}, LBM~\cite{barreiros2025careful} \\
Soft Robotics & \cite{thuruthel2018model}, \cite{li2022towards} & Soft DAgger~\cite{nazeer2023soft}, KineSoft~\cite{yoo2025kinesoft} & SS‑ILKC~\cite{meng2025sensor} & -- \\
Deformable Object & \cite{matas2018sim} & DeformerNet~\cite{hu20193}, DexDeform~\cite{li2023dexdeform} & DMfD~\cite{salhotra2022learning} &
-- \\
Mobile & \cite{wu2020spatial}, MoMa~\cite{hu2023causal} & MOMA-Force~\cite{yang2023moma}, Skill Transformer~\cite{huang2023skill} & \cite{xiong2024adaptive} & MoManipVLA~\cite{wu2025momanipvla} \\
Quadrupedal & VBC~\cite{liu2025visual}, GAMMA~\cite{zhang2024gamma} &
Human2LocoMan~\cite{niu2025human2locoman} & \cite{he2024learning}, WildLMa~\cite{qiu2024wildlma} & QUAR-VLA~\cite{ding2024quar}, GeRM~\cite{song2024germ} \\
Humanoid & \cite{xie2023hierarchical}, FLAM~\cite{zhang2025flam} & OmniH2O~\cite{he2025omnih2o}, iDP3~\cite{ze2025generalizable} & \cite{schakkal2025hierarchical} & GR00T N1~\cite{bjorck2025gr00t}, Humanoid-VLA~\cite{xu2024humanvla} \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/6_low-level_controller/il.tex <==
% --- TikZ 和 Forest 样式定义 ---
\tikzset{
    my-box/.style={
        rectangle,
        draw=black,
        rounded corners,
        text opacity=1,
        minimum height=1.5em,
        minimum width=5em,
        inner sep=2pt,
        align=center,
        fill opacity=.5,
    },
    leaf-lfa/.style={
        my-box, 
        fill=yellow!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    },
    leaf-lfo/.style={
        my-box, 
        fill=hidden-blue!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    },
    leaf-summary/.style={
        my-box, 
        fill=yellow!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    }
}

\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}
{
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\large,
            rectangle,
            draw=black,
            rounded corners,
            align=center,
            minimum width=4em,
            edge+={darkgray, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=4pt,
            line width=1.1pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center, inner xsep=5pt},
        },
        where level=1{text width=12em, font=\normalsize, align=center, inner xsep=5pt, inner ysep=3pt}{},
        where level=2{text width=12em, font=\normalsize, align=left, inner xsep=4pt}{},
        where level=3{text width=11em, font=\normalsize, align=left, inner xsep=5pt}{},
        where level=4{font=\normalsize, align=left}{},
[{Imitation Learning Methods (\S\ref{subsubsec: il})}, ver
    % ======================= 2D =======================
    [{Imitation Learn from Action}, ver
        [{Action-level IL}
            [{BC from Action}
                [{\eg \cite{xie2020deep}, Data Scaling Laws~\cite{lin2025data}, BC-Z~\cite{jang2022bc}, Most of VA/VLA/TVLA, Diffusion Policies, \textit{etc}}, leaf-lfa]
            ]
            [{BC from Pose}
                [{\eg PoseInsert~\cite{sun2025exploring}, ZeroMimic~\cite{shi2025zeromimic}, RiEMann~\cite{gao2025riemann}}, leaf-lfa]
            ]
            [{MP-based IL}
                [{\eg \cite{schaal2003computational}, \cite{ijspeert2013dynamical}, \cite{paraschos2013probabilistic}, \cite{tanwani2018generalizing}, \cite{perico2019combining}, \cite{wang2020framework}, \cite{paolillo2023dynamical}}, leaf-lfa]
            ]
            [{Search-based IL}
                [{\eg \cite{billard2004discovering}, \cite{ratliff2009learning},  \cite{mcdonald2022guided}, \cite{duan2024structured}, SAILOR~\cite{jain2025smooth}}, leaf-lfa]
            ]
            [{Optimization-based IL}
                [{\eg \cite{mronga2021learning}, \cite{dhonthi2022optimizing}, Leto~\cite{xu2024leto}, NODE-IL~\cite{zhao2024neural}, SCDS~\cite{abyaneh2025contractive}}, leaf-lfa]
            ]
        ]
        [{Reward-based IL}
            [{Inverse Reinforcement\\ Learning}
                [{\eg Inverse KKT~\cite{englert2017inverse}, SPRINQL~\cite{hoang2024sprinql}, \cite{ghasemipour2020divergence}}, leaf-lfa]
            ]
            [{Adversarial Imitation\\ Learning}
                [{\eg GAIL~\cite{ho2016generative}, Option-GAIL~\cite{jing2021adversarial}, LAPAL~\cite{wang2022latent}, DRAIL~\cite{lai2024diffusion}, OLLIE~\cite{yue2024ollie}, C-LAIfO~\cite{giammarino2024visually}}, leaf-lfa]
            ]
        ]
        [{Representation Learning\\ for IL}
            [{Latent Learning for IL}
                [{\eg \cite{zeestraten2017approach}, \cite{tamar2018imitation}, TRAIL~\cite{zolna2021task}, MCNN~\cite{sridhar2024memory}, BC-IB~\cite{bai2025rethinking}}, leaf-lfa]
            ]
            [{In-Context Imitation\\ Learning}
                [{\eg \cite{dasari2021transformers}, \cite{vosylius2023few}, ICRT~\cite{fu2024context}, Instant Policy~\cite{vosylius2025instant}, Robust Instant Policy~\cite{oh2025robust}}, leaf-lfa]
            ]
        ]
        [{Interactive IL}
            [{\cite{muhlig2012interactive}, IWR~\cite{mandlekar2020human}, TIPS~\cite{chisari2022correct}, Sirius~\cite{liu2022robot}, LILAC~\cite{cui2023no}, HITL-TAMP~\cite{mandlekar2023human}, Chg-dagger~\cite{takahashi2024chg}}, leaf-lfa]
        ]
        [{Robustness and Efficiency}
            [{Robustness}
                [{\eg Dart~\cite{laskey2017dart}, \cite{valletta2021imitation}, \cite{oh2023bayesian}, Counter-BC~\cite{sagheb2025counterfactual}, ADC~\cite{huang2025adversarial}, CCIL~\cite{ke2024ccil}, CREST~\cite{lee2021causal}, RAIL~\cite{jung2025rail}, \\ FAIL-Detect~\cite{xu2025can}}, leaf-lfa]
            ]
            [{Efficiency}
                [{\eg \cite{lin2022efficient}, TEDA~\cite{ge2024bridging},  SRIL~\cite{xie2024subconscious}, DemoSpeedup~\cite{guo2025demospeedup}, SAIL~\cite{arachchige2025sail}}, leaf-lfa]
            ]
        ]
    ]
    % ======================= 3D =======================
    [{Imitation from Observation}, ver
        [{Reward or Occupancy\\ Recovery from Observation}
            [{HOLD~\cite{alakuijala2023learning}, ADS~\cite{liu2024imitation}, DIFO ~\cite{huang2024diffusion}}, leaf-lfo]
        ]
        [{State or Representation\\ Alignment and Matching}
            [{\cite{chella2006cognitive}, \cite{sieb2020graph}, SILO~\cite{lee2020follow}, VGS-IL~\cite{jin2020geometric},   WHIRL~\cite{bahl2022human}, ZeST~\cite{cui2022can}, \cite{huang2023nift}, VIP~\cite{ma2023vip}, LIV~\cite{ma2023liv}, \cite{sikchi2025dual}}, leaf-lfo]
        ]
        [{Model- and\\ Physics-Grounded LfO}
            [{\cite{chen2023imitation}, Diff-LfD~\cite{zhu2023diff}, MimicFunc~\cite{tang2026mimicfunc}}, leaf-lfo]
        ]
        [{BC from Observation\\ and Goal-driven LfO}
            [{CNet~\cite{yang2019learning}, \cite{huang2020motion}, \cite{liang2022learning}, \cite{bharadhwaj2023zero}, \cite{kim2023giving}, Point Policy\cite{haldar2025point}}, leaf-lfo]
        ]
    ]
]
    \end{forest}
}
\caption{A structured taxonomy of IL methods.}
\label{fig: il}
\end{figure*}

==> tables/6_low-level_controller/model_free_rl.tex <==
\begin{table}[t]
\footnotesize
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3.0pt}
\caption{Representative RL methods for manipulation tasks.}
\label{tab: rl}
\begin{tabular}{ll}
\toprule
\textbf{Category} & \textbf{Representative Methods} \\
\midrule
 Pre-Training & QT-Opt~\cite{dmitry2018qt}, PTR~\cite{kumar2022pre}, V-PTR~\cite{bhateja2023robotic}\\

Fine-Tuning & Residual RL~\cite{johannink2019residual}, RLDG~\cite{xu2024rldg}, V-GPS~\cite{nakamoto2025steering}, PA-RL~\cite{mark2024policy}\\

VLA-RL & iRe-VLA~\cite{guo2025improving}, RIPT~\cite{tan2025interactive}, VLA-RL~\cite{lu2025vla}, ConRFT~\cite{chen2025conrft}\\
\bottomrule
\end{tabular}
\end{table}


==> tables/6_low-level_controller/policy.tex <==
% --- TikZ 和 Forest 样式定义 ---
\tikzset{
    my-box/.style={
        rectangle,
        draw=black,
        rounded corners,
        text opacity=1,
        minimum height=1.5em,
        minimum width=5em,
        inner sep=2pt,
        align=center,
        fill opacity=.5,
    },
    leaf-2d/.style={
        my-box, 
        fill=yellow!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    },
    leaf-3d/.style={
        my-box, 
        fill=hidden-blue!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    },
    leaf-summary/.style={
        my-box, 
        fill=yellow!32, 
        text=black,
        font=\normalsize,
        inner xsep=5pt,
        inner ysep=4pt,
        align=left,
        text width=45em,
    },
    category/.style={
      text width=27mm,
      align=left,
    }
}

\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{forest}
        forked edges,
        for tree={
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,
            child anchor=west,
            base=left,
            font=\large,
            rectangle,
            draw=black,
            rounded corners,
            align=center,
            minimum width=4em,
            edge+={darkgray, line width=1pt},
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=4pt,
            line width=1.1pt,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center, inner xsep=5pt},
        },
        where level=1{text width=10em, font=\normalsize,align=center, inner xsep=5pt, inner ysep=3pt}{},
        where level=2{text width=7em, font=\normalsize, align=left, inner xsep=3pt}{},
        where level=3{text width=30em, font=\normalsize, align=left, inner xsep=5pt}{},
        where level=4{font=\normalsize, align=left}{},
[{Policy Learning (\S\ref{subsec: policy_learning})}, ver
    % ======================= 2D =======================
    [{MLP-based Policy}
            [{R3M~\cite{nair2023r3m},VC-1~\cite{majumdar2023we},RPT~\cite{radosavovic2023real}, RoboAct-Clip~\cite{zhang2025roboact}, DyWA~\cite{lyu2025dywa}}, leaf-2d]
        ]
        [{Transformer-based Policy}, ver
            [{ACT-based Policy}, category
                [{ACT~\cite{zhao2023learning}, RoboAgent~\cite{bharadhwaj2024roboagent}, Bi-ACT~\cite{gao2024bi}, BAKU~\cite{haldar2024baku}, InterACT~\cite{lee2024interact}, Haptic-ACT~\cite{li2024haptic}, \\ALOHA Unleashed~\cite{zhao2024aloha}, Bi-LAT~\cite{kobayashi2025bi}, Chain-of-Action~\cite{pan2024chain}, Q-chunking~\cite{li2025reinforcement}}, leaf-2d]
            ]
            [{Autoregressive \\Policy}, category
                [{Act3D~\cite{gervet2023act3d}, ICRT~\cite{fu2024context}, CARP~\cite{gong2024carp}, Dense Policy~\cite{su2025dense}, HAT~\cite{qiu2025humanoid}, RVT~\cite{goyal2023rvt}, DP3~\cite{ze2024generalizable}, iDP3~\cite{ze2024generalizable}, \\ 3D-MVP~\cite{qian20243d}}, leaf-2d]
        ]
        ]
    [{Diffusion Policy}
        [{Diffusion Policy~\cite{chi2023diffusion}, DP3~\cite{ze20243d}, SDP~\cite{wang2025sparse}, ManiCM~\cite{lu2024manicm}, DPPO~\cite{ren2024diffusion}, EquiBot~\cite{yang2025equibot}, EDP~\cite{wang2025equivariant}, \\MBA~\cite{su2025motion}, OneDP~\cite{wang2024one}, Consistency Policy~\cite{prasad2024consistency}, G3Flow~\cite{chen2025g3flow}, 
        RoboDual~\cite{bu2024towards}, DP-Attacker~\cite{chen2024diffusion}, \\HDP~\cite{ma2024hierarchical}, DP4~\cite{liu2025spatial}, H\textsuperscript{3}DP~\cite{lu2025h}, Past-Token~\cite{torne2025learning}, UVA~\cite{li2025unified}, UWM~\cite{zhu2025unified}, RDP~\cite{xue2025reactive}}, leaf-2d]
    ]
    [{Flow Matching Policy}
        [{AdaFlow~\cite{hu2024adaflow}, Affordance FM~\cite{zhang2024affordance}, PointFlowMatch~\cite{chisari2024learning}, FlowPolicy~\cite{zhang2025flowpolicy}, X-IL~\cite{jia2025x}, \\FLOWER~\cite{reuss2025flower}, Streaming Flow Policy~\cite{jiang2025streaming}, 
        RTC~\cite{black2025real}, FlowRAM~\cite{wang2025flowram}, MP1~\cite{sheng2025mp1}, H-RDT~\cite{bi2025hrdt}, \\VFP~\cite{zhai2025vfp}, GenFlowRL~\cite{yu2025genflowrl}, 3D FlowMatch Actor~\cite{zhi20253dflowaction}}, leaf-2d]
        ]
    [{SSM-based Policy}
    [{MaIL~\cite{jia2024mail}, RoboMamba~\cite{liu2024robomamba}, FlowRAM~\cite{wang2025flowram}, Mamba as Motion Encoder, MTIL~\cite{zhou2025mtil}}, leaf-2d]
        ]
    [{SNN-based Policy}
    [{SDP~\cite{hou2024sdp}, STMDP~\cite{wang2024brain}, Multimodal SNN~\cite{zhang2025multimodal}, Fully Spiking A2C~\cite{zhang2025fully}}, leaf-2d]
        ]
    [{Frequency-based Policy}
    [{Fourier Transporter~\cite{huang2024fourier}, FreqPolicy~\cite{zhong2025freqpolicy}, Wavelet Policy~\cite{huang2025wavelet}}, leaf-2d]
        ]
]
    \end{forest}
}
\caption{A structured overview of policy learning for visuomotor control, organized by modeling paradigm.}
\label{fig: policy_learning}
\end{figure*}

==> tables/6_low-level_controller/rl-il.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Representative methods combining RL and IL for manipulation tasks.}
% \label{table:rl-il}
% \begin{tabular}{ll}
% \toprule
% \textbf{Category} & \textbf{Representative Methods} \\
% \midrule
% Methods support for RL and IL & Frame Mining~\cite{liu2023frame}, Dual RL~\cite{sikchi2024dualrl},  \\
% IL Pre-training + RL Fine-tuning & \cite{pastor2011skill}, SkiLD~\cite{pertsch2021guided}, FERM~\cite{zhan2021framework}, Q-attention~\cite{james2022q}, CSIL~\cite{watson2023coherent}, PLANRL~\cite{bhaskar2024planrl}, HIL-SERL~\cite{luo2025precise}, Sketch-to-Skill~\cite{yu2025sketch}  \\
% RL Pre-training + IL Fine-tuning & MoPA-PD~\cite{liu2022distilling}, \cite{lee2022spend} \\
% Reward Shaping from IL & MaxEnt IOC~\cite{finn2016guided}, \cite{brown2020better}, ~\cite{liu2018imitation}, LbW~\cite{xiong2021learning}, ~\cite{lee2021generalizable}, ~\cite{haldar2023watch}, RoboCLIP~\cite{sontakke2023roboclip}, IRIS~\cite{mandlekar2020iris}, ORIL~\cite{zolna2020offline}, ~\cite{zhu2018reinforcement}, ResiP~\cite{ankile2024imitation}, ORCA~\cite{huey2025imitation}, Concept2Robot~\cite{shao2021concept2robot} \\
% Joint Optimization & \cite{jena2021augmenting}, AW-Opt~\cite{lu2022aw}, \cite{mosbach2022accelerating}, IN-RIL~\cite{gao2025ril} \\
% In-Context RL & DCRL~\cite{dance2021conditioned} \\
% \bottomrule
% \end{tabular}
% \end{table*}


\begin{table*}[ht]
\centering
\caption{Representative methods combining RL and IL for manipulation tasks.}
\label{tab: rl-il}
\begin{tabular}{lp{0.75\textwidth}} % 第二列固定宽度
\toprule
\textbf{Category} & \textbf{Representative Methods} \\
\midrule
Methods support for RL and IL & Frame Mining~\cite{liu2023frame}, Dual RL~\cite{sikchi2024dualrl} \\
IL Pre-training + RL Fine-tuning & \cite{pastor2011skill}, SkiLD~\cite{pertsch2021guided}, FERM~\cite{zhan2021framework}, Q-attention~\cite{james2022q}, CSIL~\cite{watson2023coherent}, PLANRL~\cite{bhaskar2024planrl}, HIL-SERL~\cite{luo2025precise}, Sketch-to-Skill~\cite{yu2025sketch} \\
RL Pre-training + IL Fine-tuning & MoPA-PD~\cite{liu2022distilling}, \cite{lee2022spend} \\
Reward Shaping from IL & MaxEnt IOC~\cite{finn2016guided}, \cite{brown2020better}, \cite{liu2018imitation}, LbW~\cite{xiong2021learning}, \cite{lee2021generalizable}, \cite{haldar2023watch}, RoboCLIP~\cite{sontakke2023roboclip}, IRIS~\cite{mandlekar2020iris}, ORIL~\cite{zolna2020offline}, \cite{zhu2018reinforcement}, ResiP~\cite{ankile2024imitation}, ORCA~\cite{huey2025imitation}, Concept2Robot~\cite{shao2021concept2robot} \\
Joint Optimization & \cite{jena2021augmenting}, AW-Opt~\cite{lu2022aw}, \cite{mosbach2022accelerating}, IN-RIL~\cite{gao2025ril} \\
In-Context RL & DCRL~\cite{dance2021conditioned} \\
\bottomrule
\end{tabular}
\end{table*}



==> tables/6_low-level_controller/rl.tex <==
\begin{table*}[ht]
\centering
\caption{Representative RL methods for manipulation tasks.}
\label{tab: rl}
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{Subcategory} & \textbf{Representative Methods} \\
\midrule
\multirow{3}{*}{\textbf{Model-Free RL}}
    & Pre-Training & QT-Opt~\cite{dmitry2018qt}, PTR~\cite{kumar2022pre}, V-PTR~\cite{bhateja2023robotic}\\
\multirow{3}{*}{}
    & Fine-Tuning & Residual RL~\cite{johannink2019residual}, RLDG~\cite{xu2024rldg}, V-GPS~\cite{nakamoto2025steering}, PA-RL~\cite{mark2024policy}\\
\multirow{3}{*}{}
    & VLA-RL & iRe-VLA~\cite{guo2025improving}, RIPT~\cite{tan2025interactive}, VLA-RL~\cite{lu2025vla}, ConRFT~\cite{chen2025conrft}\\
\midrule
\multirow{3}{*}{\textbf{Model-Based RL}}
    & Imagination Trajectory Generation & Dreamer~\cite{hafner2020dream}, MWM~\cite{seo2023masked}\\
\multirow{3}{*}{}
    & Planning & GPS~\cite{levine2013guided}, TD-MPC~\cite{hansen2022temporal}\\
\multirow{3}{*}{}
    & Differentiable RL & SAPO~\cite{xing2025stabilizing}, SAM-RL~\cite{lv2023sam}, DiffTORI~\cite{wan2024difftori}\\
\bottomrule
\end{tabular}
\end{table*}


==> tables/7-bottlenecks/data.tex <==
% ===== DATA mind map (filled, compact) =====
% ===== DATA taxonomy (orthogonal edges + colored category blocks) =====

\definecolor{cjyBlue}{HTML}{87CEFA}   % 十六进制 HEX
\definecolor{cjyOrange}{HTML}{FF7F0E}
\definecolor{cjyGreen}{HTML}{8FBC8F}
\definecolor{cjyPurple}{HTML}{9467BD}
\begin{figure*}[t]
\centering
\scriptsize

\forestset{
  taxo/.style={
    for tree={
      grow'=0,
      parent anchor=east,
      child anchor=west,
      anchor=west,
      % forked edges,              % ← 开启分叉
      % fork sep=3pt,              % ← 分叉与主干之间的间隔
     edge path'={(!u.parent anchor) -- +(3pt,0) |- (.child anchor)},
      edge={draw, line width=0.6pt},
      rounded corners,
      draw,
      minimum height=4mm,
      inner xsep=4pt,
      inner ysep=2pt,
      s sep=3pt,
      l sep=6pt,
      align=left,
      font=\scriptsize
    },
    cat/.style={draw, rounded corners=2pt, minimum height=5mm, minimum width=15mm,
                 align=center, font=\bfseries},
    catBlue/.style={cat, fill=cjyBlue},
    catOrange/.style={cat, fill=orange!85!black},
    catGreen/.style={cat, fill=cjyGreen},
    catPurple/.style={cat, fill=purple!70!black},
    sub_1/.style={draw, rounded corners=2pt, fill opacity=.5, text width=22mm, inner sep=4pt},
    sub/.style={draw, rounded corners=2pt, fill=hidden-blue!32, fill opacity=0.5, text width=36mm, inner sep=4pt},
    item/.style={draw, rounded corners=2pt, fill=yellow!32, fill opacity=0.5, text width=72mm, 
    align=left,inner sep=4pt},
    badge/.style={draw, rounded corners=2pt, fill=blue!32, fill opacity=0.5, inner xsep=3pt, inner ysep=1.5pt},
    sub_new/.style={draw, rounded corners=2pt, fill=yellow!32, fill opacity=0.5, text width=75mm, 
    align=left,inner sep=4pt},
  }
}

\begin{forest} taxo
[{\rotatebox{90}{\textbf{DATA~  \ref{subsec: data}}}}, draw, inner sep=1pt, fill opacity=.5
  [{Collection}, opacity=.5, text width=12mm
    [{Human Teleoperation \\ and Demonstration}, sub_1
      [{Cost-Effective and \\ calable Teleoperation}, sub
        [{{Young et al.~\cite{young2021visual}, AnyTeleop~\cite{qin2023anyteleop}, GELLO~\cite{wu2024gello},\\ UMI~\cite{chi2024universal}, OPEN~TEACH~\cite{iyer2025open}}}, item]
      ]
      [{Feedback-Rich Teleoperation \\ for Contact and Dexterity}, sub
        [{{M2R~\cite{kim2023training}, ALPHA-BiACT~\cite{kobayashi2025alpha}, 
        RDP~\cite{xue2025reactive}, \\Bunny-VisionPro~\cite{ding2024bunny}}}, item]
      ]
      [{Egocentric and XR Interfaces \\ Aligning Viewpoints}, sub
        [{{Zhang et al.~\cite{zhang2018deep}, EgoMimic~\cite{kareer2025egomimic}, 
        ARCap~\cite{chen2024arcap},\\ Dhouioui et al.~\cite{dhouioui2024perspective}, 
        AV-ALOHA~\cite{chuang2024active}}}, item]
      ]
      [{Embodiment Alignment via \\ Exoskeletons and Replica Arms}, sub
        [{{AirExo~\cite{fang2024airexo}, DexUMI~\cite{xu2025dexumi}, 
        Tilde~\cite{si2024tilde}, TeleMoMa~\cite{dass2024telemoma}}}, item]
      ]
    ]
    [{Huma-in-the-Loop \\ Enhancement}, sub_1
      [{{RoboCat~\cite{bousmalis2023robocat}, DexCap~\cite{wang2024dexcap}, 
      IntervenGen~\cite{hoque2024intervengen}, CR-DAgger~\cite{xu2025compliant}}}, sub_new]
    ]
    [{Synthetic/Automatic \\ Data Generation}, sub_1
      [{Leverage LLM/VLM for Generation}, sub
        [{{DIAL~\cite{xiao2023robotic}, Ha et al.~\cite{ha2023scaling}, 
        SPRINT~\cite{zhang2024sprint}, \\Manipulate-Anything~\cite{duan2025manipulate}, 
        SOAR~\cite{zhou2025autonomous}, NILS~\cite{blank2025scaling}, SEIL~\cite{jia2023seil}}}, item]
      ]
      [{Synthetic Sub-Trajectory Generation}, sub
        [{{MimicGen~\cite{mandlekar2023mimicgen}, DexMimicGen~\cite{jiangdexmimicgen}, 
        SkillMimicGen~\cite{garrett2025skillmimicgen},\\ IntervenGen~\cite{hoque2024intervengen}, 
        DemoGen~\cite{xue2025demogen}}}, item]
      ]
    ]
    [{Crowdsourcing-based \\ Data Collection}, sub_1
      [{{RoboTurk~\cite{mandlekar2018roboturk}, 
      David et al.~\cite{david2024unpleasantness}, 
      MART~\cite{tung2021learning}, 
      AR2-D2~\cite{duan2023ar2}, \\
      EgoZero~\cite{liu2025egozero}, 
      Chung et al.~\cite{chung2014accelerating}}}, sub_new]
    ]
  ]
  [{Utilization}, opacity=.5, text width=12mm
    [{Data Selection}, sub_1
      [{{EAD~\cite{gandhi2023eliciting}, 
      EIL~\cite{zheng2023extraneousness}, 
      DC-IL~\cite{belkhale2023data}, 
      UVP~\cite{dasari2023unbiased}, 
      L2D~\cite{kuhar2023learning}, \\
      ILID~\cite{yue2024leverage}, 
      Re-Mix~\cite{hejna2025remix}, 
      MimicLabs~\cite{saxena2025matters}}}, sub_new]
    ]
    [{Data Retrieval}, sub_1
      [{{VINN~\cite{pari2022surprising}, 
      SAILOR~\cite{nasiriany2023learning}, 
      Behavior Retrieval~\cite{du2023behavior}, \\
      Di Palo \& Johns~\cite{di2024effectiveness}, 
      DINOBot~\cite{di2024dinobot}, 
      RAEA~\cite{zhu2024retrieval}, 
      GSR~\cite{yin2024offline}, \\
      FlowRetrieval~\cite{lin2025flowretrieval}, 
      STRAP~\cite{memmel2025strap}, 
      COLLAGE~\cite{kumar2025collage}}}, sub_new]
    ]
    [{Data Augmentation}, sub_1
      [{Label and Trajectory Relabeling}, sub
        [{{DAAG~\cite{di2025diffusion}, 
        S2I~\cite{chen2025towards}, 
        GoalGAIL~\cite{ding2019goal}, 
        OILCA~\cite{he2023offline}}}, item]
      ]
      [{Physics- and Geometry-consistent\\ Augmentation}, sub
        [{{Mitrano \& Berenson~\cite{mitrano2022data}, 
        Wang et al.~\cite{wang2023identifying}}}, item]
      ]
      [{Generative Visual, Viewpoint, \\ and Embodiment Augmentation}, sub
        [{{GenAug~\cite{chen2023genaug}, 
        RoVi-Aug~\cite{chen2025rovi}, 
        RoboPearls~\cite{tang2025robopearls}, \\
        ROSIE~\cite{zhu2024retrieval}, 
        DMD~\cite{zhang2024diffusion}, 
        VISTA~\cite{tian2025view}, 
        DABI~\cite{kobayashi2025dabi}}}, item]
      ]
    ]
    [{Data Expansion}, sub_1
      [{Synthesis and Imagined Rollouts}, sub
        [{{Generative Predecessor Models~\cite{schroecker2019generative},        
        TASTE-Rob,~\cite{zhao2025taste}, \\
        Self-Imitation by Planning~\cite{luo2021self}, SAFARI~\cite{di2020safari},\\
        Category-Level Manipulation~\cite{shen2022learning}}}, item]
      ]
      [{Reuse and Corrective Expansion}, sub
        [{{Scalable Multi-Task IL~\cite{singh2020scalable}, 
        JUICER~\cite{ankile2024juicer}, 
        Diff-DAgger~\cite{lee2025diff}}}, item]
      ]
    ]
    [{Data Reweighting}, sub_1
      [{{Beliaev et al.~\cite{beliaev2022imitation}, 
      FABCO~\cite{takahashi2025feasibility}, 
      PLARE~\cite{luu2025policy}}}, sub_new]
    ]
  ]
]
\end{forest}
\caption{Overview of robot learning data taxonomy.}
\label{fig: data-taxonomy-colored}
\end{figure*}



==> tables/8_applications/application.tex <==
\begin{table*}[ht]
\label{tab: app}
\centering
\caption{Applications of Robotic Manipulation.}
\begin{tabular}{lllll}
\toprule
\textbf{Area} & \textbf{Task Example} &  \textbf{Task Description} & \textbf{Applicable Model} \\
\midrule
\multirow{5}{*}{Household Robots}  
  & Object rearrangement & Putting household items back to their designated places. & e.g., Stable Diffusion \cite{jin2025paca} \\
  & Surface cleaning & Wiping or tidying flat surfaces such as tables or counters. & e.g., VLA \cite{li2025hamster}  \\
  & Laundry folding & Folding clothes using two-handed manipulation. & e.g., LLAMA \cite{chen2025metafold}\\
\midrule
\multirow{5}{*}{Industrial Robots}  
  & Human-robot collaboration & Assisting humans in flexible manufacturing tasks. & e.g., DNN \cite{liu2018deep} \\
  & Robot assembly & Learning to assemble components in structured tasks like peg-in-hole. & e.g., DQN\cite{li2022flexible} \\
  & Mobile Manipulation & Performing complex tasks involving both navigation and object interaction. & e.g., VLA\cite{wu2025momanipvla} \\
  \midrule
  \multirow{5}{*}{AI4Science}  
  & Medical Science & Assisting in medical tasks, e.g., surgery. & e.g., VLA \cite{he2025capsdt} \\
  & Physical Science & Assisting in physical tasks, e.g., sports  & e.g.,  SNN \cite{wang2025spikepingpong}\\
  & Chemical Science & Assisting in chemical tasks, e.g., chemical research. & e.g., LLAMA \cite{song2025multiagent}\\
  \midrule
  \multirow{5}{*}{Agriculture}  
  & Robotic planting and seeding & Automating the process of planting seeds in agricultural fields.  & e.g., VLA \cite{sapkota2025vision} \\
  & Robotic harvesting & Automating the detection and picking of crops using robotic system & e.g.,  Detection network \cite{alaaudeen2024intelligent}\\
& Robotic weeding & Identifying and removing weeds using vision-guided robotic systems & e.g., YOLOX \cite{zhu2022yolox} \\

  
  

  
  
\bottomrule
\end{tabular}
\end{table*}

% a r

==> tables/main_table.tex <==
% \begin{table*}[htbp]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{1.2cm}  % Category列宽
% >{\raggedright\arraybackslash}p{0.8cm}   % Type列宽
% >{\raggedright\arraybackslash}p{2cm}
% >{\raggedright\arraybackslash}p{2.2cm}
% >{\raggedright\arraybackslash}p{2.8cm}
% >{\raggedright\arraybackslash}p{2.2cm}
% >{\raggedright\arraybackslash}p{3.0cm}
% >{\raggedright\arraybackslash}p{3.0cm}}
% \toprule
% \textbf{Method} & \textbf{Category} & \textbf{Core Idea} & \textbf{Modalities} & \textbf{Data Regime} & \textbf{Advantages \& Use Cases} & \textbf{Limitations} \\
% \midrule

% \multirow{6}{*}{SayCan} & \multirow{6}{*}{High-level Planner} & PaLM-540B & BC-Z & (I) Internet-scale text data; (II) 80K demos & Strong semantic reasoning and task decomposition & High cost; may violate physical constraints \\
% \cmidrule(lr){1-7}
% & & Code as Policies &  &  & High compositionality and interpretability & Unsafe or invalid code may be generated \\
% \cmidrule(lr){1-7}
% & & VoxPoser &  &  & Strong physical grounding & Relies on predefined geometry; limited semantics \\
% \cmidrule(lr){1-7}
% & & CLIPort &  &  & Action-centric interaction & Affordance ambiguity in cluttered or novel scenes \\
% \cmidrule(lr){1-7}
% & & F3RM &  &  & Rich spatial reasoning & Sensitive to reconstruction errors and dynamics \\
% \midrule

% \multirow{10}{*}{RT-1} & \multirow{10}{*}{Low-level Action Modelling} & - & VE: EfficientNet, VLM: Transformer policy, AH: MLP &  &  &  \\
% \cmidrule(lr){1-7}
% & & OpenVLA & - & VE: SigLIP \& DINO v2, VLM: LLaMA2, AH: LM &  & Strong LLM alignment and scalability & Action discretization limits precision \\
% \cmidrule(lr){1-7}
% & & PI0.5 & - & VE: SigLIP, VLM: Gemma, AH: FM &  & Continuous action modeling with smooth trajectories & Higher computational cost \\
% \cmidrule(lr){1-7}
% & & UniVLA & - &  &  &  \\
% \cmidrule(lr){1-7}
% & & OpenHelix & - &  &  & Efficient real-time control & Limited high-level reasoning \\
% \cmidrule(lr){1-7}
% & & Hi Robot & PaliGemma-3B & PI0 &  &  &  \\
% \cmidrule(lr){1-7}
% & & VLA-Adapter & - &  &  & Parameter-efficient adaptation & Strongly depends on backbone quality \\
% \cmidrule(lr){1-7}
% & & ReconVLA & - &  &  &  &  \\
% \cmidrule(lr){1-7}
% & & SpatialVLA & - &  & Improved 3D spatial reasoning & Depends on accurate scene reconstruction \\
% \cmidrule(lr){1-7}
% & & LAPA & - &  &  &  &  \\

% \bottomrule
% \end{tabular}
% }
% \caption{Comparison table with Category column added next to Method.}
% \label{tab:method_comparison_with_category}
% \end{table*}
\begin{table*}[t]

\centering
\scriptsize
\caption{Comparison table copied directly from the original spreadsheet without modifying filled or empty entries.}
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{0.6cm}
>{\raggedright\arraybackslash}p{2.5cm}
>{\raggedright\arraybackslash}p{2.2cm}
>{\raggedright\arraybackslash}p{3.5cm}
>{\raggedright\arraybackslash}p{2.0cm}
>{\raggedright\arraybackslash}p{2.9cm}
>{\raggedright\arraybackslash}p{2.6cm}
>{\raggedright\arraybackslash}p{2.4cm}}
\toprule
\textbf{Type}& \textbf{Category} & \textbf{Representative Method} & \textbf{Core Idea} & \textbf{Modalities} & \textbf{Data Regime} & \textbf{Advantages \& Use Cases} & \textbf{Limitations} \\
\midrule

\multirow{13}{*}{\rotatebox{90}{\makebox[10cm][c]{High-level Planner}}}

& \makecell[l]{LLM-based \\ Task Planning \\ (Section II-A)} &SayCan&LLM-planned global reasoning with affordance-grounded feasibility & RGB images, language & (I) Internet-scale text data; (II) 80K Robotic Data & Strong semantic reasoning and task decomposition & High cost; may violate physical constraints \\
\cmidrule(lr){2-8}
& MLLM-based \newline Task Planning \newline (Section II-B)& PaLM-E & Embodied multimodal LLM for end-to-end task reasoning & RGB image, state estimation, language & 
(I) Internet-scale vision-language; (II) Less than 10\% robotics data & Unified perception and reasoning; positive transfer across tasks & High cost; may lose language capabilities \\
\cmidrule(lr){2-8}
& Code Generation (Section II-C)&Code as Policies& LLM generates executable code; calls perception and control APIs & language, perception API, control primitives & (I) Few-shot prompting with API hints ; (II) Instruction-code examples & High compositionality and interpretability & Unsafe or invalid code may be generated \\
\cmidrule(lr){2-8}
&  Geometric \newline Constraint-based\newline Planning\newline (Section II-D)&VoxPoser& Builds 3D value maps from language-vision for smooth motion  & RGB images, language, 3D voxel maps & Zero-shot & Strong physical grounding & Relies on predefined geometry; limited semantics \\
\cmidrule(lr){2-8}
& Affordance\newline Learning\newline (Section II-E)&CLIPort & Decouples semantics and localization: CLIP grounding, Transporter pick-and-place& RGB images, language & Expert demonstrations
(1-1000 per task, 10 tasks) & Action-centric interaction & Affordance ambiguity in cluttered or novel scenes \\
\cmidrule(lr){2-8}
& 3D\newline Representations\newline as Planner\newline (Section II-F)&F3RM& Distills CLIP into 3D fields for language-based pick-and-place & RGB images, language, 3D geometry& 10 demonstrations (2 per task, 5 tasks)  & Rich spatial reasoning & Sensitive to reconstruction errors and dynamics \\
\midrule

\multirow{10}{*}{\rotatebox{90}{\makebox[16cm][c]{Low-level Action Modelling}}}
& 2D\newline Non-LLM-based\newline VLA\newline (Section III-B2a)&RT-1& Transformer maps vision and language to actions; discretization enables low-level control & RGB images, language & (I) 130K robot demonstrations; (II) 744 tasks from 13 robots & Demonstration scalability and diverse manipulation skills & Weak semantic priors; limited generalization and cross-domain transfer \\
\cmidrule(lr){2-8}
& 2D \newline LLM/VLM-based\newline VLA\newline (Section III-B2a)&OpenVLA& Fine-tunes Prismatic VLM on robot data; fuses SigLIP and DINOv2 with discrete action tokens & RGB images, language & (I) Internet-scale vision-language data; (II) Open X-Embodiment (970K) & Strong LLM alignment and scalability & Action discretization limits precision \\
\cmidrule(lr){2-8}
& Latent Learning\newline for VLA\newline (Section III-B2a)& LAPA & Learns discrete latent actions via VQ-VAE; VLM predicts latent actions &  RGB images, language & (I) Large unlabeled robot video data %(e.g., Bridgev2 60K); 
(II) 100-450 labeled trajectories  & Efficient and transferable latent action abstractions &  Inference latency \\
\cmidrule(lr){2-8}
& Action\newline Quantization\newline for VLA\newline (Section III-B2a)& MiniVLA & Learns quantized motor codebooks; trajectory discretization for stable training 
& RGB images, language & (I) Llava-1.5-Instruct VQA dataset; (II) LIBERO-90 and Bridge V2 & Reduced complexity and stabilized training & Difficulty in semantic consistency and collapse avoidance \\ 
\cmidrule(lr){2-8}
& Dual-/Multi-system VLA (Section III-B2a)&OpenHelix& Dual-system VLA:frozen MLLM and pre-trained policy; separates fast reactive control and slow deliberative reasoning & language, 3D scene representation, RGB, proprioception  &  CALVIN Dataset & Efficient real-time control & Limited high-level reasoning \\
\cmidrule(lr){2-8}
& Learning with Auxiliary Tasks (Section III-B2a)  & PI0.5 & Hierarchical inference with subtask prediction; flow matching action generation
%; deterministic transport dynamics for smoother trajectories 
& RGB images, language, proprioception & (I) 400H Mobile Manipulator Data; (II) 97.6\%  Web Data & Continuous action modeling with smooth trajectories & Higher computational cost \\
\cmidrule(lr){2-8}
& Reinforcement \newline Learning\newline (Section III-B2a)&VLA-RL& Large-scale rollout RL refinement, multi-turn conversation formulation; PPO with robotic reward densification & RGB images, language, proprioception & (I) Open X-Embodiment; (II) LIBERO 40 tasks RL data   & Scalable refinement from sparse feedback and execution-aligned action decoder & Extensive online interaction and critic dependence \\
\cmidrule(lr){2-8}
& Efficient VLA\newline (Section III-B2a)&VLA-Adapter& Parameter-efficient adapters; all-layer latents and bridge attention for efficient action generation & RGB images, language, proprioception & 150K steps on LIBERO and CALVIN datasets & Parameter-efficient adaptation & Strongly depends on backbone quality \\
\cmidrule(lr){2-8}
& Robustness \newline (Section III-B2a)&BadVLA& Objective-decoupled backdoor attacks; reveals VLA security vulnerabilities & RGB images, language & (I) Open X-Embodiment; (II) poisoned training samples on LIBERO and SimplerEnv& Robust to input perturbations and fine-tuning & Limited to training-time injection \\
\cmidrule(lr){2-8}
&3D VLA\newline (Section III-B2b)&SpatialVLA& Introduces 3D positional encodings and adaptive action grids; captures transferable spatial priors & 3D point clouds or depth, RGB, language & 1.1M real robot episodes & Improved 3D spatial reasoning & Depends on accurate scene reconstruction \\


\bottomrule
\end{tabular}
}

\label{tab:method_comparison}
\end{table*}
